Post-Quantum Multi-Party Computation

We initiate the study of multi-party computation for classical functionalities (in the plain model) with security against malicious polynomial-time quantum adversaries. We observe that existing techniques readily give a polynomial-round protocol, but our main result is a construction of *constant-round* post-quantum multi-party computation. We assume mildly super-polynomial quantum hardness of learning with errors (LWE), and polynomial quantum hardness of an LWE-based circular security assumption. Along the way, we develop the following cryptographic primitives that may be of independent interest: 1. A spooky encryption scheme for relations computable by quantum circuits, from the quantum hardness of an LWE-based circular security assumption. This yields the first quantum multi-key fully-homomorphic encryption scheme with classical keys. 2. Constant-round zero-knowledge secure against multiple parallel quantum verifiers from spooky encryption for relations computable by quantum circuits. To enable this, we develop a new straight-line non-black-box simulation technique against *parallel* verifiers that does not clone the adversary's state. This forms the heart of our technical contribution and may also be relevant to the classical setting. 3. A constant-round post-quantum non-malleable commitment scheme, from the mildly super-polynomial quantum hardness of LWE.

==> basic-nmc-aborting.tex <==
\subsection{Post-Quantum Non-Malleable Commitments.}

%todo: attach ZK proofs, do GK style analysis.

==> cointossold.tex <==
\iffalse{
\begin{claim}
\label{clm:ow}
$$\Big\{ \hyb_1 \Big\}_{\secp \in \mathbb{N}}
\approx_s
\Big\{ \hyb_2 \Big\}_{\secp \in \mathbb{N}}$$
\end{claim}
\begin{proof}
Let $\mathsf{BAD}_{A^*}$ denote the set of transcripts in $\hyb_1$ that do not abort (i.e. the adversary's proofs were accepted and the adversary did not abort elsewhere), and yet the check fails.
To prove this claim, it suffices to prove that 

\begin{align} \label{eq:ct-h2-bad-event-1}
\Pr[\tau \in \mathsf{BAD}_{A^*}|\tau \leftarrow \hyb_1] = \negl(\secp)    
\end{align}    

Suppose Equation~(\ref{eq:ct-h2-bad-event-1}) is false. Then there exists a polynomial $\poly(\cdot)$ such that for infinitely many $\secp \in \bbN$:
%
\begin{align} \label{eq:ct-h2-bad-event-2}
    \Pr[\tau \in \mathsf{BAD}_{A^*}|\tau \leftarrow \hyb_1] \ge \frac{1}{\poly(\secp)}
\end{align}
which implies that $A^*$ contradicts soundness of the protocol $\zk$ according to Definition \ref{def:qsczk}. 
\end{proof}
%
%Then $A^*_\secp$ yields a prover $\zkmP^*_\secp$ that contradicts soundness according to Definition \ref{def:qsczk} of \pibs, that is,
%, in Step 6 of \proref{fig:ct}.
%Specifically, we show that there exists a $\mathsf{QPT}$ prover $\zkmP = \{\zkmP_\secp, \rho_\secp\}_{\secp \in \mathbb{N}}$ and a polynomial $\poly(.)$  such that for infinitely many $\secp \in \bbN$, $\exists i = i(\secp) \in [n(\secp)], x \in \{0,1\}^\secp \setminus \mathcal{L}$ such that
%\begin{align}
%    \Pr[\mathsf{OUT}_{\zkV_i}\langle\zkmP_\secp(\rho_\secp),\zkV_i(x)\rangle (1^\secp,1^n) = 1] \geq \frac{1}{\poly(\secp)}
%\end{align}
%The adversary $\zkmP$ which contradicts the soundness property works as follows: It
%$\zkP^*$ participates as a prover in a \pibs session with the challenger where the challenger behaves as an honest verifier. At the same time, $\zkmP$ participates as an honest player in the coin-tossing protocol with adversary $A^*$. While behaving as an honest player in the coin-tossing protocol, it sends all messages as prescribed in \proref{fig:ct}. While performing as an honest verifier in Step 6 \proref{fig:ct} with $A^*$ being the prover, it first sends across the statement $x$ and language $\cL$ (which $A^*$ wants to prove) to the challeneger, and then transparently forwards messages back and forth between the challenger and $A^*$. After this, it completes the remaining coin-tossing protocol honestly with $A^*$.\\
%
%We now calculate the probability that $\zkmP$ contradicts soundness of $\pibs$. Note that this probability is exactly equal to the probability of $\mathsf{BAD}$ event conditioned on the fact that $A^*$ proofs were accepted and that $A^*$ didn't abort elsewhere. Therefore,
%\begin{align}
%    \Pr[\mathsf{OUT}_{\zkV_i}\langle\zkmP_\secp(\rho_\secp),\zkV_i(x)\rangle (1^\secp,1^n) = 1]
%    =
%    \Pr[\tau \in \mathsf{BAD}|\tau \leftarrow \hyb_1]
%    \ge \frac{1}{\poly(\secp)}
%\end{align}
%
%which is a contradiction as desired.



%Set $(x_\secp, L_\secp) = (\{x_{i^*,j}\}_{j \in \mathbb{S}}, \{L_{i^*,j}\}_{j \in \mathbb{S}})$ as defined below.
%\begin{itemize}
    %\item $L_{i^*,j} = \{ (a, b, m) | \exists (r_1,r_2)$ s.t. $\piext_{p_{i^*,j}}(m;r_1) = a$, %$\piext_{q_{i,j}}(m;r_2) = b$, and
    %$\pinm_{t_{i^*,j}}(m,r_1;r_2) = b\}$ where $\piext_{h}$ (resp. $\pinm_{h}$) denotes an execution of $\piext$ (resp. $\pinm$) with receiver messages set to $h$.
    %\item $x_{i^*,j} = (\alpha_{i^*,j}, \beta_{i^*,j}, c_{i^*})$ where 
    %$\alpha_{i^*,j}$ and $\beta_{i^*,j}$ denote the transcript of committer %messages with $P_j$ as receiver and $P_i^*$ as committer respectively, and $c_{i^*}$ denotes the message sent on behalf of $P_{i^*}$ in Step 4.
%\end{itemize}
%\begin{itemize}
%    \item $\alpha_{i, j}$ and $p_{i,j}$ denote the sets of committer and receiver messages respectively with $P_i$ as committer and $P_j$ as receiver in Step 3, 
    %\item $\beta_{i, j}$ and $q_{i,j}$ denote the sets of committer and receiver messages respectively with $P_i$ as committer and $P_j$ as receiver in Step 4,
%    and
%    \item $\beta_{i,j}$ and $t_{i,j}$ denote the sets of committer and receiver messages respectively with $P_i$ as committer and $P_j$ as receiver in Step 2.
%\end{itemize}
%\item If an abort occurs in the process above, output $\bot$. 

%\item Set $\sigma^{x(\secp)}_{\secp} = (\tau, \overline{\rho}_\secp)$.
%, \{c'_j\}_{j \in \mathbb{S}})$, where recall $c'_j$ is the output of $\mathsf{ECom}.\mathsf{Ext}$ in Step 3.

%\item Generate proofs in Step 6 for all parties in $\mathbb{H}\setminus\{i^*\}$ using honest prover strategy according to \proref{fig:ct}.
%Additionally in all proof sessions where $P_{i^*}$ is the prover, generate proofs by executing the zero-knowledge simulator $\pibs.\simulator$ on behalf of party $P_{i^*}$. Formally, let $\zkV^*_\secp$ be a machine that forwards the verifier messages generated by $\{P_j\}_{j \in \mathbb{S}}$ in sessions where $P_{i^*}$ is prover. Then execute $\pibs.\simulator(1^\secp,1^n,\mathbb{S},\zkV^*_\secp, \sigma_\secp^{(x_\secp)})$.
%If the adversary aborts or fails to produce an accepting proof, then output $\bot$. 
%Generate all other messages identically to $\hyb_2$.
\begin{claim}
\label{clm:tw}
$$\Big\{ \hyb_2 \Big\}_{\lambda \in \mathbb{N}} \approx_c \Big\{ \hyb_3 \Big\}_{\lambda \in \mathbb{N}}$$
\end{claim}
\begin{proof}
Suppose the claim is false. Then there exists a $\mathsf{QPT}$ distinguisher $\eD$ and a polynomial $\poly(\cdot)$ such that for infinitely many $\secp \in \bbN$,
%
\begin{align} 
    \Big |
    \Pr[\eD(\hyb_2) = 1] -
    \Pr[\eD(\hyb_3) = 1]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align}
%
We will use $\eD$ to construct a verifier $\zkV^*$ which contradicts Claim \ref{claim:ind-non-abort}.
%(used in Step 6 of \proref{fig:ct})

%Specifically, we will demonstrate that:
%\dnote{denote by $\pibs.\simulator$}
%$\forall$ QPT simulator \simulator, $\exists$ non-uniform QPT $\zkV^* = \{\zkV^*_\secp, \rho_\secp \}_{\secp \in \bbN}$ representing a subset of $n$ verifiers, namely, $\{\zkV_i\}_{i \in I}$ for some set $I \subseteq [n]$ (and where $\{\rho_\secp\}_{\secp \in \mathbb{N}}$ is a polynomial-size $|I|$-instance-advice distribution), $\exists$ an instance-witness pair $(x_{i,\secp} \in \cL \cap \{0,1\}^\secp, w_{i,\secp} \in \cR_\cL), i \notin I$, for infinitely many $\secp \in \mathbb{N}$,

%\dnote{negate}
%\begin{align*}
%    &\left\{\{x_{i,\secp}\}_{i \in I}, \view_{\zkmV_\secp} \left\langle \begin{array}{c} \{\zkP_i(x_{i,\secp},w_{i,\secp})\}_{i \in [n]}, \\\zkmV_\secp(\rho_\secp^{\{x_i\}_{ \in I}}), \\ \{\zkV_i(x_{i,\secp})\}_{i \notin I} \end{array}\right\rangle (1^\secp,1^n) \ \bigg| \ \left(\{x_{i,\secp}\}_{i \in I}, \rho_\secp^{\{x_i\}_{i \in I}}\right) \leftarrow \rho_\secp \right\}_{\secp \in \mathbb{N}}\\ \approx_c     &\{\mathsf{Sim}(1^\secp,1^n,I,\zkmV_\secp, O_{\rho_\secp})\}_{\secp \in \mathbb{N}},
%\end{align*}
%where for a mixed state $\rho$, $O_\rho$ is an inputless oracle that upon activation returns a sample $\rho$.

We define the instance-advice distribution $(x_\secp, \sigma_\secp^{(x_\secp)})$ given to $\zkV^*$ as in the description of $\hyb_3$.
%
%The adversary $\zkV^*$ participates as a verifier in a $\pibs$ protocol with the challenger. The challenger either takes the role of honest prover $\zkP$ or executes $\pibs.\simulator(1^\secp, x_\secp, \zkV^*_\secp, \sigma_\secp^{(x_\secp)})$.

%$\zkV^*$ sets $A^*$'s state according to $\sigma_\secp^{(x_\secp)}$, and then on behalf of honest party $P_i$ in the $\pibs$ session where $A^*$ is the verifier, it forwards messages back and forth between the challenger and $A^*$. It generates all remaining messages in the coin tossing protocol, honestly.
%If $A^*$ aborts or if $\pibs.\simulator$ fails to produce a transcript, output $\bot$.
$\zkV^*$ receives either the real or simulated view, forwards this to $\eD$, and then mirrors the response of $\eD$. As a result,
%waits for a response. 
%If $\eD$ returns 0, $\zkV^*$ outputs 0; otherwise $\zkV^*$ outputs 1.
%
%\anote{How can $\zkV^*$ send the inner state of $A^*$ to $\eD$ since $A^*$ inner state might be private.}
%
%We now analyze the probability that $\zkV^*$ succeeds in contradicting Claim \ref{claim:ind-non-abort}. To this end, note that depending on whether the challenger takes the role of an honest prover $\zkP$ or executes $\pibs.\simulator(1^\secp, x_\secp, \zkV^*_\secp, \sigma_\secp^{(x_\secp)})$, the experiment corresponds to $\hyb_2$ or $\hyb_3$ respectively. Also, depending on whether the challenger takes the role of an honest prover $\zkP$ or executes $\pibs.\simulator(1^\secp, x_\secp, \zkV^*_\secp, \sigma_\secp^{(x_\secp)})$, the view of $V^*$ in the challenge session is same as $\mathsf{Real}_\bot(\zkV^*)$ and $\zkSim_\bot(\zkV^*)$ respectively, as defined in Claim \ref{claim:ind-non-abort}. Therefore,
%
\begin{align*}
    & \Pr[\zkV^*\big(\mathsf{Real}_\bot(\zkV^*) \big) = 1] = \Pr[\eD(\hyb_2) = 1], 
    \Pr[\zkV^*\big(\zkSim_\bot(\zkV^*)\big) = 1] = \Pr[\eD(\hyb_3) = 1] \\
%\end{align*}
%This implies
%\begin{align*}
    & \text{This implies that }\Big |
    \Pr[\zkV^*\big(\mathsf{Real}_\bot(\zkV^*) \big) = 1]
    -   \Pr[\zkV^*\big(\zkSim_\bot(\zkV^*)\big) = 1]
    \Big |
    %= \Big |
    %\Pr[\eD(\hyb_2) = 1] -
    %\Pr[\eD(\hyb_3) = 1]
    %\Big | 
    \ge 
    \frac{1}{\poly(\secp)}
\end{align*}
%
which is a contradiction, as desired.
%\dnote{Add}
\end{proof}




%generate $\pinm$ in Step 2 on behalf of party $P_{i^*}$, for all $j \in [n]$, by executing $\eC(0^{p(\secp)};s_{i^*,j})$ with uniform randomness $s_{i^*,j}$.
%\anote{The value inside $\eC$ is not consistent with the protocol requirement. Should be $\eC(0^{p(\secp)}, r_{i^*, j};s_{i^*,j})$}

\begin{claim}
$$\Big\{ \hyb_3 \Big\}_{\lambda \in \mathbb{N}} \approx_c \Big\{ \hyb_4 \Big\}_{\lambda \in \mathbb{N}}$$
\end{claim}
\begin{proof}
We define distributions $\hyb_3'$ and $\hyb_4'$ that are identical to $\hyb_3$ and $\hyb_4$ respectively, except that $\hyb_3'$ and $\hyb_4'$ {\em do not} perform the additional check described in $\hyb_2$, and as such, never attach $\cfail$ to the output.

To prove that $\hyb_3$ and $\hyb_4$ are computationally indistinguishable, it suffices to prove the following equations:
\begin{align}
    \Big\{ \hyb_3 \Big\}_{\lambda \in \mathbb{N}} \approx_c \Big\{ \hyb'_3 \Big\}_{\lambda \in \mathbb{N}} \label{eq:twenty} \\
    \Big\{ \hyb'_3 \Big\}_{\lambda \in \mathbb{N}} \approx_c \Big\{ \hyb'_4 \Big\}_{\lambda \in \mathbb{N}} \label{eq:twentyone} \\
    \Big\{ \hyb'_4 \Big\}_{\lambda \in \mathbb{N}} \approx_c \Big\{ \hyb_4 \Big\}_{\lambda \in \mathbb{N}} \label{eq:twentytwo}
\end{align}
%
Here Equation~(\ref{eq:twenty}) follows from \cref{clm:ow} and \cref{clm:tw},which imply that
%
\begin{align} \label{eq:be}
\Pr[\tau \in \mathsf{BAD}_{A^*,\hyb_3}|\tau \leftarrow \hyb_3] = \negl(\secp)    
\end{align}
%
where $\mathsf{BAD}_{A^*, \hyb_3}$ denotes the set of transcripts in $\hyb_3$ that do not abort (i.e. the adversary's proofs were accepted and the adversary did not abort elsewhere), and yet the (inefficient) check fails.

Equation~(\ref{eq:twentyone}) follows by the hiding of the commitment scheme $\nmCom$. 

In what follows, we prove Equation~(\ref{eq:twentytwo}). 
Let $\mathsf{BAD}_{A^*, \hyb_4}$ denote the set of transcripts in $\hyb_4$ that do not abort (i.e. the adversary's proofs were accepted and the adversary did not abort elsewhere), and yet the (inefficient) check fails.
To prove Equation~(\ref{eq:twentytwo}), it suffices to prove that 
%
\begin{align} \label{eq:be2}
\Pr[\tau \in \mathsf{BAD}_{A^*, \hyb_4}|\tau \leftarrow \hyb_4] = \negl(\secp)    
\end{align}    
%
Suppose towards a contradiction that Equation~(\ref{eq:be2}) is not true. 
This implies that there exists a polynomial $p(\cdot)$ such that for large enough $\lambda \in \mathbb{N}$,
\begin{align} \label{eq:be3}
\Pr[\tau \in \mathsf{BAD}_{A^*, \hyb_4}|\tau \leftarrow \hyb_4] \geq \frac{1}{p(\secp)}  
\end{align}    
which implies that in $\hyb_4$ for every large enough $\lambda \in \mathbb{N}$, there exists a $j^*$ such that $y_{j^*} \notin \LL$ with probability at least $\frac{1}{n \cdot p(\lambda)}$ (where $y_{j^*}$ was defined in $\hyb_2$).
%\begin{enumerate}
%\item $x = (\alpha_{j^*,i^*}, \beta_{j^*,i^*})$ denotes the transcript of committer messages with $P_{j^*}$ as committer and $P_{i^*}$ as receiver in Steps 2 and 3 respectively, and $c_{j^*}$ denotes the message sent by $P_{j^*}$ in Step 4,
%and 
%\item $L = \{ (a, b, m) | \exists (r_1,r_2)$ s.t. $\piext_{p_{j^*,i^*}}(m;r_1) = a$, %$\piext_{q_{j^*,i^*}}(m;r_2) = b$, and
%    $\pinm_{t_{j^*,i^*}}(m,r_1;r_2) = b\}$
%\end{enumerate}
%and where $i^*$ denotes the smallest index in $\mathbb{H}$.
   
We will use Equation~(\ref{eq:be3}) and (\ref{eq:be}) to contradict many-to-one non-malleability of $\pinm$, by building a $\mathsf{QPT}$ man-in-the-middle adversary $\mim_\secp$ that uses $A^*_\secp$ to contradict Definition~\ref{def:nmc}.

This adversary $\mim_\secp$ will interact with $|\corrupt|$ sessions of $P_{i^*}$ acting as committer on the left, and one session of $P_{i^*}$ acting as receiver on the right. The $P_{i^*}$ on the left will be committing to either $\{(0^{k(\secp)},0^\secp)\}_{j \in \corrupt}$ or $\{(c_{i^*},r_{i^*,j})\}_{j \in \corrupt}$.

%It samples $\{(c_{i^*}, r_{i^*,j}, s_{i^*,j})\}_{j \in [n]\setminus i^*}$ according to $\hyb_3$.
$\mim_\secp$ will obtain $(\rho_\secp, j^*)$ as non-uniform advice, and simulates the coin-tossing protocol with $A^*_\secp$ with initial state set to $\rho_\secp$. During step 3, it interacts with the challenger on the left committing to either $(c_{i^*}, r_{i^*,j})$ for every ${j \in \mathbb{S}}$, or to $(0^{k(\secp)},0^\lambda)$ on behalf of $P_{i^*}$. It forwards these on behalf of $P_{i^*}$ and uses the strategy in $\hyb_3$ to generate messages on behalf of all other honest parties. It sends these messages to $A^*_\secp$, and forwards receiver messages generated by $A^*_\secp$ to the challenger. Additionally, it forwards committer messages obtained from $P_{j^*}$ in its interaction with $P_{i^*}$ to the challenger on the right, and obtains receiver messages on behalf of $P_{i^*}$ from the challenger.

Finally, it obtains the messages $(c^*, r^*)$ committed by $P_{j^*}$ in its interaction with $P_{i^*}$ on the right. If this message was set to $\bot$, it aborts. It then completes an execution of the coin-tossing protocol with $A^*_\secp$ by executing the ZK simulator according to $\hyb_3$, and outputs $\bot$ if simulation fails or if there is an abort. 
If not, it checks whether $\beta^{(\com)}_{j^*, i^*}$ is obtained as the transcript of a commitment to $c^*$ with randomness $r^*$, and that $P_{j^*}$ outputs $c^*$ in Step 4.
If this check fails, $\mim_\secp$ outputs $1$, and otherwise $\mim_\secp$ outputs $0$. 

It follows from Equation~(\ref{eq:be}) and Equation~(\ref{eq:be3}) that 
$$\Pr[\mim_\secp = 1|\{\{(c_{i}, r_{i,j}, s_{i,j})\}_{j \in [n]\setminus i}\}_{i \in \mathbb{H}}] = \Pr[\mim_\secp = 1|\hyb_3] = \negl(\secp), \text{ and}$$
$$\Pr[\mim_\secp = 1|\{0^\secp\}_{j \in [n]\setminus i}\}_{i \in \mathbb{H}}] = \Pr[\mim_\secp = 1|\hyb_4] \geq \frac{1}{n\cdot p(\secp)}$$
which is a contradiction, as desired.
%\dnote{Add}
\end{proof}


\begin{claim}
\label{clm:gw}
$$\Big\{ \hyb_4 \Big\}_{\secp \in \mathbb{N}} \approx_c \Big\{ \hyb_5 \Big\}_{\secp \in \mathbb{N}}$$
\end{claim}
\begin{proof}
Suppose towards a contradiction, that the claim is not true. This implies that there exists a $\mathsf{QPT}$ distinguisher $\eD$ and a polynomial $\poly(.)$ such that for infinitely many $\secp \in \bbN$,
\begin{align} \label{eq:six}
    \Big |
    \Pr[\eD(\hyb_4) = 1] -
    \Pr[\eD(\hyb_5) = 1]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align}
We will use $\eD$ and $A^* = (A^*_\secp, \rho_\secp)$ to build a receiver $\eR^*$ that contradicts hiding of $\PECom$ according to Definition \ref{defn:qspec}.

$\eR^*_\secp$ obtains advice $\rho_\secp$ and the ``best possible'' transcript of Steps 1 and 2, together with the openings of all the commitments in Step 2. It proceeds as follows:
\begin{enumerate}
\item Initiate an interaction with a challenger for $\PECom$, obtaining $|\mathbb{S}|$ commitments to $c_{i^*}$ or to $0^{k(\lambda)}$. 
\item Forward the resulting commitments to $A^*_\secp$ in sessions where $P_{i^*}$ is committer. Generate messages on behalf of all other parties in $\mathbb{H}$ according to $\hyb_4$, and append the transcript and the adversary's state to the view.
\item Execute Step 4 according to $\hyb_4$.
\item Carry out the check described in $\hyb_2$, which is efficient given the opening of the non-malleable commitment (which $\eR^*_\secp$ has as advice).
\item Execute Step 5 according to $\hyb_5$.
\item If the adversary aborts or provides non-accepting proofs, output $\bot$. 
%\item If $\exists j \in \mathbb{S}$ such that $x_{j} \notin L$, it output $\mathsf{check}\text{-}\mathsf{fail}$, where:
%\begin{enumerate}
%\item $x_{j} = (\alpha_{j,i^*}, \beta_{j,i^*}, c_j)$ where $\alpha_{j,i^*}, \beta_{j,i^*}$ denotes the transcript of committer messages with $P_j$ as committer and $P_{i^*}$ as receiver in Steps 3, 4 respectively, and $c_j$ denotes the message sent by $P_j$ in Step 4, and 
%\item \small{$L = \{ (a, b, m) | \exists (r_1,r_2)$ s.t. $\piext_{p_{j,i}}(m;r_1) = a$, %$\piext_{q_{j,i^*}}(m;r_2) = b$, and $\pinm_{t_{j,i^*}}(m,r_1;r_2) = b\}$}
%\end{enumerate}
%Note that this check is efficient given the opening of the non-malleable commitment (which $\eR^*$ obtains as advice).
\item Finally, $\eR^*$ mirrors the output of $\eD$ on the resulting distribution. 
\end{enumerate}
Then by Equation~(\ref{eq:six}), we have that
\begin{align} \label{eq:six}
    \Big |
    \Pr[\eR^* = 1|c_i^*] -
    \Pr[\eR^* = 1|0^{k(\lambda)}]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align}
which contradicts hiding according to Definition~\ref{defn:qspec}, as desired.
\end{proof}




%by executing $\piext.\mathsf{Ext}$ in Step 3 on behalf of party $P_{i^*}$ for all $j \in [n]$.% instead of in Step 3. 
%If extraction fails or the adversary aborts at some point, output $\bot$. If the (inefficient) check fails, append $\cfail$ to the view.
%, by executing $\eC(0^\lambda;r_{i,j})$ with uniform randomness $s_{i,j}$.
\begin{claim}
\label{clm:hw}
$$\Big\{ \hyb_5 \Big\}_{\secp \in \mathbb{N}} \approx_c \Big\{ \hyb_6 \Big\}_{\secp \in \mathbb{N}}$$
\end{claim}
\begin{proof}
Suppose towards a contradiction, that the claim is not true. This implies that there exists a $\mathsf{QPT}$ distinguisher $\eD$ and a polynomial $\poly(.)$ such that for infinitely many $\secp \in \bbN$,
\begin{align} \label{eq:six}
    \Big |
    \Pr[\eD(\hyb_5) = 1] -
    \Pr[\eD(\hyb_6) = 1]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align}
We use this $A^*$ and $\eD$ to build a compliant distinguisher $\eD^*$ that contradicts extractability of the commitment according to Definition \ref{defn:qspec}.

%The adversary $\eC^*$ obtains advice $\rho_\secp$ and the ``best possible'' transcript of Steps 1 and 2, together with openings of all the commitments in Step 2. It proceeds as follows:

%\begin{enumerate}
    %\item It participates as $|I| = |\bbS|$ committers, namely, $\{\mathsf{C}_i\}_{i \in \bbS}$ in $\piext$ sessions with a challenger (which  plays the role of an honest receiver or executes $\piext.\mathsf{Ext}$ on $\eC^*$).
    
    %\item At the same time, $\eC^*$ takes the role of all honest parties $\bbH$ and initiates Step 3 of the coin-tossing protocol with adversary $A^*$.
    
    %\item While doing so, it sends all messages as prescribed in $\hyb_5$ with the following modification to Step 3: While behaving as a receiver on behalf of party $P_{i^*}$ in $\piext$, it forwards all messages generated by $A^*$ on behalf of $\{P_j\}_{j \in \mathbb{S}}$ to the challenger, and forwards messages from the challenger to $A^*$. This produces a set of $|I|$ commitment transcripts from $\eC^*$ to the challenger in accordance with Definition \ref{defn:qspec}.
    
    %\item It attaches all other messages generated by $A^*_\secp$, the state of $A^*_\secp$, as well as the non-uniform advice that it obtained, to its view.
%\end{enumerate}

$\eD^*$ obtains advice $\rho_\secp$ and the ``best possible'' transcript of Steps 1 and 2, together with the openings of all the commitments in Step 2. It proceeds as follows:
    
\begin{enumerate}
    \item Obtain input from the challenger either
    $\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\sigma_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^{n-1}))$ or $\cE(1^\secp,1^{n-1},\corrupt,\eC^*_\secp,\sigma_\secp)$ and then parse it as a tuple $(\{\tau_i\}_{i \in \corrupt},\state,\{c'_j\}_{j \in \corrupt})$.
    
    \item Use this information to finish generating the instance-advice distribution as in $\hyb_5$, including the check introduced in $\hyb_2$ which is again efficient given $\eD^*$'s non-uniform advice.
    
    %- indicating a set of transcripts, the state $\state$ of $A^*$, and the values (either real or extracted) committed by $\eC^*$.
    
    %\item Execute the remaining steps  of \proref{fig:ct} with $A^*$'s state initialized to $\state$, to obtain a view.
    
    %\item If the adversary aborts or provides non-accepting proofs, output $\bot$. 
    
    %\item As in $\hyb_5$ and $\hyb_6$, if $\exists j \in \mathbb{S}$ such that $x_j \notin L$, it additionally outputs $\mathsf{check}\text{-}\mathsf{fail}$, where:
    %\begin{enumerate}
    %\item $x_{j} = (\alpha_{j,i^*}, \beta_{j,i^*}, c_j)$ denotes the transcript of committer messages with $P_j$ as committer and $P_{i^*}$ as receiver in Steps 2 and 3, $c_j$ denotes the message sent by $P_j$ in Step 4.
    %\item $L = \{ (a, b, m) | \exists (r_1,r_2)$ s.t. $\piext_{p_{j,i^*}}(m;r_1) = a$, %$\piext_{q_{j,i^*}}(m;r_2) = b$, and
    %        $\pinm_{t_{j,i^*}}(m,r_1;r_2) = c\}$
    %\end{enumerate}
    %Note that these checks are efficient given the opening of the non-malleable commitment (which $\eD^*$ obtains as part of the view).
    
    \item If $\mathsf{check}$-$\mathsf{fail}$ occurs, $\eD^*$ outputs $0$.
    
    \item Otherwise, $\eD^*$ mirrors the output of $\eD$ on the resulting distribution. 
\end{enumerate}

We additionally define $\eD^*_1$ that behaves identically to $\eD^*$ except that in the last step, instead of mirroring the output of $\eD$ on the resulting distribution, $\eD^*$ outputs $1$.

%\dnote{The proof below is incomplete.}
Note that the check ensures that both $\eD^*$ and $\eD^*_1$ are compliant distinguishers according to Definition \ref{defn:qspec}. 

Additionally,
since 
$$\Pr[\mathsf{check}\text{-}\mathsf{fail} \text{ occurs in }\hyb_5] = \negl(\secp)$$
we have that
$$\Pr[\mathsf{check}\text{-}\mathsf{fail} \text{ occurs in }\hyb_6] = \negl(\secp)$$
otherwise 
\begin{align*}
& \Big| \Pr[\eD^* (\cE(1^\secp,1^{n-1},\corrupt,\eC^*_\secp,\sigma_\secp)) = 1] - \\
& \Pr[\eD^*_1(\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\sigma_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^{n-1}))) = 1] \Big| \\
& \geq \frac{1}{\poly(\secp)}
\end{align*}
contradicting Definition \ref{defn:qspec}.

Next,
%
\begin{align*}
    & \Pr[\eD^*(\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\sigma_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^{n-1}))) = 1]\\
    & =
    \Pr[\eD(\hyb_5) = 1| \neg \mathsf{check}\text{-}\mathsf{fail}], = \Pr[\eD(\hyb_5) = 1] \pm \negl(\secp), \text{ and } \\
    & \Pr[\eD^* (\cE(1^\secp,1^{n-1},\corrupt,\eC^*_\secp,\sigma_\secp)) = 1]\\
    & =
    \Pr[\eD(\hyb_6) = 1| \neg \mathsf{check}\text{-}\mathsf{fail}] = \Pr[\eD(\hyb_6) = 1] \pm \negl(\secp)
\end{align*}
which implies that there exists a polynomial $\poly(\cdot)$ such that
$$\Big |
    \Pr[\eD(\hyb_5) = 1|\neg \mathsf{check}\text{-}\mathsf{fail}] -
    \Pr[\eD(\hyb_6) = 1|\neg \mathsf{check}\text{-}\mathsf{fail}]
    \Big |  \ge 
    \frac{1}{\poly(\secp)}$$
%
This implies that for infinitely many $\secp \in \bbN$,
\begin{align*}
    &\Big | \Pr[\eD^*(\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\sigma_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^{n-1}))) = 1] - \Pr[\eD^* (\cE(1^\secp,1^{n-1},\corrupt,\eC^*_\secp,\sigma_\secp)) = 1 ] \Big| \\
    & =  \Big |
    \Pr[\eD(\hyb_5) = 1|\neg \mathsf{check}\text{-}\mathsf{fail}] -
    \Pr[\eD(\hyb_6) = 1|\neg \mathsf{check}\text{-}\mathsf{fail}]
    \Big |  \ge 
    \frac{1}{\poly(\secp)}
\end{align*}
%
which is a contradiction, as desired.
\end{proof} 

\iffalse{
\dnote{$\eC^*$ obtains the state up until Step 2 as non-uniform advice, then runs the part of $A^*$ that sends commitments to $P_{i^*}$. Then stops.}

\dnote{$\eD^*$ on input a view and a pair of extracted values (in one case the first is real, second extracted; in the other case, the first is extracted, second real). It finishes the rest of the protocol, and aborts if the adv aborts or provides a non-accepting proof. Then it checks for compliance by using the opening of the nmcom obtained as non-uniform advice, and appends $\cfail$ if the check fails. Next, it removes the second value from the pair, and runs $\eD$ on the resulting view.}

\dnote{Note that when check doesn't fail, both values in the pair must be identical, so the only possible difference can be in the probability of attaching $\cfail$, and therefore $\eD^*$ contradicts extractability. Prove this formally by a careful analysis conditioned on $\cfail$ happening versus not happening.}
}\fi
%\end{proof}

%\iffalse{
%\item $\hyb_7:$ Let $i$ denote the smallest index in $\mathbb{H}$.
%Sample instance-advice distribution identically to $\hyb_6$, except generate $\piext$ in Step 3 on behalf of party $P_{i^*}$ for all $j \in [n] \setminus \{i^*\}$, by executing $\eC(0^\lambda;r_{i^*,j})$ with uniform randomness $s_{i^*,j}$.
%\begin{claim}
%$$\Big\{ \hyb_6 \Big\}_{\secp \in \mathbb{N}} \approx_c \Big\{ \hyb_7 \Big\}_{\secp \in \mathbb{N}}$$
%\end{claim}
%\begin{proof}
%The proof follows identically to that of \cref{clm:gw}.
%\end{proof}

%\item $\hyb_8:$ Let $i$ denote the smallest index in $\mathbb{H}$.
%Sample instance-advice distribution identically to $\hyb_7$, except extracting values committed by $A^*$ by executing $\piext.\mathsf{Ext}$ in Step 3 on behalf of party $P_{i^*}$ for all $j \in [n]$, instead of in Step 4.
%If extraction fails or the adversary aborts at some point, output $\bot$. If the check fails, append $\cfail$ to the view.
%\begin{claim}
%$$\Big\{ \hyb_7 \Big\}_{\secp \in \mathbb{N}} \approx_c \Big\{ \hyb_8 \Big\}_{\secp \in \mathbb{N}}$$
%\end{claim}
%\begin{proof}
%The proof follows identically to that of \cref{clm:hw}.
%\end{proof}
%\end{itemize}
%\dnote{Note that the output of $\{\hyb_8\}_{\secp \in \mathbb{N}}$ corresponds to the distribution $\simulator_\bot(A^*)$. This completes the proof of our lemma. This is not true at the moment, need to add how simulation occurs.}
%\end{proof}
%}\fi


This completes the proof of the lemma. 
\end{proof}
\item $\hyb_1:$ This hybrid is identical to $\hyb_0$, except:
\begin{itemize}
    \item Let $i$ denote the smallest index in $\mathbb{H}$. 
    %Let $\rho'_\secp$ denote the intermediate state of $A^*_\secp$ at the end of Step 1 when the initial state of $A^*$ at the beginning of the protocol is $\rho_\secp$. 
    Let $A.\mathsf{ECom}^*_\secp$ be the portion of $A^*_\secp$ that produces $\mathsf{ECom}$ commitments in Step 3. Note that $A.\mathsf{ECom}^*_\secp$ also expects to obtain commitments from honest parties; these are generated identically to $\hyb_0$.
    This hybrid obtains 
    $$(\{\tau_{j,i}\}_{j \in \mathbb{S}},\{\tau_{j,i'}\}_{i' \in \mathbb{H} \setminus \{i\}, j \in \mathbb{S}},\state,\{c'_{j,i}\}_{j \in \mathbb{S}}) \gets \mathsf{Ecom}.\mathsf{Ext}(1^\secp,m,\mathbb{S},A.\mathsf{ECom}^*_\secp,\rho_\secp)$$
    If $A^*_\secp$ or $\mathsf{ECom}.\mathsf{Ext}$ aborts, then output $\bot$, otherwise continue executing $A^*_\secp$ with state updated to $\state$. Execute steps 1,2,4,5,6,7 identically to $\hyb_0$. 
    If an abort occurs, output $\bot$.
\end{itemize}

\begin{claim} \label{claim:ct-h1}
$$\Big\{ \hyb_0 \Big\}_{\secp \in \mathbb{N}}
\approx_c
\Big\{ \hyb_1 \Big\}_{\secp \in \mathbb{N}}$$
\end{claim}
\begin{proof}
%\dnote{Add\\}
Suppose Claim \ref{claim:ct-h1} is false. Then there exists a $\mathsf{QPT}$ distinguisher $\eD$ and a polynomial $\poly(.)$ such that for infinitely many $\lambda \in \bbN$,
%
\begin{align} \label{eq:mimdistinguisher}
    \Big |
    \Pr[\eD(\hyb_1) = 1] -
    \Pr[\eD(\hyb_0) = 1]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align}
%
We will use $A^*$ and $\eD$ to construct an committer $\eC^*$ and a {\em compliant} distinguisher $\eD^*$ which contradict the extractability property of the $\piext$ in Step 3 of \proref{fig:ct} as in Definition \ref{defn:qspec}. 
%Specifically, we will demonstrate that:
%A protocol violating Definition \ref{defn:qspec} implies the following:

%$\forall QPT \; \cE, \exists$ a quantum polynomial adversary $\eC^* = \{ \eC^*_\lambda, \rho_\lambda \}_{\lambda \in \bbN}$ representing a subset of $n$ committers, namely, $\{\eC_i\}_{i \in I}$ for some $I \subseteq [n]$
%and a {\em compliant} distinguisher $\eD^*$ such that for infinitely many polynomial-size sequences of inputs $\{\{m_{i,\secp}\}_{i \notin I}\}_{\secp \in \mathbb{N}}$,
%
%\begin{align*}
%    \Big | \Pr[\eD^*(\mathsf{VIEW/MESSAGES}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\rho_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^n))) = 1]  \\ -
%     \Pr[\eD^* (\cE(1^\secp,1^n,I,\eC^*_\secp,\rho_\secp)) = 1] \Big|     \ge \frac{1}{\poly(\secp)}
%\end{align*}

The adversary $\eC^*$ is as follows: 
\begin{enumerate}
    \item It participates as $|I| = |\bbS|$ committers, namely, $\{C_i\}_{i \in \bbS}$ in $\piext$ sessions with a challenger.
    %, where the challenger behaves either as an honest receiver or an extractor. 
    
    \item At the same time, $\eC^*$ takes the role of all honest parties $\bbH$ and participates in the coin-tossing protocol with adversary $A^*$.
    
    \item While doing so, it sends all messages as prescribed in \proref{fig:ct} with the following modification applied to Step 3: While behaving as a receiver on behalf of honest party $P_i$ to the $\piext$ session where $A^*$ is the committer, it forwards all messages from $A^*$ to the challenger and from the challenger to $A^*$. This produces a set of $|I|$ commitment transcripts from $\eC^*$ to the challenger in accordance with Definition \ref{defn:qspec}.
    %If $A^*$ aborts or its proofs do not verify, $\eC^*$ outputs $\bot$.
\end{enumerate}


$\eD^*$ is defined as follows:
%\dnote{Change $D^*$ to $\eD^*$.}
\begin{enumerate}
    \item Obtain input from the challenger either
    $\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\rho_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^n))$ or $\cE(1^\secp,1^n,I,\eC^*_\secp,\rho_\secp)$ - and then parse it as a tuple - $(\{\tau_i\}_{i \in I},\state,\{m_i\}_{i \in I})$ - indicating a set of transcripts, the state $\state$ of $A^*$, and the values (either real or extracted) committed by $\eC^*$.
    
    \item Execute the remaining steps  of \proref{fig:ct} with $A^*$'s state initialized to $\state$, to obtain a view.
    %It parses the state as $(\mathrm{T}, \mathsf{st}')$ where $\mathrm{T}$ represents the transcript of the coin-tossing protocol, and $\mathsf{st}'$ represents the state of the adversary.
    %\anote{Make the parsing better}
    
    \item If the adversary aborts at any point or the proofs in the transcript $\mathrm{T}$ do not verify, output $0$.
    %computes the following expression $\{ \tau^{zk}_i \}_{i \in I}$, where $\tau^{zk}$ represents the portion $\{\tau_i\}$ which is generated during Step 6 of \proref{fig:ct}
    %\begin{align}
    %    \bigwedge\limits_{i \in I} \zkV(\tau^{zk}_i)
    %\end{align}
    \item Otherwise, forward input together with the view of $A^*$ in the coin tossing protocol to $\eD$, and mirror the response of $\eD$.
\end{enumerate}

By the soundness of $\pibs$, $\eD^*$ is a compliant distinguisher according to Definition \ref{defn:qspec}.
%because of the soundness guarantee of \pibs. This follows because:
%\iffalse{
%\begin{align*}
    %\Pr[\eD^*(\{\tau_i\}_{i \in I}) = 0 | \{\tau_i\}_{i \in I} \text{ is not explainable}] = \\
    %\Pr[ \bigwedge\limits_{i \in I} \zkV(\tau^{zk}_i) = 0 | \{\tau_i\}_{i \in I} \text{ is not explainable}] \ge 1 - \negl(\secp)
%\end{align*}
%}\fi
%
%We now show that $\eD^*$ successfully contradicts the extractability property as stated in Definition \ref{defn:qspec}. To this end, note that:
Additionally,
%
\begin{align*}
    & \Pr[\eD^*(\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\rho_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^n))) = 1]
    =
    \Pr[\eD(\hyb_0) = 1], \text{ and }\\
    & \Pr[\eD^* (\cE(1^\secp,1^n,I,\eC^*_\secp,\rho_\secp)) = 1]
    =
    \Pr[\eD(\hyb_1) = 1]
\end{align*}
%
which implies that for infinitely many $\secp \in \bbN$,
\begin{align*}
    &\Big | \Pr[\eD^*(\mathsf{VIEW}^{\mathsf{msg}}_{\eC^*_\secp}(\dist{\eR,\eC^*_\secp(\rho_\secp),\{\eC_i(m_{i,\secp})\}_{i \notin I}}(1^\secp,1^n))) = 1] -
     \Pr[\eD^* (\cE(1^\secp,1^n,I,\eC^*_\secp,\rho_\secp)) = 1] \Big| 
    \\ &=
     \Big |
    \Pr[\eD(\hyb_1) = 1] -
    \Pr[\eD(\hyb_0) = 1]
    \Big | \ge 
    \frac{1}{\poly(\secp)}
\end{align*}
%
which is a contradiction, as desired.
\end{proof} 
}\fi

==> explainable-def.tex <==
\subsubsection{Explainable Verifiers}

Roughly speaking, explainable verifiers are verifiers whose messages are (almost) always in the support of the honest verifier's messages, regardless of how the prover's messages are generated. We also allow such verifiers to abort at any stage.

\begin{definition}[Explainable transcript]
Let $\prot{\zkP}{\zkV}$ be a protocol, $\zkmP$ be an arbitrary prover, and $\zkmV$ an arbitrary verifier. We say that a transcript $T$ of an execution $\prot{\zkmP}{\zkmV}(\ins)$ is explainable if there exists honest verifier coins $r$ such that $T$ is consistent with the transcript of an execution $\prot{\zkmP}{\zkV_r}$ until the point in $T$ that $\zkmV$ aborts. (Here $\zkV_r$ is the honest verifier using coins $r$).
\end{definition}

\omer{
\begin{definition}[Explainable transcript]
Let $\prot{\zkP}{\zkV}$ be a protocol. We say that a transcript $T$ is explainable if there exists an arbitrary prover $\zkmP$ and  honest verifier coins $r$ such that $T$ is consistent with the transcript of an execution $\prot{\zkmP}{\zkV_r}$. (Here $\zkV_r$ is the honest verifier using coins $r$). If $T$ contains a verifier abort message, the transcripts need to be consistent until that point.
\end{definition}
}\nir{leave as is}

% \begin{itemize}
% \item
% $\view_{\zkmV}\prot{\zkmP}{\zkmV}(\ins)$, the actual output of $\zkmV$, if all messages sent by $\zkmV$ during the execution are in the support of the honest $\zkV$; namely, there exists a random tape for the honest verifier, which explains these messages.  
% \item
% $\bot$ otherwise.
% \end{itemize}
%
\begin{definition}[Explainable verifier]\label{def:sm}
Let $\prot{\zkP}{\zkV}$ be a protocol. A (possibly probabilistic) verifier $\zkmV = \set{\zkmV_\secp}_\secp$ is explainable if there exists a negligible $\mu(\secp)$ such that for any prover $\zkmP$, $\secp\in\Nat$, and $\ins\in\zo^\secp$,
$$
\Pr_{\zkmV_\secp}\[T \text{ is explainable} \pST T\gets \prot{\zkmP}{\zkmV_\secp}(\ins)\] \geq 1-\mu(\secp)\enspace.
$$
\end{definition}


\nir{compare to semi-malicious -- key difference is that semi malicious simulator obtains adversary's random tape but explainable simulator does not. 
}

In the two-message setting, We will also consider a simpler notion of {\em always explainable verifiers}, which are deterministic verifiers that always output a message in the support of the honest verifier.

\begin{definition}[Always-explainable verifier]\label{def:ae}
A deterministic verifier $\zkmV = \set{\zkmV_\secp}_\secp$ is always explainable if for any prover $\zkmP$, $\secp\in\Nat$,  $\ins\in\zo^\secp$, and $T = \prot{\zkmP}{\zkmV_\secp}(\ins)$, $T$ is explainable and is not $\bot$.
\end{definition}


==> extra.tex <==
\iffalse{
\subsection{Random Self-Reducible Public-Key Encryption}\label{sec:RSR}

Intuitively speaking, a {\em random self reducible} (RSR) encryption scheme admits the classic notion of random self-reduction \cite{BlumM84} --- it is possible to rerandomize an arbitrary ciphertext into a random ciphertexts of the same message under the same public key. More generally, given access to an average-case distinguisher, it is possible to decrypt in the worst case. 
%We shall further require that the scheme is quasipolynomially secure.

\paragraph{Syntax.} 
An RSR encryption scheme $\rsre$ consists of $\PPT$ algorithms $(\rsreG,$ $\rsreE,$ $\rsreD,$ $\rsretD)$. 
 The first three algorithms have the standard syntax of a public-key (bit) encryption scheme. 

The fourth algorithm $\rsretD^{\rsremD}(\rsreCT,\rsrePK,1^{1/\varepsilon})$ is an oracle-aided alternative decryption algorithm, which given as input a ciphertext $\rsreCT$, public key $\rsrePK$ and (distinguishing) parameter $1^{1/\varepsilon}$, and a oracle access to a distinguisher $\rsremD$, outputs a plaintext bit $b$.  
\begin{definition}\label{def:rsr}
A public-key encryption scheme $(\rsreG,$ $\rsreE,$ $\rsreD,$ $\rsretD)$ is random self-reducible if it satisfies  
\begin{enumerate}
\item
{\bf Correctness:} for any $b\in\zo,\secp\in\Nat$,
$$
\Pr\[\rsreD_{\rsreSK}(\rsreCT)=b\pST \begin{array}{c}(\rsreSK,\rsrePK)\gets \rsreG(1^\secp)\\\rsreCT\gets \rsreE_{\rsrePK}(b)\end{array}\]=1
$$

\item
{\bf Indistinguishability:} For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_{\secp\in\Nat}$, there exists a negligible $\mu$ such that for any security parameter $\secp\in \Nat$,
\begin{align*}
\rsrePK,\rsreE_{\rsrePK}(0) \approx_{\zkmD_\secp,\mu} \rsrePK,\rsreE_{\rsrePK}(1)
\enspace,
\end{align*}
where $\rsreE_{\rsrePK}(b)$ is the distribution of encryptions of $b$ with random public key $\rsrePK\gets \rsreG(1^\secp)$.
\item
{\bf Random self-reduction:} for any public key $\rsrePK \in \rsreG(1^\secp)$ it holds that for any (possibly probabilistic) distinguisher $\rsremD$ and $\varepsilon$, 
\begin{itemize}
\item
if 
$$\abs{\EE \big(\rsremD(\rsreE_\rsrePK(0)) \big) - \EE \big(\rsremD(\rsreE_\rsrePK(1))\big)}\geq \varepsilon\enspace,$$
\item
then for any $b\in \zo$ and $\rsreCT \in \rsreE_\rsrePK(b)$,  
$$\Pr\[\rsretD^\rsremD(\rsreCT,\rsrePK,1^{1/\varepsilon})=b\]=1-2^{-\secp}\enspace,$$
where the probability is over the coins of $\rsretD$ and $\rsremD$.
\end{itemize}
\end{enumerate}
\end{definition}

\begin{remark}[Self reducibility against unbounded distinguishers]
In the above definitions of random self-reduction, the distinguisher $\zkmD$ is allowed to be unbounded. This is not essential in our constructions, but does make our proof cleaner, and is satisfied by all considered instantiations.
\end{remark}

\paragraph{Relaxed RSR.} We may consider a relaxed version of RSR encryption, where ciphertexts $\rsreCT \in \rsreE_{\rsrePK}(b)$ can be reduced to ciphertexts relative to a different encryption algorithm $\rsretE$. Such a relaxation is simpler to construct for instance under LWE.

Formally, there exists an additional $\PPT$ algorithm $\rsretE$, that satisfies:
\begin{enumerate}\item
{\bf Correctness:} similarly to $\rsreE$.
\item
{\bf Relaxed random self-reduction:} for any public key $\rsrePK \in \rsreG(1^\secp)$ it holds that for any (possibly probabilistic) distinguisher $\rsremD$ and $\varepsilon$, 
\begin{itemize}
\item
if 
$$\abs{\EE \rsremD(\rsretE_\rsrePK(0))-\EE \rsremD(\rsretE_\rsrePK(1))}\geq \varepsilon\enspace,$$
\item
then for any $b\in \zo$ and $\rsreCT \in \rsreE_\rsrePK(b)$,  
$$\Pr\[\rsretD^\rsremD(\rsreCT,\rsrePK,1^{1/\varepsilon})=b\]=1-2^{-\secp}\enspace,$$
where the probability is over the coins of $\rsretD$.
\end{itemize}
\end{enumerate}
We do not explicitly define (nor use) semantic security for the alternative encryption algorithm (although it actually follows from the semantic security of the original encryption together with relaxed RSR).

\paragraph{Instantiations.} There are various public-key encryption schemes \cite{GoldwasserM84,Elgamal85,Paillier99} based on standard algebraic assumptions, that are known to be perfectly {\em rerandomizable} and are hence random self reducible. Assuming quasipolynomial hardness of the underlying problems they are also quasipolynomially secure.

Statistically rerandomizable schemes are also known based on LWE \cite{Regev09}. However, in such schemes rerandomization is guaranteed for a random public key, whereas as we require that it holds for an arbitrary public key in the support of the generation algorithm. LWE does give relaxed RSR schemes using the standard noise flooding technique \cite{Gen09} (see \appref{sec:RRSR_LWE}). \nir{complete construction in appendix for completeness}


\subsection{Witness Encryption}

We recall the definition of witness encryption (WE).

\begin{definition}
A witness encryption scheme $(\weE, \weD)$ for an $\NP$ language $\lang$ satisfies  
\begin{enumerate}
\item
{\bf Correctness:} for any $(\ins,\wit)\in\RL$, and message $m\in\zo^*$,
$$
\weD_\wit(\weE_\ins(m))) = m \enspace.$$
\item
{\bf Indistinguishability:} For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_{\secp\in\Nat}$, there exists a negligible $\mu$ such that for any security parameter $\secp\in \Nat$, any $\ins \in \zo^\secp\setminus \lang$, and two equal-length messages $m_0,m_1$,
\begin{align*}
\weE_{\ins}(m_0) \approx_{\zkmD_\secp,\mu} \weE_{\ins}(m_1)
\enspace,
\end{align*}
where $\weE_{\ins}(m_b)$ is the distribution of encryptions of $m_b$ under $\ins$.
\end{enumerate}
\end{definition}

\paragraph{Instantiations.} Starting from the work of Garg, Gentry, Sahai, and Waters \cite{GargGSW13}, there have been several constructions of WE schemes for any language in $\NP$. State of the art schemes for $\NP$ (which haven't been broken) include constructions based on indistinguishability obfuscation \cite{GargGH0SW16} or the GGH15 multi-linear maps \cite{ChenVW18}. Witness encryption is also known for any language that has a {\em hash proof system} \cite{CramerS02}.


\subsection{Conditional Disclosure of Secrets}

Conditional disclosure of secrets for an $\NP$ language $\lang$ \cite{AielloIR01,BitanskyP12,Ananth017} can be viewed as a two-message analog of witness encryption. That is, the sender holds an instance $\ins$ and message $m$ and the receiver holds $\ins$ and a corresponding witness $\wit$. If the witness is valid, then the receiver obtains $m$, whereas if $\ins\notin\lang$, $m$ remains hidden. We further require that the protocol hides the witness $\wit$ from the sender. 

\begin{definition}
A conditional disclosure of secrets scheme $(\cdsR,\cdsS,\cdsD)$ for a language $\lang\in\NP$ satisfies:
\begin{enumerate}
    
\item
{\bf Correctness:} for any $(\ins,\wit)\in\RL$, and message $m\in\zo^*$,
$$
\Pr\[\cdsD_\cdsK(\cdsSCT) = m \pST \begin{array}{cc}
     (\cdsRCT,\cdsK) \gets \cdsR(\ins,\wit)  \\
     \cdsSCT\gets \cdsS(\ins,m,\cdsRCT)
\end{array}\]=1
\enspace.$$
\item
{\bf Message indistinguishability:} For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_{\secp\in\Nat}$, there exists a negligible $\mu$ such that for any security parameter $\secp\in \Nat$, any $\ins \in \zo^\secp\setminus \lang$, $\cdsRCT^*$, and two equal-length messages $m_0,m_1$,
\begin{align*}
\cdsS(\ins,m_0,\cdsRCT^*) \approx_{\zkmD_\secp,\mu} \cdsS(\ins,m_1,\cdsRCT^*)
\enspace.
\end{align*}

\item
{\bf Receiver simulation:} There exists a simulator $\cdsSim$, such that for any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_{\secp\in\Nat}$, there exists a negligible $\mu$ such that for any security parameter $\secp\in \Nat$, any $\ins \in \lang$, and $\wit\in\RL(\ins)$,
\begin{align*}
\cdsRCT \approx_{\zkmD_\secp,\mu} \cdsSim(\ins)
\enspace,
\end{align*}
where $\cdsRCT \gets \cdsR(\ins,\wit)$.
\end{enumerate}


\end{definition}

\paragraph{Instantiations.} CDS schemes can be instantiated assuming any two-message oblivious transfer protocol where the receiver message is computationally hidden from any semi-honest sender, and with (unbounded) simulation security against malicious receivers. Such oblivious transfer schemes are known based on DDH~\cite{NP01}, Quadratic (or $N^{th}$) Residuosity~\cite{HK12}, and LWE~\cite{BrakerskiD18}.
}\fi


\iffalse{
We rely on the standard notions of Turing machines and Boolean circuits.
\begin{itemize}
\item
We say that a Turing machine is $\PPT$ if it is probabilistic and runs in polynomial time.
\item
For a \PPT algorithm $M$, we denote by $M(x;r)$ the output of $M$ on input $x$ and random coins $r$. For such an algorithm, and any input $x$, we may write $m\in M(x)$ to denote the fact that $m$ is in the support of $M(x;\cdot)$. 
\item
A polynomial-size circuit family $\mathcal{C}$ is a sequence of circuits $\mathcal{C}=\set{C_\secp}_{\secp\in\Nat}$, such that each circuit $C_\secp$ is of polynomial size $\secp^{O(1)}$ and has $\secp^{O(1)}$ input and output bits. We also consider probabilistic circuits that may toss random coins.
\item
We follow the standard habit of modeling any efficient adversary as a family of polynomial-size circuits. For an adversary $\A$ corresponding to a family of polynomial-size circuits $\set{\A_\secp}_{\secp\in\Nat}$, we sometimes omit the subscript $\secp$, when it is clear from the context. 
%When we write $\A(x)$ for a circuit $\A$, without specifying the length of $x$, we assume that $\A$ only reads an $\ell$-bit prefix of $x$, where $\ell$ is the input-size of the circuit $\adversary$.

\item
We also consider quasipolynomial-size adversaries, which are defined analogously to polynomial-size adversaries, but are of size $2^{(\log\secp)^{O(1)}}$ instead of $\secp^{O(1)}$. By default we define the security of primitives against polynomial-size adversaries. Security against quasipolynomial-size adversaries is always defined analogously.

\item
A function $f:\Nat \rightarrow \mathbb{R}$ is negligible if $f(\secp)=\secp^{-\omega(1)}$ and is noticeable if $f(\secp)=\secp^{-O(1)}$.
%if for all constants $c > 0$, there exists $N \in \Nat$ such that for all $n > N$, $f(n) < n^{-c}$.

\item
For random variables $X$ and $Y$, distinguisher $\zkmD$, and $0<\mu<1$, we write $X \approx_{\zkmD,\mu} Y$ if
\begin{align*}
\abs{
\Pr[\zkmD(X)=1] - \Pr[\zkmD(Y)=1]
} \leq \mu.
\end{align*}

% \item
% Two ensembles of random variables $\mathcal{X}=\{X_{\secp}\}_{\secp\in \Nat}$ and $\mathcal{Y}=\{Y_{\secp}\}_{\secp\in \Nat}$ are said to be computationally indistinguishable, denoted by $\mathcal{X}\approx_c \mathcal{Y}$, if for all polynomial-size distinguishers $\zkmD=\set{\zkmD_\secp}_{\secp\in\Nat}$, there exists a negligible function $\mu$ such that for all $\secp$,
% \begin{align*}
% X_\secp \approx_{\zkmD,\mu(\secp)} Y_\secp\enspace.
% \end{align*}
\end{itemize}
}\fi


%The correctness considered there is two-sided --- they prove perfect correctness for inputs $x$ such that $f(x)=u$ and almost perfect correctness for inputs $x$ such that $f(x)\neq u$. We will only rely on the first of the two (and perfect correctness will play a role).

%In addition, they do not state explicitly the fact that simulated circuits are rejecting. However, this is satisfied by their construction, and follows readily from their simulator definition and correctness analysis (see e.g., \cite[Claim 4.11]{WichsZ17}). 

==> intro_old.tex <==
\section{Introduction}

{Zero-knowledge protocols}  are spectacular. They allow to prove any $\NP$ statement without revealing anything but the statement's validity. That is, whatever a malicious verifier learns from the protocol can be efficiently simulated from the statement alone, without ever interacting with the prover. Since their invention \cite{GoldwasserMR89} and construction for all of $\NP$ \cite{GoldreichMW91}, zero-knowledge protocols have had a profound impact on modern cryptography.

A central question in the study of zero knowledge is that of {\em round complexity}. Zero-knowledge arguments with a negligible soundness error can be achieved in four messages \cite{FeigeS90}, under the minimal assumption of one-way functions \cite{BellareJY97}.\footnote{Recall that a protocol is an argument if it is only computationally sound, and a proof if it is statistically sound.}  In terms of lower bounds, zero-knowledge arguments for languages outside $\BPP$, and without any trusted setup, require at least three messages \cite{GoldreichO94}.

Zero knowledge protocols with an optimal number of messages (and a negligible soundness error) have been pursued over the last three decades and have proven difficult to construct. Three-message zero-knowledge arguments were only constructed under {\em auxiliary-input knowledge assumptions}, which are considered implausible \cite{HadaT98,BellareP04a, BitanskyCPR14,BoyleP15,BitanskyCCGLRT17}, and more recently, under a new, non-standard, assumption on the multi-collision resistance of keyless hash functions \cite{BitanskyKP18}. Three-message protocols based on standard cryptographic assumptions remain out of reach.

\paragraph{Relaxing zero knowledge.} Given the current state of affairs, it is natural to consider relaxations of the zero-knowledge privacy guarantee. Three main relaxations considered in the literature are:

% \medskip
% \noindent \underline{{\em Witness indistinguishability} \cite{FeigeS90}}: Ensures that the verifier cannot distinguish between proofs that are generated using different witnesses. While meaningful and often useful as a building block to obtain zero knowledge, witness indistinguishability is still quite limited. In particular, in the rather common scenario where statements have a unique witness, it becomes meaningless.

% \medskip
% \noindent \underline{{\em Witness hiding} \cite{FeigeS90}}:
% Ensures that the proof does not leak an entire witness. That is, a malicious verifier cannot learn a witness, unless such a witness can be efficiently computed from the statement alone. In particular, the witness hiding requirement is also  meaningful in the unique witness case.

% \medskip
% \noindent \underline{{\em Weak zero-knowledge} \cite{DworkNRS03}}: Relaxes the zero-knowledge definition by switching quantifiers. Whereas zero knowledge requires that for every verifier there exists a {\em simulator} that generates an interaction that is indistinguishable from a real one for every {\em distinguisher}, weak zero-knowledge requires that for every verifier and {\em distinguisher}, there exists a {\em simulator} that fools this specific distinguisher. We will also allow the simulator to depend on the desired distinguishing gap.\footnote{There are several variants  of this definition strengthening/weakening different aspects \cite{DworkNRS03,ChungLP15}. For the sake of this introduction the reader may stick to the (informal) definition above. We elaborate in the technical overview below.} Weak zero-knowledge hides any (even inefficient) predicate of the statement and (prover) witness that cannot be computed from the statement alone, and implies both witness hiding and witness indistinguishability.

\begin{itemize}%[leftmargin=0.5cm]
\item {\bf Witness indistinguishability \cite{FeigeS90}:} Ensures that a malicious verifier cannot distinguish between proofs that are generated using different witnesses. While witness indistinguishability is natural and often useful as a building block in applications, it is still quite limited. For example, in the rather common scenario where statements have a unique witness, witness indistinguishability becomes meaningless.

\item{\bf Witness hiding \cite{FeigeS90}:} 
Ensures that a malicious verifier cannot learn an entire witness from the proof; that is, unless such a witness can be efficiently computed from the statement alone. In contrast to witness indistinguishability, the witness hiding requirement is also  meaningful in the unique witness case.

\item{\bf Weak zero-knowledge  \cite{DworkNRS03}:} Relaxes zero-knowledge by switching the order of quantifiers. Full-fledged zero-knowledge requires that for every verifier there exists a \underline{simulator} that generates a view, indistinguishable from the verifier's view in a real interaction, for every \underline{distinguisher}. 
In contrast, weak zero-knowledge requires that for every verifier and \underline{distinguisher}, there exists a \underline{simulator} that fools this specific distinguisher. We also allow the simulator to depend on the desired distinguishing gap.\footnote{There are several variants  of this definition strengthening/weakening different aspects \cite{DworkNRS03,ChungLP15}.}

Weak zero-knowledge hides any predicate of the statement and witness (used by the prover) that cannot be computed from the statement alone. It implies both witness hiding and witness indistinguishability.
%, as well as the notion of {\em strong witness-indistinguishability} \cite{Goldreich2001}, guaranteeing that proofs for computationally indistinguishable statements are themselves indistinguishable.
\end{itemize}
%
The above relaxations are not subject to the same lower bounds as full-fledged zero-knowledge. In fact, the only known unconditional lower bound rules out weak zero-knowledge in one message \cite{GoldreichO94}.

As for constructions, witness indistinguishability has indeed been obtained, under standard assumptions, in three \cite{GoldreichMW91,FeigeS90}, two \cite{DworkN07,BadrinarayananG17,JKKR17}, and eventually even one message \cite{BarakOV07,GrothOS12}. In contrast, weak zero-knowledge and witness hiding have proven to be just as challenging to construct as full-fledged zero-knowledge. So far, constructions with less than four messages are known only based on non-standard assumptions, which by now are considered implausible \cite{BitanskyP12,BrzuskaM14a,BellareST16}, for restricted classes of adversarial verifiers \cite{BitanskyCPR14,JKKR17}, or for restricted classes of languages \cite{FeigeS90,Pass03}. (See the related work section for more details). 

\paragraph{The black-box barrier.} The difficulty in obtaining round-optimal zero knowledge and its relaxations stems from a fundamental barrier known as the {\em black-box barrier} --- three-message zero-knowledge is impossible as long as the simulator is oblivious of the verifier's code, treating it as a black box \cite{GoldreichK96}. Similar barriers hold for both weak zero-knowledge and witness hiding \cite{HaitnerRS09}. 

Whereas classical zero-knowledge protocols all have black-box simulators, starting from the breakthrough work of Barak \cite{Barak01}, non-black-box techniques that exploit the verifier's code have been introduced (c.f., \cite{DengGS09,ChungLP13,Goyal13, BitanskyP15b, BitanskyBKPV16,ChungPS16}). However, existing techniques seem to require at least four messages (except for \cite{BitanskyKP18}, based on a non-standard assumption). 

\medskip\noindent
In conclusion, as in the case of zero knowledge, weak-zero-knowledge and witness-hiding protocols in three-message or less, based on standard cryptographic assumptions, remain out of reach.

\subsection{Results}

We devise a new non-black-box technique and apply it to obtain, under standard assumptions, weak zero-knowledge and  witness hiding beyond the black-box barrier. 

\medskip\noindent
Our main result is a two-message weak zero-knowledge argument for $\NP$.

\begin{theorem}[informal]\label{intro_thm:2wzk}
There exists a two-message weak zero-knowledge argument for $\NP$ assuming: subexponentially-secure one-way functions and quasi-polynomially-secure fully-homomorphic encryption, random-self-reducible encryption, two-message witness-indistinguishable arguments and oblivious transfer, non-interactive commitments, and compute-and-compare obfuscation.
\end{theorem}

All of the above primitives (but subexponentially-secure one-way functions) are known under quasipolynomial hardness of LWE, with the exception of fully-homomorphic encryption that also requires a circular security  assumption \cite{Gentry09,BrakerskiV14,BadrinarayananG17,GoyalHKW17,GoyalKW17,JKKR17,WichsZ17,BrakerskiD18}. 
We can also replace compute-and-compare obfuscation with fully-homomorphic encryption scheme with some additional natural properties that are satisfied by known constructions (see the technical overview for more details).

% We note that previously no positive (nor negative) results were known regarding neither weak zero-knowledge or witness hiding in one round. 
It is interesting to note that the result gives an example of a {\em natural} weak-zero-knowledge protocol that is provably not zero knowledge. Previously, a contrived separation was known assuming exponentially-hard injective one-way functions \cite{ChungLP15}.

\medskip\noindent
Our second result is a three-message protocol that is based only on polynomial hardness assumptions. 

\begin{theorem}[informal]\label{intro_thm:3wzk}
Assuming polynomial hardness of the primitives in \thmref{intro_thm:2wzk}, as well as dense commitments, there exists a three-message weak zero-knowledge argument for $\NP$.
\end{theorem}
%
The polynomially-hard version of the required primitives (including dense commitments) can be based on (polynomially-hard) fully-homomorphic encryption, LWE, and either Factoring or standard Bilinear-Group assumptions. 

\medskip\noindent
Our third result, also from polynomial hardness assumptions, is a two-message witness-hiding protocol for any language $\lang\in \NP$ that has a {\em witness encryption scheme} \cite{GargGSW13}.

\begin{theorem}[informal]\label{intro_thm:2wh}
There exists a two-message witness-hiding argument for any language $\lang \in \NP$ under the same (polynomial) assumptions as in \thmref{intro_thm:3wzk} and witness encryption for $\lang$.
\end{theorem}

For the time being, witness encryption for all of $\NP$ is only known based on indistinguishability obfuscation, or based on non-standard assumptions on multilinear maps \cite{GargGH0SW16, ChenVW18}. Witness encryption for several non-trivial languages follows from results on hash proofs systems \cite{CramerS02}.

The protocol we obtain is {\em publicly verifiable}, meaning that the proof can be verified given the transcript alone, without secret verifier randomness. We observe that the \cite{GoldreichO94} lower bound for two-message zero-knowledge extends also to two-message publicly-verifiable weak zero-knowledge, and thus we cannot expect to get a similar result for weak zero-knowledge.

% \medskip\noindent
% An interesting aspect of all of our simulators (or reductions) is that they are still {\em semi black-box} --- the next message function of the verifier is used as a black-box. Specifically, our simulators only require the code that produces the verifier's final output and that of the distinguisher (in the case of weak zero-knowledge). 
% \omer{I would remove this remark. Not that clear and not that interesting.}

\paragraph{From explainable to malicious security.} The main component in all of the above results is a weak-zero-knowledge argument for $\NP$ against a new class of verifiers that we call {\em explainable}. Such verifiers may not follow the honest verifier strategy, but they do choose their messages from the support of the honest verifier message distribution; namely, there exist honest verifier coins that explain their behavior. The notion resembles that of {\em semi-malicious} and {\em defensible} adversaries \cite{HaitnerIKLP11,BoyleG0KS13}, but differs in the fact that the verifier does not explicitly choose a random tape for the honest verifier (and it may not be possible to efficiently extract such a tape from the verifier).

\begin{theorem}[informal]\label{intro_thm:2wzksm}
Under the same assumptions as in Theorem \ref{intro_thm:2wzk} (respectively, \ref{intro_thm:3wzk}), there exists a two-message (respectively, three-message) weak zero-knowledge argument for $\NP$ against explainable verifiers.
\end{theorem}

We then give general compilers to boost explainable security to malicious security. These compilers may be of independent interest. For instance, they imply that to obtain full-fledged zero knowledge in three messages, it suffices to consider explainable verifiers.


\subsection{Technical Overview}

We now give an overview of our techniques. We focus on two-message protocols against explainable verifiers, which is the technical core behind our results. We also explain how to avoid super-polynomial hardness assumptions, at the account of adding one message to this protocol. We then describe the main ideas behind our compilers to malicious security. 

\paragraph{Warm up: a witness-hiding protocol.} Toward constructing a two-message weak-zero-knowledge protocol against explainable verifiers, let us first consider the easier goal of witness hiding. 
Recall that a protocol is witness hiding if there exists a reduction that given as input an $\NP$ statement $\ins$, and the code of a {\em  witness-finding verifier}, outputs a witness. By a witness-finding verifier, we mean a verifier that given a proof that $\ins$ is true, finds a witness for $\ins$ with noticeable probability.

Our protocol follows a classic paradigm by Feige, Lapidot, and Shamir \cite{FeigeLS99}. The first verifier message fixes a so-called {\em trapdoor statement} $\tau$. 
In parallel, the prover and verifier execute a two-message witness-indistinguishable argument that either the statement $\ins$ or the trapdoor statement $\tau$ hold. (Throughout the rest of the introduction we ignore the first message of the witness-indistinguishable argument.)

The trapdoor statement $\tau$ is meant to have two properties:
\begin{itemize}
\item
To a malicious prover, trying to convince the verifier of a false statement $\ins$, $\tau$ should be computationally indistinguishable from a false statement. Thus, by the soundness of the witness-indistinguishable argument, the prover should fail.

\item
A reduction {\em that has the code of an explainable witness-finding verifier} should be able to obtain a witness $\rho$ for the trapdoor statement $\tau$. Once such a witness is found, the reduction can use it to generate the witness-indistinguishable argument. By witness indistinguishability, the reduction's proof is indistinguishable from the honestly generated proof and, therefore, the verifier will output a valid witness $\wit$ for the statement $\ins$ with noticeable probability.   
\end{itemize}
%
The main challenge in realizing the above paradigm is to extract the trapdoor witness $\rho$ from the verifier's code. The basic idea behind our non-black-box technique, and what enables such extraction, is what we call the {\em homomorphic trapdoor paradigm}.

In our protocol, on top of the trapdoor statement $\tau$, the verifier will send an encryption $\fheCT$ of the witness $\rho$ attesting that $\tau$ holds, using a fully-homomorphic encryption scheme. On one hand, by the security of the encryption scheme, this does not compromise soundness. On the other hand, a reduction that has the code of the witness-finding verifier can obtain a witness $\wit$ for $\ins$ {\em under the encryption}. To do so, the reduction homomorphically invokes the strategy described before --- under the encryption $\fheCT$, it uses $\rho$ to compute the witness-indistinguishable argument, and obtain the witness $\wit$ from the verifier.

The above step does not find a witness $\wit$ in the clear (nor does it extract the trapdoor $\rho$). We observe, however, that an encryption of a witness $\wit$ is already a non-trivial piece of information that could only be obtained when $\ins$ is a true statement; in fact, we can use it as another trapdoor witness. Concretely, we extend our protocol to include yet another, so-called homomorphic, trapdoor statement $\tau_h$ where a witness $\rho_h$ for $\tau_h$ could be any encryption of a witness $\wit$ for $\ins$. That is, $\tau_h$ is true if and only if $\ins$ is true, and a witness $\rho_h$ for $\tau_h$ is an encryption of a witness $\wit$ for $\ins$. 

In the extended protocol, the prover gives a witness-indistinguishable argument that either the statement $\ins$, the trapdoor statement $\tau$, or the homomorphic trapdoor statement $\tau_h$ hold. The reduction first uses the encrypted trapdoor $\rho$ homomorphically to obtain a trapdoor $\rho_h$ (in the clear), and then uses $\rho_h$ to generate the witness-indistinguishable argument. By witness indistinguishability, the verifier will output a witness $\wit$, this time in the clear. Note that we crucially rely on the fact that a fully homomorphic encryption scheme satisfies  {\em compactness} in the sense that the size of the encrypted witness (and hence the trapdoor $\tau_h$) is fixed and independent of the size of the homomorphic computation performed to obtain this encryption. Indeed, this computation grows with the size of the malicious verifier, which is not apriori bounded.

One difficulty in realizing the above strategy is to prove the homomorphic trapdoor statement $\tau_h$; that is, to prove that there exists an encryption $\rho_h$ of a valid witness $\wit$ for $\ins$, when the reduction lacks the homomorphic decryption key. We discuss how to resolve this difficulty below when describing the more general weak-zero-knowledge protocol.

\paragraph{Toward weak zero-knowledge.} Recall that in weak zero-knowledge, we require that there exists a simulator that given the code of a verifier and a distinguisher $\zkmD$, simulates the verifier's output so that it fools $\zkmD$. That is, $\zkmD$ cannot $\varepsilon$-distinguish between the simulated output and the verifier's output in a real interaction with the prover, for any accuracy parameter $\varepsilon$, where the simulator is allowed to run in time polynomial in ${1/\varepsilon}$.

In this setting, the verifier's output is arbitrary and may not include a witness. Thus, we cannot employ the same strategy as before. Nevertheless, our protocol still builds on the homomorphic trapdoor paradigm, but with additional ideas. In a nutshell, instead of extracting a witness $\wit$ from the verifier under the encryption, we extract a different trapdoor witness from the distinguisher $\zkmD$, under the encryption. Then, as before, we use the encryption of this trapdoor as the homomorphic trapdoor.

\paragraph{Random self-reducible encryption.} To enable extraction from the distinguisher, we rely on a public-key encryption scheme that is {\em random self-reducible} \cite{BlumM84}. In such a scheme, any distinguisher $\zkmD$ that can tell encryptions of zero from encryptions of one with advantage $\varepsilon$, under some specific public key $\rsrePK$, can be used to decrypt arbitrary ciphertexts under the key $\rsrePK$, in time polynomial in $|\zkmD|/\varepsilon$. Such schemes are known based on various standard assumptions (see \secref{sec:RSR}).

\paragraph{The protocol.} We now describe the protocol, and then go on to analyze it.
\begin{itemize}
\item
The verifier's message, as before, includes a trapdoor statement $\tau$ and a fully-homomorphic encryption $\fheCT = \fheE_{\fheK}(\rho)$ of the corresponding witness $\rho$. In addition, it includes another trapdoor statement $\tau'$, and a random self-reducible encryption $\rsreCT' = \rsreE_{\rsrePK}(\rho')$ of the corresponding witness $\rho'$. The trapdoor statements $\tau,\tau'$ are both indistinguishable from false statements. The statements $\tau,\tau'$ also fix a homomorphic trapdoor statement $\tau_h$, asserting  that ``there exists a fully-homomorphic encryption $\rho_h$ of a valid witness $\rho'$ for $\tau'$.'' That is, $\tau_h$ is true if and only if $\tau'$ is true, and any witness $\rho_h$ for $\tau_h$ is a fully-homomorphic encryption of a witness $\rho'$ for $\tau'$.

\item
The prover, as before, gives a witness-indistinguishable argument, but now, in addition, it also sends a random-self-reducible encryption of one $\rsreCT_{\zkP}=\rsreE_{\rsrePK}(1)$. The witness-indistinguishable argument attests that either one of the statements $\ins,\tau,\tau_h$ hold, or $\rsreCT_{\zkP}$ is an encryption of zero (and not one). Note that the trapdoor statement $\tau'$ is not directly involved in the witness-indistinguishable argument, but only defines the homomorphic trapdoor statement $\tau_h$.

\item
The verifier checks that the witness-indistinguishable argument is valid and that $\rsreCT_\zkP$ decrypts to one.
\end{itemize}
%
\paragraph{Soundness.} Relying on the security of both encryption schemes, we would like to argue that the verifier's encryptions of $\rho$ and $\rho'$ can be changed to encryptions of garbage. Then, the trapdoor statements $\tau$ and $\tau'$ can be changed to false statements, in which case the homomorphic trapdoor statement $\tau_h$ also becomes false. Also, $\rsreCT_\zkP$ must not be an encryption of zero or the verifier rejects. Soundness then follows from that of the witness-indistinguishable argument.

One subtlety in the above argument is that the verifier's decision depends on the secret key of the 
the random-self-reducible encryption, and thus changing the encryption of $\rho'$ to garbage may affect the bit underlying the prover's encryption $\zkPCT$ and accordingly also the verifier's decision bit. To get around this, we require that the prover exhibits that it ``knows'' the contents of the encryption $\zkPCT$ (and therefore does not maul the encryption of $\rho'$ ). In this case, we can argue that the verifier continues to accept, even if we change the encryption of $\rho'$. To facilitate such a proof of knowledge in two messages we resort to complexity leveraging, which is the cause of reliance on super-polynomial assumptions in our two-message protocol. In the three-message setting, we rely instead on extractable commitments based on polynomial hardness assumptions.


\def \p {\mathsf{p}}
\def \s {\mathsf{s}}
\paragraph{Weak zero-knowledge.} To argue weak zero-knowledge, we follow a similar approach to that taken in previous works that constructed weak zero-knowledge \cite{BitanskyP12,JKKR17}. \omer{weak zero-knowledge appears twice in the first sentence. fix?} The simulation strategy will have two modes: a {\em secret mode} and a {\em public mode}, with two corresponding distributions on proofs, $\Pi_{\s}$ and $\Pi_{\p}$. The secret distribution $\Pi_{\s}$ is always indistinguishable from the real distribution $\Pi$ generated by the honest prover, but sampling from this distribution requires a secret $\s$. The public distribution $\Pi_\p$ can be publicly sampled without knowing $\s$. While  $\Pi_\p$ is not indistinguishable from $\Pi$, to tell them apart, the distinguisher must ``know'' the secret $\s$. That is, given any distinguisher $\zkmD$ that $\varepsilon$-distinguishes $\Pi_\p$ from $\Pi$, it is possible to extract the secret $\s$ in time polynomial in $|\zkmD|/\varepsilon$.

This gives rise to a simple simulation strategy that treats separately two types of distinguishers: those that know the secret $\s$, and those that do not. Specifically, given the code of the distinguisher $\zkmD$ and the required simulation accuracy $\varepsilon$, first try to extract the secret $\s$ from $\zkmD$, and if successful, sample from $\Pi_\s$ to simulate the proof. Otherwise, deduce that $\zkmD$ cannot $\varepsilon$-distinguish $\Pi_\p$ from $\Pi$, and sample the proof from $\Pi_\p$. As before, the main challenge in realizing this strategy is to extract the secret $\s$ from $\zkmD$. Our solution again relies on the homomorphic trapdoor paradigm.

\smallskip\noindent
Going back to our protocol, let us define the corresponding secret and public distributions $\Pi_\s,\Pi_\p$: 
\begin{itemize}
\item
The secret distribution $\Pi_\s$ is associated with the homomorphic trapdoor $\tau_h$, and can be sampled using any witness $\rho_h$ for $\tau_h$. Like the real proof distribution $\Pi$, it consists of an encryption of one $\rsreCT_\zkP=\rsreE_{\rsrePK}(1)$. However, differently from the real proof distribution, the witness-indistinguishable argument is computed using the homomorphic trapdoor witness $\rho_h$.
\item
The public distribution $\Pi_\p$ consists of an encryption of zero $\rsreCT_\zkP=\rsreE_{\rsrePK}(0)$, and the witness-indistinguishable argument is computed using the randomness of the encryption $\rsreCT_\zkP$ as a witness.
\end{itemize}
We argue that $\Pi_\s$ and $\Pi_\p$ have the required properties. The fact that $\Pi_\s$ is indistinguishable from the real proof distribution $\Pi$ follows from witness indistinguishability. We now show that any distinguisher $\zkmD$ between $\Pi_\p$ and $\Pi$ can be used to extract a witness $\rho_h$ (namely, an encryption of a witness $\rho'$ for $\tau'$), which in turn, can be used for sampling from $\Pi_\s$. We do this in two steps:
\begin{enumerate}
\item
We show that given a distinguisher $\zkmD$ between $\Pi_\p$ and $\Pi$, {\em as well as the trapdoor $\rho$}, we can obtain a distinguisher $\zkmD'$ that can tell apart encryptions of one from encryptions of zero (with about the same advantage). By random self-reducibility, such a distinguisher $\zkmD'$ can be used to decrypt arbitrary ciphertexts under the random self-reducible scheme. In particular, such $\zkmD'$ can be used to decrypt the encryption $\rsreCT'$ of the trapdoor $\rho'$ (given in the first verifier message).

The distinguisher $\zkmD'$ is defined in the natural way: given a bit encryption, it samples on its own a witness-indistinguishable argument, using $\rho$ as the witness, and then applies $\zkmD$. By witness indistinguishability, the induced distribution $\Pi_0$, corresponding to encryptions of zero, is indistinguishable from the real proof distribution $\Pi$. Similarly, the distribution $\Pi_1$, corresponding to encryptions of one, is indistinguishable from the public distribution $\Pi_\p$. Accordingly, $\zkmD'$ has roughly the same advantage as $\zkmD$.

\item
In the second step, we extract the required trapdoor $\rho_h$ allowing us to sample from $\Pi_\s$. Analogously to the witness-hiding reduction we have already seen, this is done by homomorphically applying the first step --- under the encryption $\rsreCT$ sent by the verifier, we use $\rho$ to obtain the distinguisher $\zkmD'$ and decrypt $\rsreCT'$. This results in the required trapdoor $\rho_h$, a fully-homomorphic encryption of the trapdoor $\rho'$.
\end{enumerate}

\nir{Some sort of diagram could be helpful in understanding the relations between the trapdoors}

\paragraph{How to prove homomorphic trapdoor statements.} To conclude our sketch of the weak zero-knowledge analysis, we explain how to prove the homomorphic trapdoor statement $\tau_h$. As already mentioned, the difficulty in proving that there exists an encryption $\rho_h$ of a valid witness for $\tau'$ is that the simulator does not have the corresponding secret key. Next, we discuss two possible solutions.

The first approach (which we follow in the body of the paper) is based on obfuscation for {\em compute and compare programs}. A compute and compare program $\CC{f,u}$ is given by a function $f$  (represented as a circuit) and a target output string $u$ in its range; it accepts every input $x$ such that $f(x)=u$, and rejects all other inputs. A corresponding obfuscator compiles any such program into a program $\obfC$ with the same functionality. In terms of security, provided that the target $u$ has high entropy , the obfuscated program is computationally indistinguishable from a simulated program that rejects all inputs. Such obfuscators are defined and constructed under LWE in \cite{GoyalKW17,WichsZ17}.\footnote{The known construction have a one-sided negligible correctness error. This error will not obstruct our protocol and is ignored in this introduction.}

Using compute-and-compare obfuscation, we modify our protocol as follows. We no longer sample a trapdoor statement $\tau'$, but instead, set $\rho'$ to be a random string. The homomorphic trapdoor statement $\tau_h$ is still defined so that a witness $\rho_h$ is a fully-homomorphic encryption of $\rho'$. Specifically, $\tau_h$ is given by an obfuscation $\obfC$ of the program $\CC{\fheD_{\fheK},\rho'}$ that accepts fully-homomorphic ciphertexts that decrypt to $\rho'$. Accordingly, a ciphertext $\rho_h$ is a valid witness for $\tau_h$ if and only if $\obfC(\rho_h) = 1$. The obfuscation $\obfC$ will now be specified as part of the verifier's first message, which also includes as before the trapdoor statement $\tau$, a fully-homomorphic encryption of the trapdoor witness $\rho$, and a random self-reducible encryption of the random string $\rho'$.


The simulator can obtain a fully-homomorphic encryption of $\rho'$ and use it as a trapdoor witness $\rho_h$. Furthermore, as required for soundness, $\tau_h$ is indistinguishable from a false statement, since $\obfC$ is indistinguishable from a program that rejects all inputs.



%Another advantage of using compute-and-compare obfuscation, besides from simplicity, is that it gives rise to publicly-verifiable witness-hiding protocols. Specifically, assuming also witness encryption, we obtain a protocol where verification only involves verifying a witness-indistinguishable argument. 
\nir{where to mention public verification advantage?}

\paragraph{Another approach, without compute-and-compare obfuscation.} 
\omer{I think this part is important (and eventually should be detailed in the body). Dakshita, please suggest how to make this explanation more clear.}
We now describe an alternative approach for proving the trapdoor statement, which does not rely on compute-and-compare obfuscation, but requires the homomorphic encryption to satisfy additional properties.

Here, given the fully-homomorphic encryption $\rho_h$ of $\rho'$, the simulator homomorphically evaluates the $\NP$ witness verification procedure for the statement $\tau'$ and sends the encrypted output bit. It then proves that this bit encryption was indeed obtained by homomorphically evaluating the verification procedure for $\tau'$ using the encryption $\rho_h$ as a witness. The verifier checks the proof and in addition decrypts the output bit and checks that it is accepting.

There are some subtleties to take care of: a) to preserve witness indistinguishability, the homomorphic evaluation must be {\em function hiding} and b) to preserve soundness, the prover must convince the verifier that the homomorphic computation was performed over a valid ciphertext $\rho_h$. To this end, we require a {\em validation} operation mapping arbitrary (possibly invalid) ciphertexts into valid ones, while preserving the plaintext underlying valid ciphertexts. Both properties can be achieved in existing fully-homomorphic encryption constructions (without additional assumptions) \cite{Gen09,OstrovskyPP14,HubacekW15}. (Also, a similar malleability problem as described before also occurs here and is dealt with using a proof of knowledge.)

Another issue is that the simulator cannot tell whether the encryption $\rho_h$ it obtained is indeed an encryption of a valid trapdoor witness $\rho'$ or not (in which case, it should deduce that $\zkmD$ cannot tell $\Pi$ from $\Pi_\p$ and use $\Pi_\p$ to simulate).
To deal with this, we again use the distinguisher $\zkmD'$ to decrypt $\rsreCT'$, except that we do so in the clear. Since now we do not have the trapdoor witness $\rho$, we use $\rho_h$ instead. By witness indistinguishability, if we fail to decrypt $\rsreCT'$ and obtain the witness $\rho'$ in the clear, we can deduce that $\zkmD$ cannot tell $\Pi$ from $\Pi_\p$. 

\subsubsection{From Explainable to Malicious} 
Observe that in the protocols described above, it was crucial that the verifier behaves in an explainable fashion. In particular, the simulation strongly relies on the fact that the verifier's fully-homomorphic encryption $\fheCT$ is indeed an encryption of  trapdoor witness $\rho$ for the statement $\tau$. To deal with malicious adversaries, we design compilers that take protocols secure against explainable verifiers and turn them into protocols secure against malicious verifiers. We provide three different compilers for different settings. We now explain the main ideas behind each of these compilers.
 

\omer{Motivate the notion of explainability. See text in comment}
%Our complied verifier proves that it follows the honest strategy for some random coins. However, differently from the compilation from defensible security to full security \cite{HaitnerIKLP11,BoyleG0KS13}, when compiling an explainable verifier we do not not need to prove that the verifier knows these honest random coins, only that such coins exist. This fact is crucial for designing a compiler for protocols with two or three rounds.  


\paragraph{A two-message compiler based on super-polynomial assumptions.} 
%For simplicity of exposition, we describe our two-message compiler assuming the existence of a witness encryption scheme for $\NP$. Our actual compiler uses a two-message version of witness encryption known as conditional disclosure of secrets for $\NP$, which known under standard assumptions \cite{AielloIR01,BitanskyP12,Ananth017}. In a witness encryption scheme for an $\NP$ language $\lang$, it is possible to encrypt messages using statements $\ins$ as a public-key. Decryption can be done by anyone in possession of a corresponding witness $\wit$. In contrast, for $\ins\notin\lang$, the encryption completely hides the message.
%The compiler works as follows. The parties run the original two-message protocol for explainable verifiers, only that the prover sends its message under a witness encryption, where the corresponding statement is that the verifier's message is explainable (namely, it is in the support of the honest verifier's messages). The honest verifier uses its randomness as the witness for this statement to recover the underlying message and run the verifier of the underlying protocol. 
Our first compiler is based on two-message conditional disclosure of secrets schemes for $\NP$, which is known under standard assumptions \cite{AielloIR01,BitanskyP12,Ananth017}. In such a scheme, the verifier first sends an instance $\ins'$ for some $\NP$ language $\lang'$ together with an encrypted witness. The prover responds with an encryption of a message, which the honest verifier can then decrypt. In contrast, if a cheating verifier sends $\ins'\notin\lang'$, the prover's message is completely hidden.

The compiler works as follows. The parties emulate the original two-message protocol for explainable verifiers.
The verifier also sends the first message of a conditional disclosure protocol for the statement $\ins'$ asserting that its message is explainable (namely, it is in the support of the honest verifier's messages). The prover then responds with an encryption, relative to $\ins'$, of its second message in the underlying protocol. The verifier decrypts and verifies the underlying protocol. 

Intuitively, if the verifier does not behave in an explainable manner, the statement $\ins'$ is false, the prover's message is hidden, and the verifier learns nothing. If the verifier is explainable, then the weak zero-knowledge guarantee of the underlying protocol kicks in. To argue soundness, we would like to give a reduction that can efficiently extract the prover's encrypted message, without using the verifier's randomness. To this end, the prover provides a proof-of-knowledge of its message. To enable such a proof of knowledge in only two messages, we again rely on complexity leveraging. 

%(or else, the prover might somehow maul the verifier first message in the conditional disclosure protocol). 

\paragraph{A three-message compiler based on polynomial assumptions.} A natural approach toward a three-message compiler based on polynomial assumptions is to augment the previous compiler with a three-message proof of knowledge (rather than a two-message one based on complexity leveraging). However, we do not know how to prove that this approach works. In a nutshell, the issue is that the explainability of the verifier's message may now depend on the first prover message, and cannot be efficiently tested.
%this is because the reduction only breaks witness encryption in case that the verifier message is not explainable. However, explainability is not identifiable. In the two-message setting this is not an issue as whether the verifier is explainable or not is non-uniformly determined by its first message. In the three-message setting, however, explainability may be adaptively and implicitly determined based on the first message that the verifier obtains.
% \footnote{In a nutshell, this is because the reduction only breaks witness encryption in case that the verifier message is not explainable. However, explainability is not identifiable. In the two-message setting this is not an issue as whether the verifier is explainable or not is non-uniformly determined by its first message. In the three-message setting, however, explainability may be adaptively and implicitly determined based on the first message that the verifier obtains.} 
Instead, we take a different approach inspired by \cite{BitanskyP15}. 

To understand the basic idea behind the compiler, imagine first \omer{suppose first}\nir{Imagine!} that the language $\lang$ is in $\NP\cap\coNP$. The compiler works as follows. Given the statement $\ins$, the verifier provides, together with its message, a witness-indistinguishable argument that either $\ins \notin \lang$ or that its message is explainable; namely, there exists randomness for the honest verifier strategy that is consistent with the messages. Note that $\ins \notin \lang$ is indeed an $\NP$ statement since $\lang\in\coNP$.

We first argue that the compiler preserves the privacy guarantee of the original protocol. By the soundness of the witness-indistinguishable argument, for every $\ins\in \lang$, if the verifier sends a message that is not explainable, the prover immediately aborts. Thus, the view of a malicious verifier can be simulated from that of an explainable verifier. As for soundness, if $\ins\notin \lang$, then, since $\lang\in\coNP$, there exists a witness for this fact. Given this witness as a non-uniform advice, the reduction can turn any cheating prover against the compiled scheme into a cheating prover against the original scheme. By witness indistinguishability, the reduction can use the witness for $\ins\notin \lang$ to compute the witness-indistinguishable arguments without compromising the verifier's randomness.

To extend the above to all of $\NP$, we use the first prover message to map the statement $\ins$ into a related $\coNP$ statement. For this, we rely on perfectly binding  {\em dense commitments} where every string is a valid commitment to some value. The prover, in the first message, commits to the witness $\wit$ using the dense commitment. The verifier proceeds to prove that the prover's commitment can be opened to a string which is not a valid witness for $\ins$ (or that its messages can be explained).

To argue soundness when $\ins\notin\lang$, note that the dense commitment can necessarily be opened to some string, which is not a witness. The reduction then proceeds as in the previous protocol. Weak zero-knowledge follows by a simple extension of the previous argument. If the commitment in the first message indeed contains a valid witness, then by the binding of the commitment and the soundness of the verifier's proofs, the verifier fails to prove that the commitment is to a non-witness. Thus, the view of a malicious verifier can be simulated given the view of an explainable verifier and a commitment to a witness. Furthermore, by the hiding of the commitment, such simulation is possible even given a commitment to garbage, which the simulator can generate alone. 

We note that this compiler actually preserves all natural security notions (like, zero-knowledge, weak zero-knowledge, or witness hiding).

%old explanation:
%To extend this idea to all of $\NP$, we essentially show how to map any language $\lang\in\NP$ to a related language $\lang'$ in $\NP\cap\coNP$. This mapping will be inefficient (we certainly do not show that $\NP=\coNP$), but will be indistinguishable from an efficient mapping. For this, we rely on perfectly binding  {\em dense commitments} where every string is a valid commitment to some value. We define the language 
%$$\lang' = \set{(\ins,\cmt): \text{$\cmt$ is a commitment to a witness $\wit$ for $\ins$}}\enspace.$$
%Indeed, since the commitment is dense, if $\ins\notin\lang$, the commitment $\cmt$ can always be opened to a non-witness, and thus $\lang'\in \NP\cap\coNP$. In the compiled protocol, the prover will first map $\ins$ to $(\ins,\cmt)$, where $\cmt$ is a random commitment to the witness, and then the parties will run the $\NP\cap\coNP$ protocol for $\lang'$.
%To argue soundness, note that any no instance $\ins\notin\lang$ can only be mapped to a no instance $(\ins,\cmt)\in\lang'$, and thus the soundness of the previous compiler applies. To argue weak zero-knowledge, we cannot simply invoke the previous simulator on the mapped yes instance $(\ins,\cmt)$, since the mapping cannot be computed efficiently, without the witness $\wit$. Instead, we use an indistinguishable mapping. We map $\ins$ to $(\ins,\cmt)$ where $\cmt$ is a random commitment to garbage rather than to a witness. Since the simulator and distinguisher are efficient, and the commitment is hiding they cannot tell whether we are using the real mapping or the fake mapping, and thus simulation is valid.

\paragraph{Two-message witness-hiding compilers.} We provide another two-message compiler for witness hiding protocol that is based on polynomial assumptions and is also publicly verifiable. The compiler works for any language $\lang\in\NP$ provided a witness encryption scheme for $\lang$.


The compiler is as follows. Given the statement $\ins$, the verifier sends, together with its message, an encryption of its randomness under witness encryption, using the instance $\ins$ as the public-key. The honest prover, holding a witness, can decrypt and abort in case of malicious behavior. The compiler guarantees that if the verifier is not explainable, the prover aborts. Therefore, intuitively, such a verifier does not obtain any information.
However, this intuition is misleading --- a malicious verifier may generate messages without knowing whether they are explainable, and use the prover's abort decision to learn this bit of information.\footnote{In fact, for some instantiations of the witness encryption, this protocol reveals an arbitrary bit of the witness \cite{BitanskyP15}.} Nonetheless, the compiler does preserve witness hiding --- the witness-finding reduction can simply guess if the verifier's message is explainable and simulate the prover's message accordingly. This only decreases its success probability by a factor of two.

\subsection{More on Related Work}

We next address related work in more detail. 

\paragraph{Weak zero-knowledge and witness hiding.} The notion of weak zero-knowledge is introduced in \cite{DworkNRS03} who study the connection between 3-message {\em public-coin} weak zero-knowledge and so-called {\em magic functions.}  (They also consider several variants of the definition.) The notion of witness hiding is introduced in \cite{FeigeS90} who prove that any witness-indistinguishable protocol is witness hiding for distributions on statements with at least two ``independent'' witnesses. 
In \cite{BitanskyP12}, three-message weak zero-knowledge and witness-hiding protocols are constructed based on non-standard assumptions, which by now are considered implausible \cite{BrzuskaM14a,BellareST16}. Specifically, these constructions are based on the notion of recognizable auxiliary-input point obfuscation that was shown in \cite{BellareST16} to be impossible assuming virtual-grey-box obfuscation exists.


\paragraph{Upgrading weak zero-knowledge.}
The work of \cite{ChungLP15} considers two relaxed notions of zero knowledge and proves that they are equivalent to their weak variants (where the simulator can depend on the distinguisher). The first notion they consider is distributional zero-knowledge where instances are sampled from some known distribution (and the simulator can depend on this distribution). The second notion is zero knowledge against uniform distinguishers (these distinguishers can still get an auxiliary input, but the same input is given to the simulator). In both settings, the equivalence is shown for $(t,\epsilon)$-zero-knowledge, where the distinguisher's running time and distinguishing gap are bounded by $t$ and $\epsilon$, respectively, and the simulator's running time can depend on $t$ and $1/\epsilon$. 

Combining our weak-zero-knowledge protocols with the equivalence theorems of \cite{ChungLP15} yields distributional $(t,\epsilon)$-zero-knowledge and $(t,\epsilon)$-zero-knowledge against uniform distinguishers. Note that the two-message lower bound of \cite{GoldreichO94} does not apply for these notions. 
%\footnote{All of these notions are still weak in the sense that the simulator gets any non-uniform auxiliary-input that the distinguisher does, which otherwise has to be uniform.} Indeed, our results imply these forms in two messages for $\NP\cap\coNP$.

%Next we mention results on the round complexity of several other variants of zero knowledge. 

\paragraph{Distributional security against non-adaptive verifiers.}
The work of \cite{JKKR17} constructs {\em distributional} weak-zero-knowledge and witness-hiding protocols for a restricted class of {\em non-adaptive verifiers} who choose their messages obliviously of the proven statement. 
They give protocols in three messages under standard assumptions, and in two messages under standard, but super-polynomial, assumptions. Their  simulators and (witness-finding) reductions access the verifier as a black box.

\paragraph{Bounded description adversaries.} 
Another type of relaxation considered in the literature is restricting the (adversarial) verifier or prover to a-priori bounded description (and arbitrary polynomial running time). Here (full-fledged) zero-knowledge can be constructed in two messages against bounded-description verifiers under standard, but super-polynomial, assumptions \cite{BitanskyCPR14}, and in three messages against bounded-description provers assuming also keyless hash functions that are collision-resistant against bounded-description adversaries \cite{BitanskyBKPV16}. 

\paragraph{Super-polynomial simulation.} 
Zero knowledge with simulators that run in super-polynomial time can be constructed in two messages from standard, but super-polynomial, assumptions \cite{Pass03,BadrinarayananG17}. One-message zero-knowledge with super-polynomial simulation can be constructed 
against uniform provers, 
assuming uniform collision-resistant keyless hash functions \cite{BarakP04}, or against non-uniform verifiers, but with {\em weak soundness}, assuming multi-collision-resistant keyless hash functions \cite{BitanskyL18}.
Such zero-knowledge implies a weak notion of witness hiding for distributions on instances where it is hard to find a witness, even for algorithms that run in the same super-polynomial time as the simulator.

\paragraph{Zero-knowledge proofs.} So far, we have focused on the notion of arguments (which are only computationally sound). The round complexity of zero-knowledge proofs (which are statistically sound) has also been studied extensively.
Four-message proofs are impossible to achieve via black-box simulation, except for languages in $\NP\cap\coMA$ \cite{Katz12}. Four message proofs with non-black-box simulation are only known assuming multi-collision-resistance keyless hash functions \cite{BitanskyKP18}. 
Recent evidence \cite{FleischhackerG018} suggests that, differently from zero-knowledge arguments, zero-knowledge proofs may be impossible to achieve in three messages (even with non-black-box simulation). 

\paragraph{Honest-verifier zero knowledge.}
For languages in the class $\SZK$, there exist two-message proofs with an inefficient prover (known as Arthur-Merlin proofs) that are zero knowledge only against honest verifiers \cite{AielloH91,SahaiV97}. 
%Under computational assumptions, honest-verifier two-message zero-knowledge proofs for all of $\NP$ can be obtained by instantiating the Feige-Lapidot-Shamir paradigm with two-message witness-indistinguishable proofs \cite{DworkN07}.   
Two-message honest-verifier zero-knowledge is implied by any NIZK with a common {\em random} string (such a NIZK exists under computational assumptions).

% \paragraph{Concurrent work.} In a concurrent work Deshpande and Kalai achieve a distributional notion of 2-message witness hiding based on non-standard (and in particular, non falsifiable) assumptions \cite{DeshpandeK18}.

==> old.tex <==
%james: if you like, you can use this for reference on post-quantum extractable commitments

\section{Old Constructions}
\subsection{Post-Quantum Extractable Commitments against Explainable Adversaries.}
\paragraph{Ingredients and notation:}
\begin{itemize}
%\item
%A $3$-message \WI argument $(\wiP,\wiV)$ with delayed input. We denote its messages by $(\wi_1,\wi_2)$.
\item
  A non-interactive perfectly-binding commitment scheme $\COM$. 
\item
 A fully-homomorphic encryption scheme $(\fheE,$ $\fheD,$ $\fheEv)$.
\item
  A compute-and-compare obfuscator $\O$.
\item 
 A secure function evaluation protocol $\mathsf{SFE}$.
\end{itemize}
%
We describe the protocol in \figref{fig:ext_com}.

\protocol
{\proref{fig:ext_com}}
{A constant round extractable commitment.}
{fig:ext_com}
{
\begin{description}
    %\item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\eC$'s input:] A message $m \in \{0,1\}^{p(\secp)}$.
\end{description}

\begin{enumerate}
\item
$\eR$ computes $\dk \leftarrow \sfegen(1^\secp)$, and
computes a non-interactive commitment to $\dk$,
$\cmt_1 \leftarrow \COM(1^\secp, \dk)$.
%\item
%$\eC$ computes a challenge $\beta \leftarrow \Sigma.\eR$, and proceeds to the following.
\item
$\eC$ computes $s \leftarrow U_\secp, t \leftarrow U_\secp, (\fhePK,\fheK) \leftarrow \fheKg(1^\secp)$
 and sends
$$\fhePK, \ct_\eC \leftarrow \fheE_{\fhePK}(t),
\obfC\gets \O\Big(\CC{\fheD_\fheK(\cdot)}{s}{(\mathsf{sk},m)}\Big).$$
\item $\eR$ sends $\ct_\eR \leftarrow \sfeenc_\dk(0^\secp)$, where $\dk$ is the SFE key that $\eR$ sent inside $\cmt_1$.
\item $\eC$ sends $\widehat{\ct} \leftarrow \sfeeval \Big(\CC{\mathsf{Id}(\cdot)}{t}{s}, \ct_\eR \Big)$, where $\mathsf{Id}(\cdot)$ is the identity function.
\end{enumerate}
}

\begin{remark}[FHE Compactness]\label{rem:compactness}
In the protocol the decryption circuit $\fheD_{\fheK}$ is meant to decrypt encryptions of messages of size $|s|=\secp$. Such encryptions could be the result of homomorphic evaluation, and according to the compactness property of the FHE will have fixed polynomial size in the security parameter. 
\end{remark}





==> qtagfhe.tex <==
\section{Tagged Quantum Fully-Homomorphic Encryption}

In the following we define and construct a tagged fully-homomorphic encryption that supports the homomorphic evaluation of quantum circuits. This notion is going to be instrumental to build (post-quantum secure) non-malleable commitments.

\subsection{Definition}

\gnote{The following definition is obsolete, the only correct thing is the definition of tag-based security}

In the following we defined the notion of tagged quantum fully-homomorphic encryption. Note that we define a weak notion of homomorphism, in the sense that (i) it evaluates quantum circuits over classically (encrypted) bits and (ii) evaluation correctness is guaranteed only for (multi-bit) ciphertexts encrypted with a single call of the encryption algorithm.

\begin{definition}[Tagged Quantum Fully Homomorphic Encryption]
\label{def:tag-qfhe}
For every $N \in \mathbb{N}$,
a tagged QFHE scheme for tags in $[N]$ consists of six algorithms $(\fheKg, \fheE, \fheD, \fheEv)$ with the following syntax:
\begin{itemize}
\item $(pk_\tagg,sk_\tagg) \leftarrow \fheKg(1^\secp,\tagg)$ : A PPT algorithm that given a security parameter and a tag, samples a
classical tagged public key and a classical tagged secret key.
\item $(c_{\tagg,1}, \dots, c_{\tagg,\ell}) \leftarrow \fheE_{pk_\tagg}(b_1, \dots, b_\ell)$ : A PPT algorithm that takes as input a $\ell$ bits $(b_1, \dots, b_\ell)$ and outputs $\ell$ classical ciphertexts.
\item $b \leftarrow \fheD_{sk_\tagg}(c_\tagg)$ : A PPT algorithm that takes as input a classical tagged ciphertext $c$ and a key with the same tag, and outputs a bit.
\item $(\widehat{c_{\tagg,1}}, \dots, \widehat{c_{\tagg,\ell}}) \leftarrow \fheEv_{pk_\tagg}(C, (c_{\tagg,1}, \dots, c_{\tagg,\ell}))$ : A QPT algorithm that takes as input:
\begin{enumerate}
\item A general quantum circuit $C$ with $\ell$ classical bits of input and $m$ classical bits of output.
\item $\ell$ classical ciphertexts $(c_{\tagg,1}, \dots, c_{\tagg,\ell})$ that encrypt $\ell$ classical bits.
\end{enumerate}
The evaluation algorithm outputs $m$ classical ciphertexts $(\widehat{c_{\tagg,1}}, \dots, \widehat{c_{\tagg,\ell}})$ encrypting $m$ classical bits.
\end{itemize}

The scheme satisfies classical semantic security, compactness and a weak form of correctness, as defined below:
\begin{itemize}
\item \noindent {\bf{(Weak) Correctness.}}
There exists a negligible function $\nu$ such that for every $\secp\in\mathbb{N}$, every quantum circuit $C$ with $\ell$ classical bits of input and $m$ classical bits of output, every set of inputs $(b_1, \dots, b_\ell)$, every tag  $\tagg \in [N]$, and every $(\pk_\tagg,\sk_\tagg)$ in the support of $\fheKg(1^\secp, \tagg)$, it holds that
$$
\Pr\left[C(b_1, \dots, b_\ell) \neq \fheD_{\sk_\tagg}(\fheEv_{\pk_\tagg}(C, \fheE_{pk_\tagg}(b_1, \dots, b_\ell)))\right] = \nu(\secp).
$$
\end{itemize}

Additionally, it satisfies tag-based security as described below:
\begin{itemize}
\item \noindent {\bf{Tag-based security.}}
For every explainable QPT adversary $\A$, there exists a negligible function $\nu$ such that for $\tagg, \ttagg \in [N]$ such that $\tagg > \ttagg$, the probability that the challenger $\mathsf{Ch}$ outputs $1$ in \proref{fig:requirement} is $\nu(\secp)$.
\end{itemize}
\end{definition}

\gnote{Clarify Protocol 1}

\subsection{Construction}

\gnote{Construction from LR-PKE and QFHE}

\begin{theorem}
Assuming quantum hardness of LWE, plus a circular security assumption on LWE, there exists a tagged Quantum Fully Homomorphic encryption scheme for tags in $[\log \secp]$ satisfying Definition \ref{def:tag-qfhe}.
\end{theorem}
\begin{proof}
\dnote{TBD, looks like this follows from Urmila's scheme.}

How to instantiate: 
%Let QFHE scheme with security parameter $k$ be such that on input message of size $\mu$ and key of size $k$, the ciphertext is of size $r.\mu + k^c$ for some constants $r$ and $c$.
On input $(1^\lambda, \tagg)$, the keygen algorithm outputs the secret key for a scheme with security parameter $\tagg \cdot \lambda$.

Need to use leakage resilience to argue that the adversary cannot guess $m$ with only $\ttagg\cdot\lambda$ bits of leakage on $\fhePK_\tagg, \ct_\tagg$.
\end{proof}

%Moreover, the size of public key corresponding to $\tagg$ is at most a constant multiple of the size of public key corresponding to $\tagg'$.

\protocol
{\proref{fig:requirement}}
{Requirement on FHE.}
{fig:requirement}
{
\begin{itemize}
    \item $\mathsf{Ch}$ samples $(\fhePK_\tagg, \fheK_\tagg) \leftarrow \fheKg(1^\secp,\tagg)$ and outputs $\fhePK_\tagg$.
    \item $\A$ on input $(\tagg, \fhePK_\tagg)$ outputs $(\ttagg, \fhePK'_{\ttagg})$.
    \item $\mathsf{Ch}$ samples $t \leftarrow U_{\tagg \cdot \secp}$. It computes $\ct_\tagg = \fheE_{\fhePK_\tagg}(t)$,
    and outputs $\ct_\tagg$.
    \item $\A$ on input $\ct_\tagg$ outputs $\ct'_{\ttagg}$.
    \item $\mathsf{Ch}$ on input $(\fhePK'_{\ttagg}, \ct'_{\ttagg})$ computes the lexicographically first $t' \in \{0,1\}^{\ttagg \cdot \secp}$ such that $\exists r'$ such that $\ct'_{\ttagg} = \fheE_{\fhePK_{\ttagg}}(t';r')$, and outputs $t'$. It outputs $\bot$ if no such $t'$ exists. 
    %\dnote{A unique $t'$ is guaranteed to exist for every explainably chosen set of values, by our definition of QFHE.}.
    \item $\A$ on input $t'$ outputs $m$.
    \item $\mathsf{Ch}$ outputs $1$ if and only if $\ttagg \neq \tagg$ and $m = t$.
\end{itemize}
}


==> weakzk-old.tex <==
\section{Weak Zero-Knowledge against Explainable Verifiers}\label{sec:semi_mal}

In this section, we construct \WZK protocols against explainable verifiers. We start with the three-message protocol and then move to the 2-message protocol, which will be a special case of the 3-message protocol.

\subsection{The Three-Message Protocol}\label{sec:3wzk_expl}

In this section, we construct a three-message \WZK argument against explainable verifiers.

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
 A 3-message extractable commitment $(\comS,\comR,\comV)$. We denote its messages by $(\cm_1,\cm_2,\cm_3)$.
\item
a 2-message \WI argument $(\wiP,\wiV)$ with delayed input. We denote its messages by $(\wi_1,\wi_2)$.
\item
  A non-interactive perfectly-binding commitment scheme $\COM$. 
\item
 A fully-homomorphic encryption scheme $(\fheE,$ $\fheD,$ $\fheEv)$.
\item
  A compute-and-compare obfuscator $\O$.
  \item
  A random self-reducible public-key encryption $(\rsreG,$ $\rsreE,$ $\rsreD,$ $\rsretD)$. (In fact, relaxed RSR suffices. To simplify the description of the protocol, we rely on standard RSR, and later remark why relaxed RSR suffices.)
\end{itemize}
%
We describe the protocol in \figref{fig:wzk_prot}.

\protocol
{\proref{fig:wzk_prot}}
{A 3-message $\WZK$ argument for $\NP$ against explainable verifiers.}
{fig:wzk_prot}
{
\begin{description}
    \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
\end{description}

\begin{enumerate}
\item
$\zkP$ computes $(\cm_1,\tau) \gets \comS(0^\secp)$, the first message and state of an extractable commitment to zero. It sends $\cm_1$.
\item
$\zkV$ computes
\begin{itemize}
\item
$\cm_2 \gets \comR(\cm_1)$, the second message of the extractable commitment.
\item
$(\wi_1,\tau_\zkV) \gets \wiV_1(1^\secp)$, the first \WI message and a corresponding state.
\item
$\cmt \gets \COM(0;r)$, a commitment to zero, using randomness $r \gets \zo^\secp$,
\item
$\zkVCT \gets \fheE_{\fheK}(r)$, an encryption of the commitment randomness, under a randomly chosen secret key $\fheK\gets \zo^\secp$.
\item
$\obfC\gets \O(\CC{\fheD_\fheK,u})$, an obfuscation of the CC program given by the FHE decryption circuit and a random target $u\gets \zo^\secp$.
\item
$\zkVCT' \gets \rsreE_{\rsrePK}(u)$, an RSR encryption of the target $u$, where $(\rsreSK',\rsrePK')\gets \rsreG(1^\secp)$ are randomly chosen keys.
\end{itemize}
It sends $(\cm_2,\wi_1,\cmt,\zkVCT,\obfC,\zkVCT',\rsrePK')$.
\item 
$\zkP$ computes
\begin{itemize}
\item
$\cm_3 \gets \comS(\cm_1,\cm_2;\tau)$, the third message of the extractable commitment.
\item
$\zkPCT\gets \rsreE_{\rsrePK'}(1)$, an RSR encryption of $1$.
\item
$\wi_2 \gets \wiP(\Psi,\wit,\wi_1)$, the second $\WI$ message for the statement
\begin{align*}
\Psi(\ins,\cmt,\obfC,&\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3) :=\\
     &\exists \wit  \; : \; (\ins,\wit) \in \RL \hspace{2mm} &\bigvee\\ &\exists r \; : \;
    \cmt = \COM(0;r) \hspace{2mm} &\bigvee\\ 
    &\exists \evciph \; : \;
    \obfC(\evciph) = 1 \hspace{2mm} &\bigvee\\ 
    &\exists r' \; : \; \zkPCT = \rsreE_{\rsrePK'}(0;r')  \hspace{2mm}\bigwedge\hspace{2mm} (\cm_1,\cm_2,\cm_3) \in \comS(r')
    \hspace{2mm}\enspace.
\end{align*}
% using the witness $\wit\in\RL(\ins)$.
 \end{itemize}
 It sends $(\cm_3,\zkPCT,\wi_2)$.
 \item
    $\zkV$ verifies 
    \begin{itemize}
    \item
    the commitment $\comV(\cm_1,\cm_2,\cm_3)=1$,
    \item
    that the WI argument is accepted: $\wiV_2(\Psi,\wi_1,\wi_2;\tau_\zkV)=1$,
    \item
    that the prover's ciphertext decrypts to one: $\rsreD_{\rsreSK'}(\zkPCT)=1$.
    \end{itemize}
\end{enumerate}
}

\begin{remark}[FHE Compactness]\label{rem:compactness}
In the protocol the decryption circuit $\fheD_{\fheK}$ is meant to decrypt encryptions of messages of size $|u|=\secp$. Such encryptions could be the result of homomorphic evaluation, and according to the compactness property of the FHE will have fixed polynomial size in the security parameter. 
\end{remark}

\subsubsection{Analysis}

We now analyze the protocol. We first show that it is sound, and then that it is $\WZK$ against explainable verifiers.

\begin{proposition}
\proref{fig:wzk_prot} is sound.
\end{proposition}
\begin{proof}
Assume toward contradiction that there exists a polynomial-size (w.l.o.g deterministic) prover $\zkmP=\set{\zkmP_\secp}$ that (for infinitely many $\secp\in\Nat$) breaks soundness with noticeable probability $\varepsilon(\secp) =\secp^{-O(1)}$. Fix $\secp\in\Nat$ and $\ins\in \zo^\secp\setminus \lang$ such that $\zkmP_\secp$ convinces the verifier of accepting with probability $\varepsilon$. 

\paragraph{Augmenting the interaction with extraction.} We parse any verifier message $(\cm_2,\wi_1,\cmt,\zkVCT,\obfC,\zkVCT',\rsrePK')$, as two parts $(\cm_2,z)$. For any $z$, we consider a sender $\commS_z$ whose first message is the same $\cm_1$ output by $\zkmP_\secp$, and given a message $\cm_2$ from the receiver $\comR$, computes the third message $\cm_3$ by running $\zkmP_\secp$ on $(\cm_2,z)$, emulating a message form $\zkV$. For any transcript $T=(\cm_1,(\cm_2,z),(\cm_3,\zkPCT,\wi_2))$ of an execution between $\zkmP_\secp$ and $\zkV$, we consider the result $s_T$ of running the witness extractor $s_T \gets \zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$. (Note that $s_T$ is a random variable that may depend on $T$ and the extractor's coins.)

Let $F$ be the event, over a transcript $T$ and coins of the extractor $\zkE$, that: 
\begin{enumerate}
    \item
    $\zkV$ successfully verifies the commitment transcript $(\cm_1,\cm_2,\cm_3)$,
    \item $\zkV$ accepts the WI argument $(\wi_1,\wi_2)$,
    \item
    the
    the extracted string $s_T$ does {\bf not} attest that $\zkPCT$ is a zero encryption; that is, $s_T$ is {\bf not} randomness $r'$ such that $\zkPCT = \rsreE(0;r')$.
\end{enumerate} 
%
We next consider several hybrid experiments and show that the probability that $F$ occurs is preserved through these experiments, upto a negligible difference. To reach a contradiction, we show that $F$ occurs in the first hybrid with probability at least $\varepsilon$ and with probability at most $\varepsilon/2$ in the last hybrid. This is a contradiction since the gap $\varepsilon/2$ is noticeable. In what follows, in each hybrid $i$, we will denote by  $p_i$ the probability that $F$ occurs in that hybrid.  

\paragraph{$\hyb_0$:} This is the real protocol.

\begin{claim}
$p_0 \geq \varepsilon$.
\end{claim}
\begin{proof}
By definition, whenever $\zkV$ accepts, it decrypts $\zkPCT$ to $1$; thus, by the correctness of $\rsre$, the ciphertext $\zkPCT$ cannot be opened to an encryption of $0$.  The claim now follows from the fact that $\zkmP_\secp$ convinces $\zkV$ with probability $\varepsilon$.
\end{proof}


\paragraph{$\hyb_1$:} In this hybrid, $\zkVCT'$ is an encryption of $0^\secp$ instead of the target $u$. 

\begin{claim}
$\abs{p_0-p_1} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the semantic security of the scheme $\rsre$. Indeed, given a noticeable difference between $p_0$ and $p_1$, we can distinguish an RSR encryption of a random $u$ from one of $0^\secp$, by emulating an interaction between $\zkmP_\secp$ and $\zkV$, running the extractor, and testing whether $F$ occurs. 
\end{proof}



\paragraph{$\hyb_2$:} In this hybrid, the obfuscation $\obfC \gets \ccSim(1^\secp,1^\ell)$ is simulated rather than an obfuscation of $\CC{\fheD_{\fheK},u}$, where $\ell$ is the size of the decryption circuit $\fheD_{\fheK}$.


\begin{claim}
$\abs{p_1-p_2} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the CC simulation guarantee. Indeed, given a noticeable difference between $p_1$ and $p_2$, we can distinguish, given $\fheK$, an obfuscation of $\CC{\fheD_{\fheK},u}$ for a random $u$, from a simulated obfuscation contradicting the CC guarantee. Using the fact that now $\zkVCT'$ is an encryption of $0^\secp$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}


\paragraph{$\hyb_3$:} In this hybrid, $\zkVCT$ is an encryption of $0^\secp$ instead of the commitment randomness $r$.


\begin{claim}
$\abs{p_2-p_3} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the semantic security of the FHE scheme $\fhe$. Indeed, given a noticeable difference between $p_2$ and $p_3$, we can distinguish, an encryption of a random $r$ from an encryption of $0^\secp$. Since now the FHE key $\fheK$ is not needed to compute the obfuscation $\obfC$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}


\paragraph{$\hyb_4$:} In this hybrid, $\cmt$ is a commitment to $1$ instead of $0$.

\begin{claim}
$\abs{p_3-p_4} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by hiding of the commitment. Given a noticeable difference between $p_3$ and $p_4$, we can distinguish, a commitment to zero from a commitment to one. In this hybrid, $\zkVCT$ no longer depends on the commitment randomness, so we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}

.

\medskip\noindent
It is left to show that in $\hyb_4$, $F$ occurs with probability at most $\varepsilon/2$. 

\begin{claim}
$p_4 \leq \varepsilon/2$.
\end{claim}
\begin{proof}
Assume toward contradiction that $p_4 > \varepsilon/2$. First, observe that in hybrid $\hyb_4$:
\begin{itemize}
\item
$\ins\notin \lang$.
\item
$\cmt \in \COM(1)$, and by perfect binding there does not exist $r$ such that $\cmt = \COM(0;r)$.
\item
By the CC simulation guarantee, except with negligible probability $2^{-\secp}$, there does not exist $\evciph$ such that $\obfC(\evciph) = 1$.
\end{itemize}
In particular, we can fix the second part $z$ of the  verifier's message such that with probability at least $\varepsilon/2-2^{-\secp}$, over $\cm_2$:
\begin{enumerate}
    
    \item 
    The above three conditions hold (for $\cmt,\obfC$ fixed by $z$).
    \item
    The WI verifier $\wiV$ accepts the argument (for the statement $\Psi$).
    \item
    The commitment verifier $\comV$ accepts the transcript $(\cm_1,\cm_2,\cm_3)$.
    \item
    The extractor $\zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$ outputs $s_T$ that does not attest that $\zkPCT$ is a zero encryption. 
\end{enumerate}
Invoking the soundness of the $\WI$ argument, it follows that with probability at least $\varepsilon/2-2^{-\secp} \secp^{-\omega(1)}\gg 2^{-\secp}$, over $\cm_2$:
\begin{enumerate}
    \item 
    The commitment verifier $\comV$ accepts the transcript $(\cm_1,\cm_2,\cm_3)$.
    \item
    $\exists r'$ such that $(\cm_1,\cm_2,\cm_3) \in \comS(r')$, and $r'$ attests that $\zkPCT$ is a zero encryption.
    \item
    The extractor $\zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$ outputs $s_T$ that does not attest that $\zkPCT$ is a zero encryption. In particular, $s_T\neq r'$. 
\end{enumerate}
This contradicts the extraction guarantee of the commitment.
\end{proof}
This concludes the proof of soundness.
\end{proof}

\begin{proposition}\label{prp:sim}
\proref{fig:wzk_prot} is weak zero-knowledge against explainable verifiers.
\end{proposition}

\begin{proof}
\def \ranmal {r^*}  
We describe the simulator $\zkS$. Throughout, we assume w.l.o.g that the malicious verifier $\zkmV$ outputs its view consisting of its random coins and prover messages.
(Otherwise, we consider a new verifier of this form, along with a new distinguisher who computes internally the original verifier output, and then applies the original distinguisher.)

\medskip
\paragraph{$\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
\begin{enumerate}
\item
Sample coins $\ranmal$ for $\zkmV_\secp$. Henceforth, $\zkmV_{\ranmal}$ denotes the corresponding (deterministic) verifier.
\item
Sample a random $r'\gets \zo^\secp$ and a first commitment message and state $(\cm_1,\tau)\gets \comS(r')$ corresponding to a commitment to $r'$. Store the randomness $r_{\cm}$ used to generate the commitment. Feed $\cm_1$  to $\zkmV_{\ranmal}$. 
\item
If the verifier aborts, output $(\ranmal,\cm_1,\bot)$.
\item \label{stp:ver_mes}
Obtain $(\cm_2,\cmt,\zkVCT,\obfC, \zkVCT',\rsrePK',\wi_1)$ from $\zkmV_{\ranmal}$
\item
Compute the third commitment message $\cm_3 \gets \comS(\cm_1,\cm_2;\tau)$.
\item
Construct the ({\em homomorphic simulation}) circuit $\HC(r)$ that given an input $r$:
\begin{itemize}
\item
Construct a distinguisher $\rsremD'(\zkPCT)$ for the RSR encryption that given a ciphertext $\zkPCT$: 
\begin{itemize}
\item
Samples at random a second $\WI$ message $$\wi_2 \gets \wiP(\Psi,r,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r$ attesting that $\cmt=\COM(0;r)$.
\item
Runs $\zkmD_\secp(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{itemize}
\item 
Applies the decryptor
$$
\tilde u \gets \rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon})\enspace,
$$
and output $\tilde u$.
\end{itemize}  
All randomness required by the above is hardwired into $\HC$.
\item
Compute $\evciph = \fheEv(\HC,\zkVCT)$.

\item \label{stp:td1}
If $\obfC(\evciph)=1$: 
\begin{itemize}
\item
Sample $\zkPCT\gets \rsreE_{\rsrePK'}(1)$. 
\item
Sample a second $\WI$ message 
$$\wi_2 \gets \wiP(\Psi,\evciph,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness $\evciph$ attesting that $\obfC(\evciph)=1$. 
\end{itemize}
\item
Otherwise:\label{stp:td2}
\begin{itemize}
\item
Compute $\zkPCT =  \rsreE_{\rsrePK'}(0;r')$, where $r'$ is the randomness underlying the extractable commitment. 
\item
Sample a second $\WI$ message 
$$\wi_2 \gets \wiP(\Psi,(r',r_\cm),\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r'$ attesting that $\zkPCT\gets \rsreE_{\rsrePK'}(0;r')$ and the commitment randomness $r_\cm$. 
\end{itemize}
\item
Output $(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{enumerate}

\paragraph{Simulation validity.} The simulator clearly runs in polynomial time (in its input length). We focus on proving validity. Let $\zkmV=\set{\zkmV_\secp}_\secp$ be a polynomial-size explainable verifier, let $\zkmD=\set{\zkmD_\secp}_\secp$  be a polynomial-size distinguisher, and let $\varepsilon(\secp)=\secp^{-O(1)}$. 
% Fix any $\secp$, and $x\in \lang\cap\zo^\secp$ such that the message sent by $\zkmV_\secp$ is explainable (i.e., it is consistent with some honest verifier message as specified in \proref{fig:wzk_prot}).

We consider a sequence of hybrid simulators that transition from the simulator to the prover, and prove that the views generated by each two consecutive hybrids are indistinguishable.

\paragraph{$\zkS_0$:} This is the real simulator $\zkS$.

\paragraph{$\zkS_1$:} This simulator is the same as $\zkS$, only that in Step \ref{stp:td2}, if it needs to give an argument (due to unsuccessful extraction of a proper $\evciph$), it uses the witness $\wit$, instead of $(r',r_\cm)$.
%\daksh{Here, I suggest that instead of using the witness $\wit$ only when there is unsuccessful extraction of a proper $\evciph$, the simulator {\em always} uses $\wit$ to generate the WI arguments (that is, in steps 6, 8, 9). Even though its possible that the distinguisher breaks WI under the hood, the overall view at the end of the simulation (including the probability of unsuccessful extraction of $\evciph$) cannot change. Then it seems like we can switch directly from $S_2$ to $P_0$ below, without requiring any non-uniform fixing. But then why do we even need $\mathsf{com}(0;r)$ from the receiver? What do you think? I may be missing something.}

\paragraph{$\zkS_2$:} This simulator is the same as $\zkS_1$, only that instead of an extractable commitment $(\cm_1,\cm_2,\cm_3)$ to $r'$, it provides a commitment to $0^\secp$.

\paragraph{$\zkS_3$:} This simulator is inefficient. It acts the same as $\zkS_2$, only that:
\begin{itemize}
    \item
    It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
    \item
    Then it finds the commitment randomness $r$, and uses it to provide proofs both in Step \ref{stp:td1} and in Step \ref{stp:td2}.
\end{itemize}

\paragraph{$\zkP_1$:} This simulator is also inefficient. It acts the same as the honest prover $\zkP$, only that:
\begin{itemize}
    \item
    It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
    \item
    Then it finds the commitment randomness $r$, and uses it to provide the \WI argument.
\end{itemize}

\paragraph{$\zkP_0$:} This simulator emulates the real prover.

To deduce the validity of the simulator, we prove:
\begin{claim}\label{clm:wzk_main}
There exists a negligible $\nu(\secp)$ such that for all $\secp\in\Nat$, $\ins\in\lang\cap\zo^\secp$, $\wit\in\RL(\ins)$, $i\in [3]$,
\begin{align*}
\zkS_{i-1}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\nu}
\zkS_{i}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace,\\
\zkS_{3}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\varepsilon+2^{-\secp}}
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins) \enspace,\\
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins)  &\approx_{\zkmD_\secp,\nu}
\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\enspace.
\end{align*}
\end{claim}

\begin{proof}
We prove the indistinguishability of each two consecutive hybrid simulators.

\medskip\noindent
\underline{$\zkS \approx \zkS_1$:} Recall that the only difference between these two simulators is that $\zkS_1$ uses the witness $\wit$ in Step \ref{stp:td2}, instead of $(r',r_{\cm})$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument.

$\wimV$ runs $\zkS$ to sample a transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS$ produces. Instead, it outputs as the first \WI message the message $\wi_1$ produced by $\zkmV$ during the simulation, as well as the statement $\Psi$ and $\wit_0=(r',r_\cm)$ and $\wit_1 = \wit$ as the two witnesses. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generated by $\zkS$, except that $\wi_2$ generated by $\zkS$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\zo$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkS_1 \approx \zkS_2$:} Recall that the only difference between these two simulators is that $\zkS_2$ commits to $0^\secp$ instead of to $r'$ like $\zkS_1$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$, then we construct a receiver $\commR$ that breaks the indistinguishability of the extractable commitment with the same advantage $\delta$. 

$\commR$ emulates $\zkS_1$, when sampling $r'$, $\commR$ submits to the challenger $s_1=r'$ and $s_2 = 0^\secp$. Then, instead of sampling $\cm_1$ as part of the simulation, $\commR$ obtains it from an outside challenger. It proceeds with the emulation of $\zkS_1$, feeding $\cm_1$ to $\zkmV$, and obtaining $\cm_2$ as part of $\zkmV$'s message. $\commR$ sends  $\cm_2$ to the challenger and obtains $\cm_3$. It then performs the rest of the emulation using $\cm_3$ (note that $\zkS_1$ no longer requires the randomness underlying the commitment in Step \ref{stp:td2}). 

It is left to observe that for each $i\in\set{1,2}$, when the challenger commits to $s_i$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\commR$ has advantage $\delta$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkS_2 \approx \zkS_3$:} Recall that the difference between these two simulators is that $\zkS_3$ aborts if the verifier's message is not explainable, and if it is uses the commitment randomness $r$ as the witness in Steps \ref{stp:td1} and $\ref{stp:td2}$, instead of $\evciph$ and $\wit$, respectively. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the simulator $\zkS_3$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two simulators are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkS$ from $\zkS_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkS_2$ starting from the point it obtains the message from $\zkmV$ (Step \ref{stp:ver_mes}), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS_2$ produces. Instead: 
\begin{itemize}
    \item If the transcript reaches Step \ref{stp:td1} (corresponding to successful extraction of $\evciph$), $\wimV$ sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_2 = \evciph$ and $\wit_3 = r$.
    \item
    If the transcript reaches Step \ref{stp:td2} (corresponding to unsuccessful extraction of $\evciph$), $\wimV$ sends to the challenger $\wi_1$ and $\Psi$ with witnesses $\wit_2 = \wit$ and $\wit_3 = r$.
\end{itemize}
It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkS_2$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\set{2,3}$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkP_1 \approx \zkP$:} We jump to prove this indistinguishability as it is very similar to the previous one (the tired reader is advised to skip it).

Recall that the difference between these two provers is that $\zkP_1$ aborts if the verifier's message is not explainable, and if it is, uses the commitment randomness $r$ as the witness when proving $\Psi$ instead of $\wit$ like $\zkP$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two provers with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the prover $\zkP_1$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two provers are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkP$ from $\zkP_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkP$ starting from the point it obtains the message from $\zkmV$ (the third protocol message), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkP_1$ produces. Instead, it sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_0 = \wit$ and $\wit_1 = r$. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkP$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\set{0,1}$, the generated view is distributed identically to that generated by $\zkP_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge.

\medskip\noindent
\underline{$\zkS_3 \approx \zkP_1$:} Note that up to receiving the verifier's $\zkmV$ message, and adding the generation of $\cm_3$, the views generated by the two simulators are distributed identically. Thus, to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability of these two simulators, it suffices to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability conditioned on any fixing of the first prover message, verifier randomness $\ranmal$ and message, and $\cm_3$. Note that if the verifier's message is not explainable, \daksh{Previously, it said not explainable or $\bot$ -- I found this confusing. Moreover, since $\bot$ is not explainable, I just removed ``or $\bot$''.} both simulators abort, and thus we concentrate on the case that the verifier's message is explainable. From hereon consider such a fixing and let $r$ be the corresponding randomness.

Let $\Delta$ be the advantage of the probabilistic distinguisher $\rsremD'$ (as defined in the simulation procedure) in distinguishing zero-encryptions from one-encryptions:
\begin{align*}\Delta := \abs{\underset{\rsremD',\rsreE}{\EE}\[\rsremD'(\rsreE_{\rsrePK'}(0))- \rsremD'(\rsreE_{\rsrePK'}(1))\]}\enspace.
\end{align*}
%
We consider two cases.

\paragraph{Case 1: $\Delta > \varepsilon$.} Let $u$ be the target string underlying the obfuscated CC program $\obfC$, and recall that $\zkVCT'\in \rsreE_{\rsrePK'}(u)$, due to explainability. Then by the random self reducibility of $\rsre$, with overwhelming probability $1-2^{-\secp}$, over the coins of $\rsretD$, it holds that
$$
\rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon}) = u\enspace,
$$
in which case, $\HC(r) = u$. Assume that this is indeed the case.

By the correctness of $\fhe$, the ciphertext $\evciph=\fheEv(\HC,\evciph)$ obtained by the simulator $\zkS_3$ satisfies:
$$
\fheD_{\fheK}(\evciph) = u\enspace,
$$
and thus by the one-sided correctness of the CC obfuscator $\O$,
$$
\obfC(\evciph) = 1\enspace.
$$
This corresponds to successful extraction of $\evciph$, and will result in the simulator $\zkS_3$ behaving identically to the prover $\zkP_1$ (in Step \ref{stp:td1}) --- sampling $\zkPCT$ as a one encryption and $\wi_2$ using the witness $r$. 

Thus, in case 1, we have $(\zkmD_\secp,2^{-\secp})$-indistinguishability.

\paragraph{Case 2: $\Delta \leq \varepsilon$.} Here we consider two sub-cases according to whether the simulator still obtains a ciphertext $\evciph$ such that $\obfC(\evciph)=1$ or not. In case it does obtain such $\evciph$, the simulator behaves exactly like $\zkP_1$. Henceforth, we assume that the simulator does not obtain such a witness, in which case it reaches Step \ref{stp:td2}. Here the difference between the simulator $\zkS_3$ and prover $\zkP_1$ is that the first samples $\zkPCT \gets \rsreE_{\rsrePK'}(0)$, whereas the second samples $\zkPCT \gets \rsreE_{\rsrePK'}(1)$. The advantage of $\zkmD_\secp$ in distinguishing the two is exactly the advantage $\Delta \leq \varepsilon$ of $\rsremD'$. This completes the proof of this case, and of \clmref{clm:wzk_main}.
\end{proof}



\begin{remark}[On using relaxed random self-reducible encryption]
We can rely on relaxed RSR encryption by slightly tweaking the protocol. Specifically, in the protocol, the encryption $\zkPCT$ will be under the alternative RSR encryption algorithm $\rsretE$. The simulation and analysis remain the same.
\end{remark}

\subsection{The Two-Message Protocol}\label{sec:2wzk_expl}

We also construct, under stronger assumptions, a two-message \WZK argument against explainable verifiers and quasipolynomial provers. Specifically we strengthen the ingredients as follows.

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
 A {\bf 2-message} extractable commitment $(\comS,\comR,\comV)$ with a quasipolynomial extractor. We denote its messages by $(\cm_2,\cm_3)$; this is for consistency with the three-message protocol ($\cm_1$ is always empty). 
\item
a 2-message \WI argument $(\wiP,\wiV)$ with delayed input, {\bf sound against quasipolynomial provers.}
\item
  A non-interactive perfectly-binding commitment scheme $\COM$, {\bf hiding against qausipolynomial distinguishers.} 
\item
 A fully-homomorphic encryption scheme $(\fheE,$ $\fheD,$ $\fheEv)$, {\bf secure against qausipolynomial distinguishers.}
\item
  A compute-and-compare obfuscator $\O$, {\bf secure against qausipolynomial distinguishers.}
  \item
  A random self-reducible public-key encryption $(\rsreG,$ $\rsreE,$ $\rsreD,$ $\rsretD)$, {\bf secure against qausipolynomial distinguishers.} (In fact, relaxed RSR suffices. To simplify the description of the protocol, we rely on standard RSR, and later remark why relaxed RSR suffices.)
\end{itemize}
%
The protocol is identical to the one in \figref{fig:wzk_prot}, only that since the first commitment message $\cm_1$ is always empty, it consists of only two messages.


\begin{proposition}
Protocol \figref{fig:wzk_prot}, instantiated with the above ingredients, is a 2-message \WZK protocol against explainable verifiers and soundness against quasipolynomial provers. 
\end{proposition}

\begin{proof}[Proof sketch.]
The proof is essentially identical to that of the previous protocol, only taking into account the above enhancements.

In the proof of soundness, the prover $\zkmP$ and the extractor $\zkE$ are now quasipolynomial instead of polynomial. Thus, each of the reductions in the proof is now quasipolynomial instead of polynomial, and breaks the quasipolynomial (rather than polynomial) security of the underlying primitives.

The same \WZK proof applies. In fact, it can be simplified. This is because obtaining the commitment randomness $r$ can now be done efficiently (non-uniformly), which means that we can invoke the indistinguishability of the extractable commitment in the presence of any one of the simulators. Thus instead of first switching to simulating the argument in the simulation Step \ref{stp:td2} with $\wit$, we can directly switch to $r$. 
\end{proof}

\section{Witness Hiding against Explainable Verifiers with Public Verification}\label{sec:pub_ver}

In this section, relying on witness encryption, we give a two-message protocol that is also publicly-verifiable. The new protocol, however, is only \WH. We start by presenting the protocol and then proceed to analyze it.

\paragraph{Ingredients and notation:} %Fix any language  $\lang\in\NP$. We use the following ingredients.
\begin{itemize}
\item
 A 2-message publicly-verifiable $\WI$ argument for \NP with delayed input $(\wiP,\wiV)$. We denote its messages by $(\wi_1,\wi_2)$.
\item
  A non-interactive perfectly-binding commitment scheme $\COM$. 
\item
 A fully-homomorphic encryption scheme $(\fheE,$ $\fheD,$ $\fheEv)$.
\item
  A compute-and-compare obfuscator $\O$.
  \item
  A witness encryption scheme $(\weE,\weD)$ for languages in \NP.
\end{itemize}
%
We describe the protocol in \figref{fig:pubv_prot}.

\protocol
{\proref{fig:pubv_prot}}
{A publicly-verifiable 2-message $\WH$ argument $\prot{\zkP}{\zkV}$ for $\lang$.}
{fig:pubv_prot}
{
\begin{description}
    \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
\end{description}

\begin{enumerate}
\item
$\zkV$ computes
\begin{itemize}
\item
$\wi_1$, the first message of the $\WI$ argument,
\item
$\cmt \gets \COM(0;r)$, a commitment to zero, using randomness $r \gets \zo^\secp$,
\item
$\zkVCT \gets \fheE_{\fheK}(r)$, an encryption of the commitment randomness, under a randomly chosen secret key $\fheK\gets \zo^\secp$.
\item
$\obfC\gets \O(\CC{\fheD_\fheK,u})$, an obfuscation of the CC program given by the FHE decryption circuit and a random target $u\gets \zo^\secp$.
\item
$\zkVCT' \gets \weE_{\ins}(u)$, a witness encryption of the target $u$.
\end{itemize}
It sends $(\wi_1,\cmt,\zkVCT,\obfC,\zkVCT')$.
\item 
$\zkP$ computes $\wi_2$, the second $\WI$ message for the statement $\Psi(\ins,\cmt,\obfC)$ given by:
\begin{align*}
     &\exists \wit  \; : \; (\ins,\wit) \in \RL \hspace{2mm} &\bigvee\\ &\exists r \; : \;
    \cmt = \COM(0;r) \hspace{2mm} &\bigvee\\ 
    &\exists \evciph \; : \;
    \obfC(\evciph) = 1 \enspace,
\end{align*}
using the witness $\wit\in\RL(\ins)$. It sends $\wi_2$.
 \item
    $\zkV$ verifies the $\WI$ argument $(\wi_1,\wi_2)$ for the statement $\Psi$.
\end{enumerate}
}

\begin{remark}[FHE Compactness]
Remark \ref{rem:compactness} regarding the fixed size of the circuit $\fheD_\fheK$ holds for the above protocol as well.
\end{remark}

\paragraph{Public verification.} The verification of an argument in the above system amounts to applying the public verification of the $\WI$ argument, and involves no private randomness.

\subsection{Analysis}

We now analyze the protocol. We first show that it is sound, and then that it is $\WH$ against explainable verifiers.

\begin{proposition}
\proref{fig:pubv_prot} is sound.
\end{proposition}
%
The soundness analysis is a simplification of that of \proref{fig:wzk_prot}. We include it here for completeness (a reader who already went through the latter proof, may want to skip this one).

\begin{proof}
To prove soundness, we consider several hybrid protocols, transitioning from the real system to a system where no prover cannot convince the verifier of accepting. We show that the probability that the prover convinces the verifier to accept is preserved throughout the hybrids. Since the argument is publicly verifiable, it suffices to show that the prover's view is indistinguishable between these hybrids.

\paragraph{$\hyb_0$:} This is the real protocol.

\paragraph{$\hyb_1$:} In this hybrid, $\zkVCT'$ is an encryption of $0^\secp$ instead of the target $u$. 

Since $\ins\notin\lang$, this hybrid is indistinguishable from the previous one by the semantic security of witness encryption scheme $\we$.

\paragraph{$\hyb_2$:} In this hybrid, the obfuscation $\obfC \gets \ccSim(1^\secp,1^\ell)$ is simulated rather than an obfuscation of $\CC{\fheD_{\fheK},u}$, where $\ell$ is the size of the decryption circuit $\fheD_{\fheK}$.

This hybrid is indistinguishable from the previous one by the CC simulation guarantee; indeed, in the previous hybrid, the target $u$ is uniformly random and independent of $\fheD_{\fheK}$, and the rest of the experiment. 

\paragraph{$\hyb_3$:} In this hybrid, $\zkVCT$ is an encryption of $0^\secp$ instead of the commitment randomness $r$.

This hybrid is indistinguishable from the previous one by the semantic security of the FHE scheme $\fhe$.

\paragraph{$\hyb_4$:} In this hybrid, $\cmt$ is a commitment to $1$ instead of $0$.

This hybrid is indistinguishable from the previous one by hiding of the commitment.

\medskip\noindent
It is left to show that in $\hyb_4$, no malicious prover can convince the verifier to accept a false statement $\ins \notin\lang$, except with negligible probability.  

Observe that in this hybrid:
\begin{itemize}
\item
$\ins\notin \lang$.
\item
$\cmt \in \COM(1)$, and by perfect binding there does not exist $r$ such that $\cmt = \COM(0;r)$.
\item
By the CC simulation guarantee, except with negligible probability $2^{-\secp}$, there does not exist $\evciph$ such that $\obfC(\evciph) = 1$.
\end{itemize}
Overall we deduce that, with overwhelming probability $1-2^{-\secp}$, the statement $\Psi(\ins,\cmt,\obfC)$ is false. By the soundness of the $\WI$ argument, the prover cannot cheat in this hybrid except with negligible probability.   
\end{proof}

\begin{proposition}
\proref{fig:pubv_prot} is witness hiding against explainable verifiers.
\end{proposition}

\begin{proof}
\nir{add details}
We describe the witness-finding reduction $\zkR$. 

\medskip
\paragraph{$\zkR(\ins,\zkmV_\secp,1^{1/\varepsilon})$:}
\begin{itemize}

\item 
Obtain $(\wi_1,\cmt,\zkVCT,\obfC, \zkVCT')$ from $\zkmV_\secp$.
\item
Construct the ({\em homomorphic simulation}) circuit $\HC(r)$ that given an input $r$:
\begin{itemize}
\item
Sample a second $\WI$ message $\wi_2$ for the statement $\Psi(\ins,\cmt,\obfC)$, using as the witness the randomness $r$ attesting that $\cmt=\COM(0;r)$.
\item
Feed $\wi_2$ to $\zkmV_\secp$ and obtain a candidate witness $\tilde \wit$.
\item 
Apply the witness decryptor
$$
\tilde u \gets \weD_{\tilde \wit}(\zkVCT')\enspace,
$$
and output $\tilde u$.
\end{itemize}
All randomness required by the above is hardwired to $\HC$.
\item
Compute $\evciph = \fheEv(\HC,\zkVCT)$.

\item
If $\obfC(\evciph)=1$, repeat the following at most $1/\varepsilon$ times:
\begin{itemize}
\item
Sample a second $\WI$ message $\wi_2$ for the statement $\Psi(\ins,\cmt,\obfC)$, using as the witness $\evciph$ attesting that $\obfC(\evciph)=1$, feed it to $\zkmV_\secp$. \item
If $\zkmV_\secp$ outputs a witness $\wit\in\RL(\ins)$, output $\wit$.
\end{itemize}
\item
Otherwise, output $\bot$.
\end{itemize}


\paragraph{Reduction validity.} 
The reduction clearly runs in polynomial time. We now prove its validity for always-explainable verifiers (which is w.l.o.g, \remref{rem:aev}). Let $\zkmV=\set{\zkmV_\secp}_\secp$ be any always-explainable polynomial-size verifier. Fix any $\secp$, and $x\in \lang\cap\zo^\secp$, and assume that $\zkmV_\secp$ outputs a witness $\wit\in \RL(\ins)$ with probability $\delta$.
 
Let $r$ be the randomness underlying the commitment $\cmt = \COM(0;r)$ given by $\zkmV_\secp$. We argue that the circuit $\HC(r)$ outputs the target $u$ underlying the CC obfuscation $\obfC$ with probability $\delta-\secp^{-\omega(1)}$, over its own coins. First, we argue that when $\HC$ gives $\zkmV_\secp$ the second \WI message $\wi_2$, $\zkmV_\secp$ outputs a witness $\wit$ with probability $\delta-\secp^{-\omega(1)}$. Otherwise, we can construct a verifier $\wimV$ that breaks witness indistinguishability. The verifier $\wimV_\secp$ has the witness $r$ non-uniformly hardwired. It obtains $\zkmV_\secp$'s message, and gives the challenger the $\WI$ first message $\wi_1$ generated by $\zkmV_\secp$, along with the statement $\Psi$, and two witnesses $\wit_0 =\wit$ and $\wit_1 = r$, when it receives $\wi_2$, it uses it to complete the emulation of $\zkmV_\secp$. It then check if $\zkmV_\secp$ outputs a witness for $\ins$, if it does $\wimV_\secp$ outputs $0$, and otherwise outputs $1$. By construction the advantage of $\wimV$ is exactly the difference between the probabilities of outputting a witness. 

Next, note that whenever the verifier $\zkmV$ outputs a witness (under the encryption), the witness decryption operation performed by $\HC$, will indeed result in the target $u$. 

By the correctness of $\fhe$, the ciphertext $\evciph=\fheEv(\HC,\evciph)$ obtained by the reduction satisfies:
$$
\fheD_{\fheK}(\evciph) = u\enspace,
$$
and thus by the one-sided correctness of the CC obfuscator $\O$,
$$
\obfC(\evciph) = 1\enspace.
$$
It follows that in this case, except with negligible probability $\secp^{-\omega(1)}$, the reduction obtains a valid witness $\evciph$ for the statement $\Psi$. By witness indistinguishability given the second \WI message $\wi_2$, using $\evciph$ as the witness, $\zkmV_\secp$ outputs a witness with probability $\delta-\secp^{-\omega(1)}$. Otherwise, we can again construct $\wimV$ that will break witness indistinguishability similarly to the previous reduction, but now using the (non-uniformly hardwired) $\evchiph$. By Markov's inequality, in this case, the reduction (which makes $1/\varepsilon$ attempts), obtains a witness with probability at least $1- \frac{\varepsilon}{\delta} -\secp^{-\omega(1)}$.

Overall, the reduction obtains a witness with probability at least
$$\(\delta-\secp^{-\omega(1)}\)\cdot \(1- \frac{\varepsilon}{\delta} -\secp^{-\omega(1)}\) =\delta-\varepsilon-\secp^{-\omega(1)}\enspace,
$$
as required.
\end{proof}


\section{From Explainable Verifiers to Malicious Ones}

In this section, we present three generic transformations that compile protocols that 
are private (according to some natural notion, such as ZK, WZK, WH) against explainable verifiers into ones that satisfy the same privacy guarantee against malicious verifiers.

This includes the following:
\begin{itemize}
\item
A 3-message transformation that preserves \WZK (or $\ZK$), based on polynomial hardness assumptions. 
\item
A 2-message transformation that preserves \WZK, based on super-polynomial hardness assumptions.
\item
A 2-message transformation that preserves WH, based on polynomial witness encryption. 
\end{itemize}

\subsection{The Three-Message Transformation}

We provide a transformation that compiles any 3-message \WZK protocol against explainable verifiers into one against malicious verifiers.  
% We also show that under additional (standard) assumptions, we can remove the semi-black-box requirement. This variant of the transformation can also be applied for \ZK, rather than \WZK, protocols.

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
 A 2-message $\WI$ argument for \NP with delayed input $(\wiP,\wiV)$. We denote its messages by $(\wi_1,\wi_2)$.

\item
  A non-interactive dense commitment scheme $\COM$. 
\item
 A $3$-message argument system $\prot{\zkP}{\zkV}$ for an $\NP$ language $\lang$ that is \WZK against explainable verifiers. We denote its messages by $(\pmes_1,\vmes_2,\pmes_3)$.
 \end{itemize}
%
We describe the protocol in \figref{fig:sm_to_m_prot}.

\protocol
{\proref{fig:sm_to_m_prot}}
{A \WZK argument $\prot{\bar \zkP}{\bar \zkV}$ for $\NP$ against malicious verifiers.}
{fig:sm_to_m_prot}
{
\begin{description}
    \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\bar \zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
\end{description}

\begin{enumerate}
\item
$\bar \zkP$ computes
\begin{itemize}
\item
$\pmes_1$, the first message in the original protocol.
\item
$\cmt \gets \COM(\wit)$ a commitment to the witness.
\item
$\wi_1$, the first message of a $\WI$ argument.
\end{itemize}
It sends $(\pmes_1,\cmt,\wi_1)$.
\item
$\bar \zkV$ computes
\begin{itemize}
\item
$\vmes_2$, the second message in the original protocol.
\item
$\wi_2$, the second \WI message for the statement $\Phi(\ins,\cmt,\pmes_1,\vmes_2)$:
\begin{align*}
&\exists r \; : \; \vmes_2 = \zkV(\ins,\pmes_1;r)
\hspace{2mm} \bigvee \hspace{2mm} \exists r,s \; : \; \cmt = \COM(s;r), s \notin \RL(\ins)\enspace.
\end{align*}
\end{itemize}
It sends $(\vmes_2,\wi_2)$.
\item 
$\bar \zkP$ verifies the $\WI$ argument $(\wi_1,\wi_2)$ for the statement $\Phi$, and aborts if it does not accept. 

It then computes $\pmes_3$, the third message in the original protocol, and sends it.

 \item
    $\bar \zkV$ verifies the argument $(\pmes_1,\vmes_2,\pmes_3)$.
\end{enumerate}
}

\paragraph{Analysis.} We now analyze the transformation.

\begin{proposition}
\proref{fig:sm_to_m_prot} is sound.
\end{proposition}

\begin{proof}
To prove soundness, we show how to transform any cheating prover $\zkbmP$ against \proref{fig:sm_to_m_prot} into a cheating prover $\zkmP$ against the original protocol. 

Fix any polynomial-size prover $\zkbmP = \set{\zkbmP_\secp}_\secp$. We describe a new prover $\zkmP=\set{\zkmP_\secp}_\secp$, and show that for any $\ins \in \zo^\secp\setminus\lang$, if $\zkbmP_\secp$ convinces $\bar \zkV$ to accept with probability $\varepsilon$, the new prover convinces $\zkmP$ convinces $\zkV$ to accept with probability $\varepsilon-\secp^{-\omega(1)}$. For this, consider the first message $(\pmes_1,\cmt,\wi_1)$ sent by $\zkbmP_\secp$. Since the commitment $\COM$ is dense, there exists an underlying string $s$ and randomness $r$, such that $\cmt=\COM(s;r)$. The constructed $\zkmP_\secp$ will have $(s,r)$ non-uniformly hardwired into its code, and will operate as follows.

\paragraph{$\zkmP_\secp$:}
\begin{itemize}
\item
It sends $\pmes_1$ to $\zkV$, and obtains $\vmes_2$.
\item
It  computes the argument message $\wi_2$ for $\Phi(\ins,\cmt,\pmes_1,\vmes_2)$ using the witness $(r,s)$.
\item
It then feeds $(\vmes_2,\wi_2)$ to $\zkbmP_\secp$, and obtains back $\pmes_3$. It sends $\pmes_3$ to $\zkV$.
\end{itemize}

\paragraph{Prover analysis.} $\zkmP$ is clearly of polynomial size. We now analyze its cheating probability. 
First, note that since $\ins \notin \lang$, it necessarily holds that $s\notin \RL(\ins)$, and accordingly $(r,s)$ is also a valid witness for any statment $\Phi(\ins,\cmt \arg_1,\arg_2)$, regardless of $\arg_2$.

Next, observe that the only difference between the view of $\zkbmP$ in a real interaction with $\bar \zkV$ and its view as emulated by $\zkmP$ is that in the first, the \WI argument $(\wi_1,\wi_2)$ is computed using  the randomness of the honest verifier $\zkV$ as the witness, whereas in the second it is computed using the witness $(r,s)$.

By the witness indistinguishability of the argument, it follows that $\zkmP$ convinces $\zkV$ with the same probability $\varepsilon$ that $\zkbmP$ convinces $\bar \zkV$, up to a negligible difference.  
\end{proof}

\begin{proposition}
Assume that the original protocol $\prot{\zkP}{\zkV}$ is \WZK against explainable verifiers, then \proref{fig:sm_to_m_prot} is \WZK.
\end{proposition}

\begin{proof}
 Fix any polynomial-size (malicious) verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ against
\proref{fig:sm_to_m_prot} and a polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_\secp$ . To prove that the  protocol is $\WZK$, we first prove that $\zkbmV$ can be converted into an explainable verifier against the original protocol, which is given as auxiliary input a commitment to the witness.
\begin{claim}\label{clm:exp_sim}
There exists a $\PPT$ simulator $\zkE$ such that:
\begin{itemize}
\item
$\zkmV=\set{\zkmV_{\ins,\cmt} := \zkE^{\zkbmV_\secp}(\ins,\cmt)}_{\ins,\cmt}$ is an explainable verifier against the original protocol $\prot{\zkP}{\zkV}$ for all $\ins\in \lang\cap\zo^\secp$, $\wit\in\RL(\ins)$, and $\cmt\in \COM(\wit)$.
\item
For any $\secp\in \Nat$, $\ins\in\lang \cap \zo^\secp$, and $\wit\in\RL(\ins)$,  
$$
\view_{\zkbmV_\secp}\prot{\zkP(\wit)}{\zkbmV_\secp}(\ins) \equiv \view_{\zkmV_{\ins,\cmt}}\prot{\zkP(\wit)}{\zkmV_{\ins,\cmt}}(\ins) \enspace,
$$
where  $\cmt\gets \COM(\wit)$.
\end{itemize}
\end{claim}

\noindent
Before proving the claim let us show that it implies that the protocol is $\WZK$. For this purpose, we describe the corresponding $\WZK$ simulator.

\paragraph{$\zkbS(\ins,\zkbmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
\begin{itemize}
\item
Sample a commitment of zero $\cmt \gets \COM(0^{|\wit|})$.
\item
Construct the verifier $\zkmV_{\ins,\cmt} := \zkE^{\zkbmV_\secp}(\ins,\cmt)$.
\item
Output $\zkS(\ins,\zkmV_{\ins,\cmt},1^{1/\varepsilon})$, where $\zkS$ is the simulator of the original protocol $\prot{\zkP}{\zkV}$.
\end{itemize}
%
To prove the validity of $\zkbS$, we consider an alternative $\zkbS_\wit$ that acts similarly, except that it samples a commitment of the witness $\cmt \gets \COM(\wit)$, rather than a commitment of zero.  
Then by the hiding of the commitment 
$$\zkbS(\ins,\zkbmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) \hspace{2mm} \approx_{\zkmD_\secp,\secp^{-\omega(1)}}\hspace{2mm} \zkbS_\wit(\ins,\zkbmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace.
$$
Furthermore, by construction 
$$\zkbS_\wit(\ins,\zkbmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) \equiv \zkS(\ins,\zkbV_{\ins,\cmt},\zkmD_\secp,1^{1/\varepsilon}) \enspace,
$$
where $\cmt\gets \COM(\wit)$. By the first part of \clmref{clm:exp_sim}, the corresponding verifier $\zkbV_{\ins,\cmt}$ is explainable, and thus by the \WZK guarantee of the original protocol $\prot{\zkP}{\zkV}$, 
$$
\zkS(\ins,\zkbV_{\ins,\cmt},\zkmD_\secp,1^{1/\varepsilon}) 
\approx_{\zkmD_\secp,\varepsilon+\secp^{-\omega(1)}}
\view_{\zkmV_{\ins,\cmt}}\prot{\zkP(\wit)}{\zkmV_{\ins,\cmt}}(\ins)
\enspace.
$$
By the second part of \clmref{clm:exp_sim},
we deduce
$$\zkbS(\ins,\zkbmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) \approx_{\zkmD_\secp,\varepsilon+\secp^{-\omega(1)}}  \view_{\zkbmV_\secp}\prot{\zkP(\wit)}{\zkbmV_\secp}(\ins)
\enspace,
$$
as required.

\begin{proof}[Proof of \clmref{clm:exp_sim}]

We describe the explainable simulator $\zkE$.

\paragraph{$\zkmV_{\ins,\cmt} := \zkE^{\zkbmV_\secp}(\ins,\cmt)$:}

\begin{itemize}
    \item 
    Given prover message $\pmes_1$ from $\zkP$, sample a first $\WI$ message $\wi_1$, feed $(\pmes_1,\cmt,\wi_1)$ to $\zkbmV_\secp$, and obtain its message $(\arg_2,\wi_2)$.
    
    \item
    Verify the $\WI$ argument $(\wi_1,\wi_2)$ for the statement $\Phi(\ins,\cmt,\pmes_1,\cmes_2)$. \item
    If verification does not pass, emulate an abort:
    \begin{itemize}
        \item Send $\zkP$ message $\bot$.
        \item Feed $\zkbmV_\secp$ with a message $\bot$ (emulating an abort of $\zkbP$), and output whatever $\zkbmV_\secp$ does.
    \end{itemize}
    \item
    Otherwise, send $\arg_2$ to $\zkP$, obtain $\pmes_3$, feed it to $\zkbmV_\secp$, and output whatever $\zkbmV_\secp$ does.
\end{itemize}
%
First, by the construction of $\zkE$, for any $\secp\in \Nat$, $\ins\in\lang \cap \zo^\secp$, and $\wit\in\RL(\ins)$,  
$$
\view_{\zkbmV_\secp}\prot{\zkP(\wit)}{\zkbmV_\secp}(\ins) \equiv \view_{\zkmV_{\ins,\cmt}}\prot{\zkP(\wit)}{\zkmV_{\ins,\cmt}}(\ins) \enspace.
$$
We now prove that $\zkmV=\set{\zkmV_{\ins,\cmt} := \zkE^{\zkbmV_\secp}(\ins,\cmt)}_{\ins,\cmt}$ is explainable for all $\ins\in \lang\cap\zo^\secp$, $\wit\in\RL(\ins)$, and $\cmt\in \COM(\wit)$.

Assume toward contradiction that when interacting with $\zkP$, $\zkmV_\secp$ outputs a message that is not explainable with noticeable probability $\delta(\secp)$. We use $\zkmV$ to construct a prover $\wimP$ that breaks the soundness of the $\WI$ argument. Given a first \WI message $\wi_1$, $\wimP_\secp$ emulates $\zkmV_\secp$, but replaces the message $\wi_1$ that $\zkmV_\secp$ generates with the one received from the challenger. It then obtains from the emulated $\zkmV_\secp$, the statement $\Phi(\ins,\cmt,\pmes_1,\pmes_2)$ and second $\WI$ message $\wi_2$, it returns $(\Phi,\wi_2)$ to the challenger. By construction and the assumption that $\zkmV_\secp$'s message is not explainable with probability $\delta$, $\wimP$ breaks soundness with probability exactly $\delta$.

This completes the proof of the claim.
\end{proof}
\end{proof}

\begin{remark}[Zero knowledge]
We note that the above transformation holds just the same for $\ZK$ --- the constructed explainable verifier $\zkmV$ only depends on the malicious verifier $\zkbmV$, and not on the distinguisher.
\end{remark}

\subsection{The Two-Message Transformation}

We provide a transformation that compiles any 2-message \WZK protocol against explainable verifiers with soundness against quasipolynomial provers (like the one from \secref{sec:2wzk_expl}) into one against malicious verifiers.

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
 A 2-message $\WI$ argument for \NP with delayed input with a quasipolynomial witness extractor $\prot{\wiP}{(\wiV_1,\wiV_2)}$. We denote its messages by $(\wi_1,\wi_2)$.
\item
A conditional disclosure of secrets scheme $(\cdsR,\cdsS,\cdsD)$ for $\NP$, with receiver simulation security against quasi-polynomial time senders.
\item
 A $2$-message argument system $\prot{\zkP}{\zkV}$ for an $\NP$ language $\lang$ that is \WZK against explainable verifiers and sound against quasipolynomial provers. We denote its messages by $(\vmes_1,\pmes_2)$.
 \end{itemize}
%
We describe the protocol in \figref{fig:sm_to_m_prot2}.

\protocol
{\proref{fig:sm_to_m_prot2}}
{A \WZK argument $\prot{\bar \zkP}{\bar \zkV}$ for $\NP$ against malicious verifiers.}
{fig:sm_to_m_prot2}
{
\begin{description}
    \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\bar \zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
\end{description}
\begin{enumerate}

\item
$\bar \zkV$ computes
\begin{itemize}
\item
$(\wi_1,\tau_\zkV) \gets \wiV_1(1^\secp)$, the first \WI message.
\item
$\vmes_1$, the verifier message in the original protocol $\prot{\zkP}{\zkV}(\ins)$. It stores the randomness $r$ used by the verier to generate the message.
\item
$(\cdsRCT,\cdsK) \gets \cdsR(\Psi,r)$, a CDS receiver message for the statement $\Psi(\vmes_1)$ attesting that $\vmes_1$ was computed according to the honest verifier $\zkV$, using $r$ as the witness.
\end{itemize}
It sends $(\wi_1,\vmes_1,\cdsRCT)$.
\item 
$\bar \zkP$ computes
\begin{itemize}
\item
$\pmes_2$, the prover message in the original protocol $\prot{\zkP}{\zkV}$.
\item
$\cdsSCT\gets \cdsS(\Psi,\pmes_2,\cdsRCT)$, a CDS sender message encrypting $\pmes_2$.
\item
$\wi_2 \gets \wiP(\Phi,\pmes_2,\wi_1)$, the second \WI message for the statement 
\begin{align*}
\Phi(\ins,\Psi,\cdsSCT,\cdsRCT):= \hspace{2mm} \exists \pmes \; : \; \cdsSCT \in \cdsS(\Psi,\pmes,\cdsRCT) \hspace{2mm}\bigvee\hspace{2mm} \ins\in \lang\enspace.
\end{align*}
\end{itemize}
It sends $(\cdsSCT, \wi_2)$.
 
 \item
    $\bar \zkV$ then
    \begin{itemize}
    \item
    Runs $\wiV_2(\Phi,\wi_1,\wi_2;\tau_\zkV)$ to verify the $\WI$ argument for the statement $\Phi$.
    \item
    Decrypts $\widetilde \pmes_2 \gets \cdsD_\cdsK(\cdsSCT)$.
    \item
    Verifies the original argument $(\vmes_1,\widetilde \pmes_2)$.
    \end{itemize}
\end{enumerate}
}

\paragraph{Analysis.} We now analyze the transformation.

\begin{proposition}
\proref{fig:sm_to_m_prot2} is sound.
\end{proposition}
\begin{proof}
To prove soundness, we transform any cheating prover $\zkbmP$ against \proref{fig:sm_to_m_prot2} into a quasi-polynomial cheating prover $\zkmP$ against the original protocol $\prot{\zkP}{\zkV}$. We describe $\zkmP$.

\paragraph{${\zkmP_\secp}$:}
\begin{itemize}
\item
Obtain the first message $\vmes_1$ from the verifier $\zkV$.
\item
Simulate the CDS receiver first message $\cdsRCT = \cdsSim(\Psi)$, relative to the statement $\Psi(\vmes_1)$ attesting that $\vmes_1$ is honest.
% \item
% Construct from $\zkbmP_\secp$ a prover for the \WI argument of knowledge $\zkmP_{\wi}$ that has $\vmes_1, \cdsRCT$ hardwired and works as follows:
% \begin{itemize}
% \item
% Given $\wi_1$ from the $\WI$ verifier, it feeds $(\wi_1,\vmes_1,\cdsRCT)$ to $\zkbmP$.
% \item
% It obtains $(\cdsSCT,\wi_2)$, and sends $\wi_2$ as the second message.
% \end{itemize}
\item 
Sample a first $\WI$ message $\wi_1$, feed $(\wi_1,\vmes_1,\cdsRCT)$ to $\zkbmP_\secp$, and obtain $(\cdsSCT,\wi_2)$.
\item
Apply the quasipolynomial witness extractor $\pmes_2 \gets \zkE(\Phi,\wi_1,\wi_2)$ for the statement $\Phi(x, \pmes_1, \cdsSCT,\cdsRCT)$.
\item
Send the extracted $\pmes_2$ to $\zkV$.
\end{itemize}

\paragraph{Prover analysis.} Fix any polynomial-size prover $\zkbmP=\{\zkbmP_\lambda\}_{\lambda}$. First note that the corresponding new prover $\zkmP$ runs in quasipolynomial time. We show that for any $x \not \in \mathcal{L}$, if $\zkbmP_\secp$ convinces $\zkbV$ to accept with noticeable probability $\varepsilon(\secp)$, the new prover $\zkmP_\secp$ convinces $\zkV$ to accept with probability $\varepsilon - \secp^{-\omega(1)}$.

First, we consider a hybrid experiment where the prover strategy $\zktmP$ is identical to that of ${\zkmP}$, except that
instead of sampling a simulated CDS receiver message $\cdsRCT \gets  \cdsSim(\Psi)$ for the statement $\Psi(\vmes_1)$, $\zktmP$ obtains externally a CDS message $\cdsRCT \gets  \cdsR(\Psi,r)$ corresponding to the randomness used by $\zkV$ to sample $\vmes_1$. ($\zktmP$ then uses $\cdsRCT$ like $\zkmP$). 

\begin{claim}
$\zktmP$ convinces $\zkV$ with the same probability as $\zkmP$ does, up to a negligible difference. 
\end{claim}

\begin{proof}
Otherwise, we can use $\zktmP$ to construct a quasipolynomial distinguisher $\zkmD$ that breaks the receiver simulation property. $\zkmD_\secp$ emulates an interaction between $\zktmP_\secp$ and $\zkV$. It then submits $\Psi(\vmes_1)$ and $r$ to a challenger, where $\vmes_1$ is the message generated by $\zkmV$ using randomness $r$. It receives back $\cdsRCT$, and completes the emulation. It is left to note that if $\cdsRCT \gets \cdsSim(\Psi)$, then the view of $\zkV$ is distributed as in an interaction with $\zkmP_\secp$, whereas if $\cdsRCT\gets \cdsS(\Psi,r)$, the view is distributed as in an interaction with $\zktmP_\secp$.  
\end{proof}

From hereon we focus on proving that $\zktmP$ convinces $\zkV$ of accepting with probability $\varepsilon-\secp^{-\omega(1)}$. Let $\arg_1$ be the message received from $\zkV$, let $\cdsSCT$ be sender encryption emulated by $\zktmP_\secp$, let $\pmes_2$ be the prover message that $\zktmP_\secp$ extracts from $\zkbmP_\secp$, and let $\widetilde{\pmes}_2 =\cdsD_{\cdsK}(\cdsSCT)$ be the decrypted message with respect to the secret key $\cdsK$ produced when generating the receiver message $\cdsRCT$. Also let $(\wi_1,\wi_2)$ be the \WI argument for the statement  $\Phi(\ins,\Psi,\cdsRCT,\cdsSCT)$ generated by $
\zkbmP_\secp$ during its emulation by $\zktmP_\secp$. 

\begin{claim}\label{clm:zktmP}
With probability at least $\varepsilon-\secp^{-\omega(1)}$,
\begin{enumerate}
    \item 
    $\zkV$ accepts $(\vmes_1,\widetilde{\pmes}_2)$.
    \item
    $\widetilde{\pmes}_2 = \pmes_2$.
\end{enumerate}
\end{claim}

This implies that that $\zktmP$, who sends $\pmes_2$, convinces $\zkV$ with probability at least $\varepsilon-\secp^{-\omega(1)}$, as required and would complete the proof.

\begin{proof}[Proof of \clmref{clm:zktmP}]
By construction, an interaction between $\zktmP$ and $\zkV$ perfectly emulates an interaction between $\zkbmP$ and $\zkbV$. In such an interaction the verifier $\zkbV$ both accepts the \WI argument $(\wi_1,\wi_2)$ for $\Phi(\ins,\Psi,\cdsRCT,\cdsSCT)$ and accepts the underlying $(\pmes_1,\widetilde{\pmes}_2)$. Since $\ins\notin \lang$, it follows by the extraction guarantee, that except with negligible probability $\secp^{-\omega(1)}$, $\cdsSCT$ is a valid CDS encryption of $\pmes_2$. Furthermore, by CDS correctness, it holds that $\widetilde{\pmes}_2 = \cdsD_\cdsK(\cdsSCT) = \pmes_2$.
\end{proof}

This completes the proof of sounenss.


% By the AoK guarantee, in the extraction phase, 
% $\zkmP$ outputs a witness for $\wi$ with probability $1 - \mathsf{negl}(\lambda)$.
% Since $x \not \in \mathcal{L}$, this witness corresponds to $\arg_2$, the opening of $\cdsS$.
% We now analyze the probability that $(\vmes_1, \pmes_2)$ is an accepting transcript of the original protocol. 

% First, we consider a hybrid experiment $\widehat{\zkmP}$ where the prover strategy is identical to that of ${\zkmP}$, except that $\widehat{\zkmP}$ additionally obtains the randomness $r$ that is used to compute message $\vmes_1$. 
% $\widehat{\zkmP}$ then computes $\cdsRCT = \cdsR(\vmes_1, r)$, and carries out the rest of the experiment identically to $\zkmP$.
% In this experiment, if $\wiV$ outputs accept, 
% then by soundness of $\wi$, since $x \not \in \mathcal{L}$, $\widehat{\zkmP}$ outputs $\widehat{\pmes}_2$ that corresponds to the opening of $\cdsS$. 
% Furthermore, since $\zkbmP$ breaks soundness, this implies that $(\arg_1, \widehat{\pmes}_2)$ is an accepting transcript of the original protocol with probability $\epsilon - \mathsf{negl}(\lambda)$.

% By security of $\cds$ against quasi-polynomial senders, the joint distribution $(\arg_1, \widehat{\arg}_2)$ output by $\widehat{\zkmP}$ remains indistinguishable from the joint distribution $(\arg_1, \arg_2)$ output by $\zkmP$.
% Indeed otherwise, a reduction that generates $\arg_1$ with randomness $r$, then obtains $\cdsRCT$ externally as either a commitment to $0$ or a commitment to $r$, can break semantic security of $\cdsRCT$ based on whether it obtained $\arg_2$ or $\widehat{\arg}_2$.

% Therefore, $(\arg_1, \arg_2)$ is an accepting transcript of the original protocol with probability $\epsilon - \mathsf{negl}(\lambda)$, which is a contradiction, as desired.
\end{proof}

\begin{proposition}
\proref{fig:sm_to_m_prot2} is weak zero-knowledge against malicious verifiers.
%There exists a $\PPT$ simulator $\zkS$ such that for any polynomial-size (malicious) verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ against \proref{fig:sm_to_m_prot}:
%\begin{itemize}
%\item
%$\zkmV := \zkS^{\zkbmV}$ is an explainable verifier against the original protocol $\prot{\zkP}{\zkV}$.
%\item
%For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_\secp$ there exists a negligible $\mu$ such that for any $\secp\in \Nat$ and any $\ins\in\lang \cap \zo^\secp$,
%$$
%\view_{\zkbmV}\prot{\zkP(\wit)}{\zkbmV}(\ins) \approx_{\zkmD_\secp,\mu} \view_{\zkmV}\prot{\zkP(\wit)}{\zkmV}(\ins) \enspace.
%$$
%\end{itemize}
\end{proposition}


\begin{proof}
We describe a simulator $\zkbS$. Throughout, we assume w.l.o.g that the simulated verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ is deterministic and always outputs the prover message it receives (\remref{rem:random}). 

% It relies on the simulator $\zkS$ of the original protocol in order to simulate the view of $\zkmV$ against $\zkmD_\secp$.

\paragraph{$\zkbS(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon})$:}
\begin{itemize}
    \item Obtain $(\wi_1, \vmes_1, \cdsRCT)$ from $\zkbmV_\secp$.
    \item
    Construct a new verifier $\zkmV_\secp$ that sends $\vmes_1$ as its first message, and given $\pmes_2$ from $\zkP$, outputs it.
    \item
    Construct a new distinguisher $\zkmD_\secp$ that given $\pmes_2$ from $\zkP$: 
    \begin{itemize}
        \item
            Samples $\cdsSCT \gets \cdsS(\Psi,\pmes_2,\cdsRCT)$, an encryption of $\pmes_2$ under $\Psi(\vmes_1)$.
            \item
            Samples $\wi_2\gets \wiP(\Phi,(\pmes_2,r_\cds),\wi_1)$, a second \WI message  for the statement $\Phi(\ins,\Psi,\cdsRCT,\cdsSCT)$, using as the witness the message $\pmes_2$ and randomness $r_\cds$ used for generating $\cdsSCT$.
            \item
            Runs $\zkbmD_\secp(\cdsSCT,\wi_2)$.
        \end{itemize}
        \item
        Obtain $\widetilde{\pmes}_2\gets \zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$, where $\zkS$ is the simulator for the protocol $\prot{\zkP}{\zkV}$.
        \item
        Compute a CDS encryption $\cdstSCT \gets \cdsS(\Psi,\widetilde{\pmes}_2,\cdsRCT)$.
        \item
            Compute a second \WI message $\widetilde{\wi}_2\gets \wiP(\Phi,(\widetilde{\pmes}_2,\tilde r_\cds),\wi_1)$, using as the witness the message $\widetilde{\pmes}_2$ and randomness $\tilde r_\cds$ used for generating $\cdstSCT$.
            \item
            Output $(\cdstSCT,\widetilde{\wi}_2)$.
    \end{itemize}

    


\paragraph{Simulator analysis.}
The simulator $\zkbS$ clearly runs in polynomial time. We now prove its validity.

Assume toward contradiction that there exist polynomial-size distinguisher $\zkbmD=\set{\zkbmD_\secp}_\secp$ and verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ that for infinitely many $\ins \in \lang$ and $\wit\in\RL(\ins)$ distinguishes $\zkbS(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon})$ from $\view_{\zkbmV_\secp}\prot{\zkbmP(\wit)}{\zkbmV_\secp}(\ins)$ with advantage $\varepsilon(\secp)+\delta(\secp)$ for noticeable $\varepsilon,\delta$. We consider two cases.

\paragraph{Case 1:} There exists a set $H$ of infinitely many $\ins$ as above such that the verifier's message $\vmes_1$ is in the support of the honest verifier's messages. We show that this contradicts \WZK against explainable verifiers. 

By the \WZK guarantee of $\prot{\zkP}{\zkV}$ against explainable verifiers, there exists a negligible $\mu(\secp)$ such that for any $\ins\in H\cap\zo^\secp$, 
\begin{align*}
\zkmD_\secp(\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)) \approx_{\varepsilon+\secp^{-\omega(1)}} \zkmD_\secp(\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon}))\enspace.
\end{align*}
%
Furthermore, by the definition of $\zkbS,\zkmD$, for any such $\ins$, 
\begin{align*} 
\zkmD_\secp(\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon}))\equiv \zkbmD_\secp(\zkbS(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon}))\enspace.     
\end{align*}
%
Finally, by the definition of $\zkmD,\zkmV,\zkP$, for any such $\ins$, 
\begin{align*} 
\zkbmD_\secp(\view_{\zkbmV_\secp}\prot{\zkbP(\wit)}{\zkbmV_\secp}(\ins)) \equiv \zkmD_\secp(\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins))\enspace.
\end{align*}
It follows that for any $\ins\in H\cap\zo^\secp$, 
\begin{align*}
\view_{\zkbmV_\secp}\prot{\zkbP(\wit)}{\zkbmV_\secp}(\ins)
\approx_{\zkbmD_\secp,\varepsilon+\secp^{-\omega(1)}}
\zkbS(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon})
\enspace.
\end{align*}
%
This disproves Case 1.

\paragraph{Case 2:} There exists a set $M$ of infinitely many $\ins$ as above such that the verifier's message $\vmes_1$ is malicious (not in the support of the honest verifier's messages). We show how to use $\zkbmV,\zkvmD,\zkbmS$ to break the CDS message hiding. First we consider an alternative simulator $\zkbmS'$ that has the witness $\wit\in\RL(\ins)$ hardwired. It computes $\widetilde{\wi_2}$ in the simulation using the witness $\wit$ instead of using as the witness $\widetilde{\pmes_2},\tilde r_\cds$. Similarly, we consider an alternative prover $\zkbP'$, which computes its own message $\wi_2$ using $\wit$ instead of $\pmes_2$ and $r_\cds$. By witness indistinguishability:
\begin{align*}
\view_{\zkbmV_\secp}\prot{\zkbP'(\wit)}{\zkbmV_\secp}(\ins)
&\approx_{\zkbmD_\secp,\secp^{-\omega(1)}}
\view_{\zkbmV_\secp}\prot{\zkbP(\wit)}{\zkbmV_\secp}(\ins)\\
\zkbS'(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon})
&\approx_{\zkbmD_\secp,\secp^{-\omega(1)}}
\zkbS(\ins,\zkbmV_\secp,\zkbmD_\secp,1^{1/\varepsilon})
\enspace.
\end{align*}
Thus $\zkbmD$ distinguishes the view $(\cdsS(\Psi,\widetilde{\pmes}_2,\cdsRCT)), \widetilde{\wi}_2(\wit)$ generated by $\zkbS'$ from $(\cdsS(\Psi,{\pmes}_2,\cdsRCT)), {\wi}_2(\wit)$ generated by $\zkP'$ with advantage $\varepsilon+\delta-\secp^{-\omega(1)}$. However, since the verfier's message is malicious $\Psi(\vmes_1)$ is false. Thus in this case we obtain a distinguisher against the CDS message hiding.

This completes the proof of the proposition.
\end{proof}


% \begin{proof}
% We describe the simulator $\zkbS$ that is as input the instance $\ins$, verifier $\zkmV_\secp$, distinguisher $\zkmD_\secp$ and error parameter $\varepsilon$. 

% % It relies on the simulator $\zkS$ of the original protocol in order to simulate the view of $\zkmV$ against $\zkmD_\secp$.

% \paragraph{$$\zkbS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
% \begin{itemize}
%     \item Obtains $\wi_1, \vmes_1, \cdsRCT$ from $\zkmV$. 
%     \item Computes distinguisher $\zkmD'_\secp$ that on input $(z', \vmes'_1, \pmes'_2)$,
%     \begin{itemize}
%         \item Parses $z' = (z, \wi_1, \vmes_1, \cdsRCT)$.
%         \item Computes $\cdsSCT.{\mathsf{Sim}} \gets \cdsS(\Psi, \pmes'_2, \cdsRCT)$.
%         \item Computes $\wi_{2,\mathsf{Sim}} \gets \wiP(\Phi, \pmes'_2, \wi_1)$, the second WI message for the statement
%         $$\Phi(x, \Psi, \cdsSCT.{\mathsf{Sim}}, \cdsRCT) := \exists \arg: \cdsSCT.\mathsf{Sim}(\Psi, \arg, \cdsR) \bigwedge x \in \mathcal{L}.$$
%         \item Outputs $\zkmD_\secp (z, (\wi_1, \vmes'_1, \cdsRCT), (\cdsSCT.{\mathsf{Sim}}, \wi_{2, \mathsf{Sim}})).$
%     \end{itemize}
%     \item Computes ${\zkV}_x$ that outputs $\vmes'_1$ on input $x$ and $\bot$ otherwise.
%     \item Computes $\pmes_{\mathsf{Sim}} \gets \zkS^{{\zkV}_x} (x, \zkmD'_\secp, 1^{1/\epsilon})$.
%     \item Computes $\cdsSCT \gets \cdsS(\Psi, \arg_{\mathsf{Sim}}, \cdsRCT)$.
%     \item Computes $\wi_2 \gets \wiP(\Phi, \pmes_{\mathsf{Sim}}, \wi_1)$, the second WI message for the statement
%     $$\Phi(x, \Psi, \cdsSCT, \cdsRCT) := \exists \arg: \cdsSCT(\Psi, \arg, \cdsR) \bigwedge x \in \mathcal{L}.$$
%     \item Sends $(\cdsSCT, \wi_2)$.
% \end{itemize}

% \paragraph{Simulator analysis.}
% The simulator $\bar \zkS$ runs in polynomial time. 
% Next, we prove indistinguishability of real and simulated views by case analysis. Without loss of generality, it suffices to assume that $\zkmV$ is deterministic.
% Fix any $\secp$ and $x$. 
% This fixes the first message $(\vmes_1, \wi_1, \cdsRCT)$ of $\bar \zkV$.
% We have the following two cases:
% \begin{itemize}
%     \item {\bf $\vmes_1$ is in the support of honest verifier messages for the original protocol.} 
%     %\textcolor{red}{Set reference to 2 message explainable protocol.}
%     In this case, ${\zkV}_x$ is an explainable verifier.
%     Therefore, by simulation security of 
%     $\zkS^{\zkV} (x, \zkmD'_\secp, 1^{1/\epsilon})$ outputs $\pmes_{\mathsf{Sim}}$ such that 
%     $$\arg_2 \approx_{\zkmD'_\secp, \mu} \arg_{\mathsf{Sim}}$$
%     which implies
%     $$(\cdsSCT,\wi_2) \approx_{\zkmD_\secp,\epsilon+\mu} 
%     (\cdsSCT.\mathsf{Sim},\wi_{2, {\mathsf{Sim}}}).$$
%     \item {\bf $\vmes_1$ is not in the support of honest verifier messages for the original protocol.} 
%     This implies that $\nexists r$ such that $\cdsRCT, k = \cdsR(\Psi, r)$.
%     In this case, by message indistinguishability of $\cds$, we have
%     $$(\cdsSCT,\wi_2) \approx (\cdsSCT.\mathsf{Sim},\wi_{2, {\mathsf{Sim}}}).$$
% \end{itemize}
% Therefore, for any polynomial-size distinguisher $ \{\zkmD_\secp\}_{\secp}$, there exists a negligible $\mu$ such that for any $\secp \in \mathbb{N}$ and any $x \in \mathcal{L} \cap \zo^\secp$,
% $$\mathsf{OUT}_{\zkmV} \langle P(w), \zkmV \rangle (x) \approx_{\zkmD_\secp, \epsilon+\mu}
% \bar \zkS^{\zkmV}(x, \zkmD_\secp, 1^{1/\epsilon})$$
% This completes the proof of the proposition.
% \end{proof}

% \subsection{The 2-Message Transformation for $\NP\cap\coNP$.}
% Here we only consider the  case that the original protocol is also a 2-message one. 

% \paragraph{Ingredients and notation:}
% \begin{itemize}
% \item
%  A non-interactive $\WI$ proof for \NP. We denote the proof by $\niwi$.
% \item
%  A $2$-message argument system $\prot{\zkP}{\zkV}$ for an $\NP\cap \coNP$ language $\lang$. We denote its messages by $(\vmes_1,\pmes_2)$. 
%  \end{itemize}
% %
% The protocol can be viewed as a simplified version of \proref{fig:sm_to_m_prot}, where the verifier, rather than arguing that the prover's commitment is to a non-witness, argues directly that the instance $\ins$ is a no-instance, which is indeed an $\NP$ statement since $\lang\in \coNP$.

% We describe the protocol in \figref{fig:sm_to_m_prot_coNP}.

% \protocol
% {\proref{fig:sm_to_m_prot_coNP}}
% {An argument $\prot{\bar \zkP}{\bar \zkV}$ for $\NP\cap\coNP$ against malicious verifiers.}
% {fig:sm_to_m_prot_coNP}
% {
% \begin{description}
%     \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
%     \item[$\bar \zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
% \end{description}
% \begin{enumerate}
% \item
% $\bar \zkV$ computes
% \begin{itemize}
% \item
% $\vmes_1$, the first message in the original protocol.
% \item
% $\niwi$, a \WI proof for the statement $\Phi(\ins,\vmes_1)$ given by:
% \begin{align*}
% \exists r \; : \; \vmes_1 = \zkV(\ins;r)
% \hspace{2mm} \bigvee \hspace{2mm}
% \exists \bar \wit  \; : \; \bar \wit \in \rel_{\zo^*\setminus \lang}(\ins)\enspace.
% \end{align*}
% \end{itemize}
% It sends $(\vmes_1,\niwi)$.
% \item 
% $\bar \zkP$ verifies the $\NIWI$ proof $\niwi$ for the statement $\Phi$, and aborts if it does not accept. 

% It then computes $\pmes_2$, the second message in the original protocol, and sends it.
%  \item
%     $\bar \zkV$ verifies the original argument $\vmes_1,\pmes_2$.
% \end{enumerate}
% }

% \paragraph{Analysis.} We now analyze the transformation.

% \begin{proposition}
% \proref{fig:sm_to_m_prot_coNP} is sound.
% \end{proposition}
% \begin{proof}
% To prove soundness, we show how to transform any cheating prover $\zkbmP$ against \proref{fig:sm_to_m_prot} into a cheating prover $\zkmP$ against the original protocol. The constructed $\zkmP$ requires a witness for the fact that the instance is a no-instance. Such a witness can be obtained non-uniformly (the reduction is uniform, however, provided the witness). 

% Fix any polynomial-size prover $\zkbmP = \set{\zkbmP_\secp}_\secp$. We describe a new prover $\zkmP$, and show that for any $(\ins,\bar \wit) \in \rel_{\zo^*\setminus \lang}$, if $\zkbmP$ convinces $\bar \zkV$ to accept with probability $\varepsilon$, the new prover convinces $\zkmP$ convinces $\zkV$ to accept with probability $\varepsilon-\secp^{-\omega(1)}$.

% \medskip
% \paragraph{${\zkmP}^{\zkbmP}(\ins,\bar \wit)$:}
% \begin{itemize}
% \item
% Obtains $\vmes_1$ from $\zkV$.
% \item
% Computes the \NIWI proof $\niwi$ for $\Phi(\ins,\vmes_1)$ using the witness $\bar \wit$.
% \item
% It then feeds $(\vmes_1,\niwi)$ to $\zkbmP$, and obtains back $\pmes_2$, which it sends to $\zkV$.
% \end{itemize}

% \paragraph{Prover analysis.} $\zkmP$ clearly runs in polynomial time. 

% We analyze the success probability. Observe that the only difference between the view of $\zkbmP$ in a real interaction with $\bar \zkV$ and its view as emulated by $\zkmP$ is that in the first the \NIWI proof $\niwi$ is computed using  the randomness of the honest verifier $\zkV$ as the witness, whereas in the second it is computed using $\bar \wit$. By the witness indistinguishability of the argument, it follows that $\zkmP$ convinces $\zkV$ with the same probability $\varepsilon$ that $\zkbmP$ convinces $\bar \zkV$, up to a negligible difference.  
% \end{proof}


% \begin{proposition}
% There exists a $\PPT$ simulator $\zkS$ such that for any polynomial-size (malicious) verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ against
% \proref{fig:sm_to_m_prot_coNP}:
% \begin{itemize}
% \item
% $\zkmV := \zkS^{\zkbmV}$ is an explainable verifier against the original protocol $\prot{\zkP}{\zkV}$.
% \item
% For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_\secp$ there exists a negligible $\mu$ such that for any $\secp\in \Nat$ and any $\ins\in\lang \cap \zo^\secp$,
% $$
% \view_{\zkbmV}\prot{\zkP(\wit)}{\zkbmV}(\ins) \approx_{\zkmD_\secp,\mu} \view_{\zkmV}\prot{\zkP(\wit)}{\zkmV}(\ins) \enspace.
% $$
% \end{itemize}
% \end{proposition}

% \begin{proof}
% We describe the simulator $\zkS$.

% \medskip
% \paragraph{$\zkS^{\zkbmV}(\ins)$:}
% \begin{itemize}
% \item 
% Obtains $(\vmes_1,\niwi)$ from $\zkbmV$. 
% \item
% Verifies the $\NIWI$ proof $\niwi$ for the statement $\Phi(\ins,\vmes_1)$. 
% \item
% If the argument is invalid, it simulates an abort message from $\bar \zkP$, feeds it to $\zkbmV$, obtains its output, and outputs the same (aborting the interaction with $\zkP$).
% \item
% Otherwise, it sends $\vmes_2$ to $\zkP$ and obtains $\pmes_2$. 
% \item
% Feeds $\pmes_2$ to $\zkbmV$, obtains its output, and outputs the same.
% \end{itemize}

% \paragraph{Simulator analysis.} The above simulator clearly runs in polynomial time. Furthermore, by construction, the view of the emulated $\zkbmV$ is distributed identically to its view in an interaction with $\bar \zkP$.

% We prove that $\zkmV = \zkS^{\zkbmV}$ is explainable. For this, note that since $\ins\in \lang$, $\Phi(\ins,\vmes_1)$ is true only if  
% $\vmes_2 \in \zkV(\ins)$. By the soundness of the \NIWI proof, it follows that $\niwi$ is rejected, and $\zkS$ aborts, unless $\vmes_1$ is explainable.
% \end{proof}


\subsection{The Two-Message \WH Transformation} Here we again only consider the  case that the original protocol is also a 2-message one. 

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
 A witness encryption scheme $\we$ for $\lang$.
\item
 A $2$-message \WH argument system $\prot{\zkP}{\zkV}$ for $\lang$. We denote its messages by $(\vmes_1,\pmes_2)$. 
 \end{itemize}
%
The protocol can be viewed as a variant of \proref{fig:sm_to_m_prot}, where the verifier, rather than using a \WI system to prove that it behaves honestly, proves it using a witness encryption of its coins under $\ins$. This proof is simulatable if $\ins \notin \lang$, and otherwise is sound.

We describe the protocol in \figref{fig:sm_to_m_prot_we}.

\protocol
{\proref{fig:sm_to_m_prot_we}}
{An argument $\prot{\bar \zkP}{\bar \zkV}$ for $\NP$ against malicious verifiers.}
{fig:sm_to_m_prot_we}
{
\begin{description}
    \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
    \item[$\bar \zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
\end{description}
\begin{enumerate}
\item
$\bar \zkV$ computes
\begin{itemize}
\item
$\vmes_1$, the first message in the original protocol.
\item
$\weCT \gets \weE_{\ins}(r)$, a witness encryption of the coins $r$ used to generate $\vmes_1$.
\end{itemize}
It sends $(\vmes_1,\weCT)$.
\item 
$\bar \zkP$ decrypts $\tilde r \gets \weD_{\wit}(\weCT)$, and verifies that $\vmes_1 = \zkV(\ins;r)$. If this is not the case, it aborts. 
\item
It then computes $\pmes_2$, the second message in the original protocol, and sends it.
 \item
    $\bar \zkV$ verifies the original argument $\vmes_1,\pmes_2$.
\end{enumerate}
}

\paragraph{Analysis.} We now analyze the transformation.

\begin{proposition}
\proref{fig:sm_to_m_prot_we} is sound.
\end{proposition}
\begin{proof}
To prove soundness, we show how to transform any cheating prover $\zkbmP$ against \proref{fig:sm_to_m_prot_we} into a cheating prover $\zkmP$ against the original protocol. 

Fix any polynomial-size prover $\zkbmP = \set{\zkbmP_\secp}_\secp$. We describe a new prover $\zkmP$, and show that for any $\ins \notin \lang$, if $\zkbmP$ convinces $\bar \zkV$ to accept with probability $\varepsilon$, the new prover convinces $\zkmP$ convinces $\zkV$ to accept with probability $\varepsilon-\secp^{-\omega(1)}$.

\medskip
\paragraph{${\zkmP}^{\zkbmP}(\ins)$:}
\begin{itemize}
\item
Obtains $\vmes_1$ from $\zkV$.
\item
Computes a witness encryption of zeros $\weCT\gets \weE_{\ins}(0^\secp)$.
\item
It then feeds $(\vmes_1,\weCT)$ to $\zkbmP$, and obtains back $\pmes_2$, which it sends to $\zkV$.
\end{itemize}

\paragraph{Prover analysis.} $\zkmP$ clearly runs in polynomial time. 

We analyze the success probability. Observe that the only difference between the view of $\zkbmP$ in a real interaction with $\bar \zkV$ and its view as emulated by $\zkmP$ is that in the first $\weCT$ is an encryption of  the randomness $r$ of the honest verifier $\zkV$, whereas in the second it is an encryption of zeros. Since $\ins\notin\lang$, it follows by the security of the witness encryption that $\zkmP$ convinces $\zkV$ with the same probability $\varepsilon$ that $\zkbmP$ convinces $\bar \zkV$, upto a negligible difference.  
\end{proof}


\begin{proposition}
\proref{fig:sm_to_m_prot_we} is witness hiding.
\end{proposition}

\begin{proof}
Let $\zkR$ be the witness be the witness-finding reduction of the original protocol $\prot{\zkP}{\zkV}$, we describe the witness-finding reduction $\zkbR$ for the new protocol $\prot{\zkbP}{\zkbV}$. In what follows let $\zkbmV=\set{\zkbmV_\secp}_\secp$ be a polynomial-size verifier.

\medskip
\paragraph{$\zkbR(\ins,\zkbmV_\secp,1^{1/\varepsilon})$:}
\begin{itemize}
\item
Runs $\zkbmV_\secp(\ins)$ and and obtains $(\vmes_1,\weCT)$.
\item
Emulates an abort message from $\zkbP$, feeds it to $\zkbmV_\secp$, and tests whether it outputs a witness $\wit\in\RL(\ins)$, and if so outputs it.
\item 
Otherwise, constructs from $\zkbmV_\secp$ a verifier $\zkmV_\secp$ that sends $(\vmes_1,\weCT)$ as its first message, obtains $\pmes_2$ from $\zkP$, feeds it to $\zkbmV$ and outputs whatever $\zkbmV$ does.
\item
Runs $\zkR(\ins,\zkmV_\secp,1^{1/\varepsilon})$.
\end{itemize}

\paragraph{Reduction analysis.} The above reduction clearly runs in polynomial time. We now analyze its validity. 

Let $\zkmV=\set{\zkmV_\secp}_\secp$ be a (w.l.o.g deterministic) polynomial-size verifier. Assume toward contradiction that there exist an infinite set $X$ of $\ins\in\lang\cap\zo^\secp$ and $\wit\in\RL(\ins)$ such that for some noticeable $\delta(\secp)$
$$ \Pr\[\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\] >   \Pr\[\zkR(\ins,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]+\varepsilon(\secp)+\delta(\secp)\enspace.
$$
We argue that for any $\ins$ such as above the verifier's message $\vmes_1$ is in the support of the honest verifier. Indeed, if it is not, then the reduction $\zkR$ first emulates a prover abort just as in the real system, where the prover detects the witness encryption does decrypt to randomness that explains $\vmes_1$. Thus,
$$ \Pr\[\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\] \leq    \Pr\[\zkR(\ins,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]\enspace.
$$
Thus, we can construct an explainable verifier ${\zkmV_\ins}_{\ins\in X}$ that on input $\ins$ behaves like $\zkmV$, and on any other input sends an abort message $\bot$. This verifier is explainable and fails the witness-finding reduction.  
\end{proof}


% \begin{proof}
% Let $\zkR$ be the witness be the witness-finding reduction of the original protocol $\prot{\zkP}{\zkV}$, we describe the witness-finding reduction $\zkbR$ for the new protocol $\prot{\zkbP}{\zkbV}$. In what follows let $\zkbmV=\set{\zkbmV_\secp}_\secp$ be a polynomial-size verifier.

% \medskip
% \paragraph{$\zkbR(\ins,\zkbmV_\secp,1^{1/\varepsilon})$:}
% \begin{itemize}
% \item 
% Constructs from $\zkbmV_\secp$ a verifier $\zkmV_\secp$ for the original protocol defined as follows:
% \begin{itemize}
% \item
% Runs $\zkbmV_\secp(\ins)$ and and obtains $(\vmes_1,\weCT)$.
% \item
% Emulates an abort message from $\zkbP$, feeds it to $\zkbmV_\secp$, and tests whether it outputs a witness $\wit\in\RL(\ins)$.
% \item
% If so, it discards $\zkbmV$'s message and sends $\zkP$ an honestly generated message $\vmes_1' \gets \zkV(\ins)$, obtains $\pmes'$ from $\zkP$, and output $\wit$.
% \item
% If $\zkbmV_\secp$ did not output a witness, it continues emulating the interaction using $\zkbmV$'s message: it sends $\zkP$ the $\vmes_1$, obtains $\pmes_2$, feeds it to $\zkbmV_\secp$, obtains its output, and outputs the same. 
% \end{itemize}
% \item
% Runs $\zkR'(\ins,\zkmV_\secp,1^{1/\varepsilon})$.

% Here $\zkR'(\ins,\zkmV_\secp,1^{1/\varepsilon})$ first constructs a new verifier $\zkmV_\ins$ that given $\ins$ acts exactly as $\zkmV_\secp$, and for any other $\ins$ acts honestly according to $\zkV$ and outputs $\bot$. It then runs $\zkR(\ins,\zkmV_\ins,1^{1/\varepsilon})$, 
% \end{itemize}

% \paragraph{Reduction analysis.} The above reduction clearly runs in polynomial time. We now analyze its validity. 

% We first argue that 
% %any two-message $\WH$ protocol against explainable verifiers is also weakly $\WH$ (against arbitrary verifiers), where weak $\WH$ is defined below.
% %\begin{definition}[Weak \WH]\label{def:wwh}
% %A protocol $\prot{\zkP}{\zkV}$ is weakly $\WH$ if 
% there exists a %\PPT reduction $\zkR'$, 
% %such that for any polynomial-size verifier $\zkmV=\set{\zkmV_\secp}_\secp$ and noticeable $\varepsilon(\secp)$, 
% negligible $\mu(\secp)$, such that for any $\secp\in\Nat$ and $\ins\in\lang\cap\zo^\secp$,
% $$ \Pr\[\hview_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\] \leq   \Pr\[\zkR'(\ins,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]+\varepsilon(\secp)+\mu(\secp)\enspace.
% $$
% %\end{definition}

% %To see this, let 
% %, we describe a variant $ \zkR'$ of $\zkR$ that establishes that the system is weakly $\WH$.

% %where $\zkR$ is the witness-finding reduction for an explainable two-message $\WH$ $\prot{\zkP}{\zkV}$.

% %We now argue that $\zkR'$ satisfies the weak \WH property. 
% Now fix any polynomial-size $\zkmV=\set{\zkmV_\secp}_\secp$, and assume toward contradiction that there exist noticeable $\varepsilon(\secp),\delta(\secp)$ such that for infinitely many $\secp \in \Nat$ and $\ins_\secp \in \zo^\secp\cap \lang$ and $\wit_\secp\in\RL(\ins_\secp)$, it holds that 
% $$ \Pr\[\hview_{\zkmV_\secp}\prot{\zkP(\wit_\secp)}{\zkmV_\secp}(\ins_\secp)\in\RL(\ins_\secp)\] >   \Pr\[\zkR'(\ins_\secp,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins_\secp)\]+\varepsilon(\secp)+\delta(\secp)\enspace.
% $$
% Then, in particular, for any such $\ins_\secp$, $\zkmV_\secp$ sends an explainable message. This means that the verifier $\set{\zkmV_{\ins_\secp}}_\secp$, as defined above, is explainable. 

% Furthermore, by the above equation, and the definition of $\zkR'$,
% $$ \Pr\[\view_{\zkmV_{\ins_\secp}}\prot{\zkP(\wit_\secp)}{\zkmV_{\ins_\secp}}(\ins_\secp)\in\RL(\ins_\secp)\] >   \Pr\[\zkR(\ins_\secp,\zkmV_{\ins_\secp},1^{1/\varepsilon})\in\RL(\ins_\secp)\]+\varepsilon(\secp)+\delta(\secp)\enspace,
% $$
% which contradicts $\WH$ against explainable verifiers.


% Next, we argue
% $$ \Pr\[\view_{\zkbmV_\secp}\prot{\zkbP(\wit)}{\zkbmV_\secp}(\ins)\in\RL(\ins)\] \leq \Pr\[\hview_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\]\enspace;
% $$
% namely, the probability that $\zkbmV$ outputs a witness equals that probability that the honest truncation of $\zkmV$ outputs one.

% Indeed, we consider the following cases:
% \begin{itemize}
% \item
% Assume $\zkbmV$ behaves maliciously, but outputs a witness given an abort message. Then, by construction, $\zkmV$ behaves in an explainable manner (in fact, honestly) and outputs a witness.

% \item
% Assume $\zkbmV$ is explainable. Then $\zkmV$ either finds a witness when emulating an abort, or perfectly emulates the view of $\zkbmV$, and thus outputs a witness with the same probability. 
% \end{itemize}



% To conclude the proof, recall that
% $$ \Pr\[\hview_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\] \leq   \Pr\[\zkR'(\ins,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]+\varepsilon(\secp)+\mu(\secp)\enspace.
% $$
% and thus
% \begin{align*}
% &\Pr\[\view_{\zkbmV_\secp}\prot{\zkbP(\wit)}{\zkbmV_\secp}(\ins)\in\RL(\ins)\]\leq&\\
% &\Pr\[\hview_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\in\RL(\ins)\] \leq& \Pr\[\zkR'(\ins,\zkmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]+\varepsilon(\secp)+\secp^{-\omega(1)}=\\ &&\Pr\[\zkbR(\ins,\zkbmV_\secp,1^{1/\varepsilon})\in\RL(\ins)\]+\varepsilon(\secp)+\secp^{-\omega(1)}\enspace,
% \end{align*}
% concluding the proof.
% \end{proof}

\begin{remark}
The transformation given by \proref{fig:sm_to_m_prot_we} preserves public verifiability. Indeed, verification is the same as in the original protocol.
\end{remark}

\bibliographystyle{alpha}
\bibliography{main}

\appendix

\section{Relaxed Random Self-Reducible Public-Key Encryption from LWE}\label{sec:RRSR_LWE}

\def \A {\mathbf{A}}
\def \t {\mathbf{t}}
\def \s {\mathbf{s}}
\def \c {\mathbf{c}}
\def \u {\mathbf{u}}
\def \tc {\widetilde{\mathbf{c}}}
\def \e {\mathbf{e}}
\def \ZZ {\mathbb{Z}}
\def \gaus {\overline{\Psi}}
In this appendix, we describe a relaxed random self-reducible public-key based on LWE. 

\paragraph{Lattice preliminaries.} In what follows, $q$ is a prime and $\alpha,\beta,m,n$ are such that $\alpha 2^{n^{0.1}}<\beta<\frac{q}{8m}$ and $n < \frac{m}{3\log q} < n^{O(1)}$. We denote by $\gaus_{m,\sigma}$ the truncated discrete Gaussian distribution on $\ZZ^m$ with parameter $\sigma$, where any sample $x$ such that $\|x\|>\sqrt{m}\sigma$ is replaced by $0$. Following common habit, we will identify the security parameter (denoted by $\secp$ in the rest of the paper) with the lattice dimension $n$.

\nir{cite some lemmas}

\paragraph{The scheme:}
\begin{itemize}
    \item
    $\rsreG(1^n):$ outputs a public key $\A \in\ZZ_q^{m\times n}$ and secret key $\t \in \zo^{m-1}$ such that $\A$ is statistically close to uniform and $(1|\t^T) \A = 0$.
    \item
    $\rsreE_\A(b):$ samples $\s\gets \ZZ_q^n$, $\e \gets \gaus_{m,\alpha}$ and outputs $\c=\A\s+\e +b\(\frac{q}{2}|0^{m-1}\)$.
    \item
    
    $\rsreD_{\t}(\c):$ outputs $0$ if $|\langle \c,(1|\t^T) \rangle|\leq q/4$, and $1$ otherwise.
    \item
    $\rsretE_\A(b):$ similar to $\rsreE$, only that $\e \gets \gaus_{m,\beta}$.
    \item
    $\rsretD^{\rsremD}(\c,\A,1^{k}):$
    \begin{itemize}
        \item
        Let $\tc$ be the distribution given by sampling $\s' \gets \ZZ_{q}^n$, $\e' \gets \gaus_{m,\beta}$, and outputting $\c+\A\s'+\e'$.
        \item
        Compute estimations: 
        \begin{itemize}
            \item
            $\tilde \rho$ of $\rho:=\EE \rsremD(\tc)$,
            \item
            $\tilde \rho_0$ of $\rho_0:=\EE \rsremD(\rsretE_\A(0))$,
                \item
            $\tilde \rho_1$ of $\rho_1:=\EE \rsremD(\rsretE_\A(1))$,
        \end{itemize} using $k^2\cdot n$ samples for each.
        \item 
        Output $0$ if $|\rho - \rho_0|\leq |\rho - \rho_1|$ and $1$ otherwise.
        \end{itemize}
\end{itemize}

\begin{claim}
Assuming $\text{LWE}_{n,q,\alpha}$, the scheme is a relaxed RSR encryption.
\end{claim}

\begin{proof}[Proof sketch.] We prove that the scheme satisfies the properties required in \defref{def:rsr}.

\paragraph{Correctness:} for any $b\in\zo,n\in\Nat$,
\begin{align*}
\rsreD_{\t}(\rsreE_{\A}(b)) = & \left\langle \A\s+\e+b\(\frac{q}{2}\pST 0^{m-1}\),(1 | \t^T) \right\rangle =\\ 
& 0 +\langle \e, (1 | \t^T)\rangle +bq/2\enspace.    
\end{align*}
Correctness then follows from the fact that
\begin{align*}
|\langle \e, (1 | \t^T)\rangle| \leq \|\e\|\cdot \|(1 | \t^T)\| \leq \alpha\sqrt{m}\cdot\sqrt{m} \leq q/8\enspace. 
\end{align*}
For $\rsretE_{\A}(b)$, correctness is shown similarly, where the only exception is that $\|\e\|\leq \beta\sqrt{m}$. Still, $$|\langle \e, (1 | \t^T)\rangle|\leq \beta m \leq q/8\enspace.$$


\paragraph{Indistinguishability:} by the $\text{LWE}_{n,q,\alpha}$ assumption, for any polynomial-size distinguisher $\zkmD=\set{\zkmD_n}_{n\in\Nat}$, there exists a negligible $\mu$ such that for any security parameter $n\in \Nat$ and any $b\in \zo$,
\begin{align*}
\A,\rsreE_{\A}(b) = \A,\A \s +\e + b\(\frac{q}{2} \pST 0^{m-1}\) 
\approx_{\zkmD_n,\mu} \A, \u
\enspace,
\end{align*}
where $\A \gets \ZZ_q^{m\times n},\s \gets \ZZ_q^{n},\u \gets \ZZ_q^{m}$, and $\e \gets \gaus_{n,\alpha}$.


\paragraph{Random self-reduction:} fix any $\A$ and distinguisher $\rsremD$ such that 
$\abs{\rho_0-\rho_1}\geq \varepsilon\enspace$, and fix any ciphertext $\c = \A\s+\e+ b\(\frac{q}{2} \pST 0^{m-1}\)  \in \rsreE_\A(b)$.

For this, we rely on {\em noise flooding} \cite{Gen09}: for $\s'\gets \ZZ_q^n, \e'\gets \gaus_{m,\beta}$
$$\tc = \c +\A\s'+\e' = \A(\s+\s')+(\e+ b\(\frac{q}{2} \pST 0^{m-1}\)+\e')$$
is statistically close to a fresh sample $$\rsretE_\A(b) = \A\s'+\e'\enspace.$$
Our random self reduction process now succeeds by standard concentration bounds. 


\end{proof}



\end{document}


% may be useful for non-generic transformation.

% \paragraph{Ingredients and notation:}
% \begin{itemize}
% \item
%  A 2-message $\WI$ argument for \NP with delayed input. We denote its messages by $(\wi_1,\wi_2)$.
% \item
%  A 3-message $\WI$ argument of knowledge for \NP. We denote its messages by $(\wik_1,\wik_2,\wik_3)$.
% \item
%   A non-interactive perfectly-binding commitment scheme $\COM$. 
% \item
%  A $3$-message argument system $\prot{\zkP}{\zkV}$ for an $\NP$ language $\lang$ that is \WZK against explainable verifiers and has a semi-black-box simulator. We denote its messages by $(\pmes_1,\vmes_2,\pmes_3)$.
 
%  \end{itemize}
% %
% We describe the protocol in \figref{fig:sm_to_m_prot}.

% \protocol
% {\proref{fig:sm_to_m_prot}}
% {A \WZK argument $\prot{\bar \zkP}{\bar \zkV}$ for $\NP$ against malicious verifiers.}
% {fig:sm_to_m_prot}
% {
% \begin{description}
%     \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
%     \item[$\bar \zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
% \end{description}
% \begin{enumerate}
% \item
% $\bar \zkP$ computes
% \begin{itemize}
% \item
% $\pmes_1$, the first message in the original protocol.
% \item
% $\cmt_0,\cmt_1 \gets \COM(\wit)$, two independent commitments to the witness.
% \item
% $\wik_1$, the first message of a \WI argument of knowledge for the statement $\Psi(\cmt_0,\cmt_1)$:
% \begin{align*}
% \exists r_0,s_0  \; : \; \cmt_0 = \COM(s_0;r_0) \hspace{2mm} \bigvee \hspace{2mm} \exists r_1,s_1  \; : \; \cmt_1 = \COM(s_1;r_1) \enspace,
% \end{align*}
% using $(r_0,s_0)$ as the witness.
% \item
% $\wi_1$, the first message of a $\WI$ argument.
% \end{itemize}
% It sends $(\pmes_1,\cmt_0,\cmt_1,\wik_1,\wi_1)$.
% \item
% $\bar \zkV$ computes
% \begin{itemize}
% \item
% $\vmes_2$, the second message in the original protocol.
% \item
% $\wik_2$, the second \WI argument of knowledge message for $\Psi(\cmt_0,\cmt_1)$.
% \item
% $\wi_2$, the second \WI message for the statement $\Phi(\ins,\cmt_0,\cmt_1,\pmes_1,\vmes_2)$:
% \begin{align*}
% &\exists r \; : \; \vmes_2 = \zkV(\ins,\pmes_1;r)
% \hspace{2mm} &\bigvee\\
% &\exists r_0,s_0  \; : \; \cmt_0 = \COM(s_0;r_0), s_0 \notin \RL(\ins)
% \hspace{2mm} &\bigvee\\ 
% &\exists r_1,s_1  \; : \; \cmt_1 = \COM(s_1;r_1), s_1 \notin \RL(\ins)\enspace.
% \end{align*}
% \end{itemize}
% It sends $(\vmes_2,\wik_2,\wi_2)$.
% \item 
% $\bar \zkP$ verifies the $\WI$ argument $(\wi_1,\wi_2)$ for the statement $\Phi$, and aborts if it does not accept. 

% It then computes
% \begin{itemize}
% \item
% $\pmes_3$, the third message in the original protocol.
% \item

% $\wik_3$, the third message of the \WI argument of knowledge $\Psi(\cmt_0,\cmt_1)$.
% \end{itemize}
% It sends $(\pmes_3,\wik_3)$.
%  \item
%     $\bar \zkV$ verifies 
%     \begin{itemize}
%     \item
%     the $\WI$ argument $(\wik_1,\wik_2,\wik_3)$ for the statement $\Psi$,
%     \item
%     the original argument $(\pmes_1,\vmes_2,\pmes_3)$.
%     \end{itemize}
% \end{enumerate}
% }

% \paragraph{Analysis.} We now analyze the transformation.

% \begin{proposition}
% \proref{fig:sm_to_m_prot} is sound.
% \end{proposition}
% \begin{proof}
% To prove soundness, we show how to transform any cheating prover $\zkbmP$ against \proref{fig:sm_to_m_prot} into a cheating prover $\zkmP$ against the original protocol. 

% Fix any polynomial-size prover $\zkbmP = \set{\zkbmP_\secp}_\secp$. We describe a new prover $\zkmP$, and show that for any $\ins \notin \lang$, if $\zkbmP$ convinces $\bar \zkV$ to accept with probability $\varepsilon$, the new prover convinces $\zkmP$ convinces $\zkV$ to accept with probability $\varepsilon-\secp^{-\omega(1)}$.

% \medskip
% \paragraph{${\zkmP}^{\zkbmP}(\ins,1^{1/\varepsilon})$:}
% \begin{itemize}
% \item
% Constructs from $\zkbmP$ a prover for the \WI argument of knowledge $\zkmP_{\wik}$ that works as follows:
% \begin{itemize}
% \item 
% Obtains $(\pmes_1,\cmt_0,\cmt_1,\wik_1,\wi_1)$ from $\zkbmP$, and sends $\wik_1$ as the first message.
% \item
% Given $\wik_2$ from the $\WI$ verifier, it honestly emulates a second message $\vmes_2$ of $\zkV$, and honestly emulates the $\WI$ argument second message $\wi_2$. It feeds $(\vmes_2,\wik_2,\wi_2)$ to $\zkbmP$.
% \item
% It obtains $(\pmes_3,\wik_3$, and sends $\wik_3$ as the third message.
% \end{itemize}
% It now applies the knowledge extractor $\zkE^{\zkmP_\wik}(\ins,1^{1\varepsilon})$ to obtain a witness for the statement $\Psi(\cmt_0,\cmt_1)$.
% \item
% If the extractor fails to find a witness, $\zkmP$ aborts. Otherwise, let $(r,s)$ be the extracted witness; that is, an opening to $\cmt_0$ or $\cmt_1$.
% \item 
% $\zkmP$ now proceeds to its interaction with $\zkV$.
% \item
% It sends $\pmes_1$ to $\zkV$, and obtains $\vmes_2$.
% \item
% It emulates the argument of knowledge message $\wik_2$ honestly, and computes the argument message $\wi_2$ for $\Phi(\ins,\cmt_0,\cmt_1,\pmes_1,\vmes_2)$ using the witness $(r,s)$ previously obtained.
% \item
% It then feeds $(\vmes_2,\wik_2,\wi_2)$ to $\zkbmP$, and obtains back $(\pmes_3,\wik_3)$. It sends $\pmes_3$ to $\zkV$.
% \end{itemize}

% \paragraph{Prover analysis.} First, note that $\zkmP$ runs in polynomial time (in its input length $\secp+1/\varepsilon$).

% We now analyze the success probability. 
% First, by the extraction guarantee, in the extraction phase, we onbtain a witness $(r,s)$ with probability $1-\secp^{-\omega(1)}$. Note that since $\ins \notin \lang$, it necessarily holds that $s\notin \RL(\ins)$, and accordingly $(r,s)$ is also a valid witness for any statment $\Phi(\ins,\cmt_0,\cmt_1,\arg_1,\arg_2)$, regardless of $\arg_2$.

% Next, observe that the only difference between the view of $\zkbmP$ in a real interaction with $\bar \zkV$ and its view as emulated by $\zkmP$ is that in the first the \WI argument $(\wi_1,\wi_2)$ is computed using  the randomness of the honest verifier $\zkV$ as the witness, whereas in the second it is computed using the extracted witness $(r,s)$.

% By the witness indistinguishability of the argument, it follows that $\zkmP$ convinces $\zkV$ with the same probability $\varepsilon$ that $\zkbmP$ convinces $\bar \zkV$, up to a negligible difference.  
% \end{proof}

% \begin{proposition}
% Assume that the original protocol $\prot{\zkP}{\zkV}$ is \WZK \nir{XX}, then, \proref{fig:sm_to_m_prot} is \WZK.
% \end{proposition}

% \begin{proof}
% \begin{claim}
% There exists a $\PPT$ simulator $\zkS$ such that for any polynomial-size (malicious) verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ against
% \proref{fig:sm_to_m_prot}:
% \begin{itemize}
% \item
% $\zkmV := \zkS^{\zkbmV}$ is an explainable verifier against the original protocol $\prot{\zkP}{\zkV}$.
% \item
% For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_\secp$ there exists a negligible $\mu$ such that for any $\secp\in \Nat$ and any $\ins\in\lang \cap \zo^\secp$,
% $$
% \view_{\zkbmV}\prot{\zkP(\wit)}{\zkbmV}(\ins) \approx_{\zkmD_\secp,\mu} \view_{\zkmV}\prot{\zkP(\wit)}{\zkmV}(\ins) \enspace.
% $$
% \end{itemize}

% \end{claim}
% \end{proof}

% \begin{proposition}
% There exists a $\PPT$ simulator $\zkS$ such that for any polynomial-size (malicious) verifier $\zkbmV=\set{\zkbmV_\secp}_\secp$ against
% \proref{fig:sm_to_m_prot}:
% \begin{itemize}
% \item
% $\zkmV := \zkS^{\zkbmV}$ is an explainable verifier against the original protocol $\prot{\zkP}{\zkV}$.
% \item
% For any polynomial-size distinguisher $\zkmD=\set{\zkmD_\secp}_\secp$ there exists a negligible $\mu$ such that for any $\secp\in \Nat$ and any $\ins\in\lang \cap \zo^\secp$,
% $$
% \view_{\zkbmV}\prot{\zkP(\wit)}{\zkbmV}(\ins) \approx_{\zkmD_\secp,\mu} \view_{\zkmV}\prot{\zkP(\wit)}{\zkmV}(\ins) \enspace.
% $$
% \end{itemize}
% \end{proposition}

% \begin{proof}
% We describe the simulator $\zkS$.

% \medskip
% \paragraph{$\zkS^{\zkbmV}(\ins)$:}
% \begin{itemize}
% \item 
% Obtains $\pmes_1$ from $\zkP$. 
% \item
% Emulates the first message of $\bar \zkP$ by computing:
% \begin{itemize}
% \item
% $\cmt_0,\cmt_1 \gets \COM(0^{|\wit|})$.
% \item
% $\wik_1$, the first message of a \WI argument of knowledge for the statement $\Psi(\cmt_0,\cmt_1)$. For this it uses $(r_0,s_0=0^{\wit})$ as the witness.
% \item
% $\wi_1$, the first message of a $\WI$ argument.
% \end{itemize}
% Feeds the emulated message $(\pmes_1,\cmt_0,\cmt_1,\wik_1,\wi_1)$ to the oracle $\zkbmV$, and obtains $(\vmes_2,\wik_2,\wi_2)$. 
% \item
% Verifies the $\WI$ argument $(\wi_1,\wi_2)$ for the statement $\Phi(\ins,\cmt_0,\cmt_1,\pmes_1,\vmes_2)$. 
% \item
% If the argument is invalid, it simulates an abort message from $\bar \zkP$, feeds it to $\zkbmV$, obtains its output, and outputs the same (aborting the interaction with $\zkP$).
% \item
% Otherwise, it sends $\vmes_2$ to $\zkP$ and obtains $\pmes_3$. 
% \item
% Emulates the third message (of $\bar \zkP$) by computing $\wik_3$, the third message of the \WI argument of knowledge for the statement $\Psi(\cmt_0,\cmt_1)$.
% \item
% Feeds the emulated message $(\pmes_3,\wik_3)$ to $\zkbmV$, obtains its output, and outputs the same.
% \end{itemize}

% \paragraph{Simulator analysis.} The above simulator clearly runs in polynomial time. Furthermore, by construction, the view of the emulated $\zkbmV$ is distributed identically to its view in an interaction with $\bar \zkP$.

% From hereon, we focus on proving that $\zkmV = \zkS^{\zkbmV}$ is explainable. For this, it suffices to show that with overwhelming probability, unless $\vmes_2$ is explainable (i.e., $\vmes_2 =  \zkV(\ins,\pmes_1;r)$ for some $r$), the $\WI$ argument $(\wi_1,\wi_2)$ given by $\zkbmV$ is rejected. To show this, we consider several hybrids and show that the probability that the above event occurs is preserved throughout the hybrids.

% \paragraph{$\hyb_0$:} This is the real protocol.

% \paragraph{$\hyb_1$:} In this hybrid, the commitment $\cmt_1$ is a commitment to $\wit\in\RL(\ins)$ instead of $0^{|\wit|}$.

% This hybrid is indistinguishable from the previous one by the hiding of the commitment.

% \paragraph{$\hyb_2$:} In this hybrid, the \WI argument of knowledge $(\wik_1,\wik_2,\wik_3)$ is computed using $(r_1,s_1 = \wit)$ as the witness instead of $(r_0,s_0=0^{|\wit|})$.

% This hybrid is indistinguishable from the previous one by the witness indistinguishability of the argument. 

% \paragraph{$\hyb_3$:} In this hybrid, the commitment $\cmt_0$ is a commitment to $\wit\in\RL(\ins)$ instead of $0^{|\wit|}$.

% This hybrid is indistinguishable from the previous one by the hiding of the commitment.

% \medskip\noindent
% It is left to show that in $\hyb_3$, except with negligible probability, $\zkbmV$ fails to produce an accepting $\WI$ argument unless $\vmes_2$ is explainable. 

% In this hybrid both 
% $\cmt_0, \cmt_1$ are commitments to a valid witness, and by the perfect binding of $\COM$, they cannot be opened to a non-witness. Accordingly,  $\Phi(\ins,\cmt_0,\cmt_1,\pmes_1,\vmes_2)$ is true only if  
% $\vmes_2 \in \zkV(\ins,\pmes_1)$. By the soundness of the \WI argument, it follows that except with negligible probability $(\wi_1,\wi_2)$ is rejected unless $\vmes_2$ is explainable.
% \end{proof}


% section{Weak Zero-Knowledge against Explainable Verifiers}\label{sec:semi_mal}
% \nir{old section}

% \subsection{A Three-Message Protocol}\label{sec:3wzk_expl}

% In this section, we construct a three-message \WZK argument against explainable verifiers with a semi-black-box simulator. We start by presenting the protocol and then proceed to analyze it.

% \paragraph{Ingredients and notation:}
% \begin{itemize}
% \item
%  A 3-message instance-dependent $\WI$ argument of knowledge for \NP with delayed input $(\wiP,\wiV)$, where $\wiP=(\wiP_1,\wiP_2)$, $\wiV=(\wiV_1,\wiV_2)$. We denote its messages by $(\wi_1,\wi_2,\wi_3)$.
% \item
%   A non-interactive perfectly-binding commitment scheme $\COM$. 
% \item
%  A fully-homomorphic encryption scheme $(\fheE,$ $\fheD,$ $\fheEv)$.
% \item
%   A compute-and-compare obfuscator $\O$.
%   \item
%   A random self-reducible public-key encryption $(\rsreG,$ $\rsreE,$ $\rsreD,$ $\rsretD)$. (In fact, relaxed RSR suffices. To simplify the description of the protocol, we rely on standard RSR, and later remark why relaxed RSR suffices.)
% \end{itemize}
% %
% We describe the protocol in \figref{fig:wzk_prot}.

% \protocol
% {\proref{fig:wzk_prot}}
% {A 3-message $\WZK$ argument for $\NP$ against explainable verifiers.}
% {fig:wzk_prot}
% {
% \begin{description}
%     \item[Common Input:] an instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp$.
%     \item[$\zkP$'s auxiliary input:] a witness $\wit\in \RL(\ins)$.
% \end{description}

% \begin{enumerate}
% \item
% $\zkP$ computes $(\wi_1,\tau_\zkP) \gets\wiP_1^\ins(1^\secp)$, the first $\WI$ message relative to the instance $\ins$ and a corresponding state. It sends $\wi_1$.
% \item
% $\zkV$ computes
% \begin{itemize}
% \item
% $(\wi_2,\tau_\zkV) 
% \gets \wiV_1^{\ins}(\wi_1)$, the second \WI message and a corresponding state.
% \item
% $\cmt \gets \COM(0;r)$, a commitment to zero, using randomness $r \gets \zo^\secp$,
% \item
% $\zkVCT \gets \fheE_{\fheK}(r)$, an encryption of the commitment randomness, under a randomly chosen secret key $\fheK\gets \zo^\secp$.
% \item
% $\obfC\gets \O(\CC{\fheD_\fheK,u})$, an obfuscation of the CC program given by the FHE decryption circuit and a random target $u\gets \zo^\secp$.
% \item
% $\zkVCT' \gets \rsreE_{\rsrePK}(u)$, an RSR encryption of the target $u$, where $(\rsreSK',\rsrePK')\gets \rsreG(1^\secp)$ are randomly chosen keys.
% \end{itemize}
% It sends $(\wi_2,\cmt,\zkVCT,\obfC,\zkVCT',\rsrePK')$.
% \item 
% $\zkP$ computes
% \begin{itemize}
% \item
% $\zkPCT\gets \rsreE_{\rsrePK'}(1)$, an RSR encryption of $1$.
% \item
% $\wi_3 \gets \wiP_2^{\ins}(\Psi,\wit,\wi_1,\wi_2;\tau_\zkP)$, the third $\WI$ message for the statement
% \begin{align*}
% \Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK') :=\\
%      &\exists \wit  \; : \; (\ins,\wit) \in \RL \hspace{2mm} &\bigvee\\ &\exists r \; : \;
%     \cmt = \COM(0;r) \hspace{2mm} &\bigvee\\ 
%     &\exists \evciph \; : \;
%     \obfC(\evciph) = 1 \hspace{2mm} &\bigvee\\ 
%     &\exists r' \; : \; \zkPCT = \rsreE_{\rsrePK'}(0;r') 
%     \hspace{2mm}\enspace,
% \end{align*}
% using the witness $\wit\in\RL(\ins)$.
%  \end{itemize}
%  It sends $(\zkPCT,\wi_3)$.
%  \item
%     $\zkV$ verifies 
%     \begin{itemize}
%     \item
%     that the WI proof is accepted: $\wiV_2(\Psi,\wi_1,\wi_2,\wi_3;\tau_\zkV)=1$.
%     \item
%     that the prover's ciphertext decrypts to one: $\rsreD_{\rsreSK'}(\zkPCT)=1$.
%     \end{itemize}
% \end{enumerate}
% }

% \subsubsection{Analysis}

% We now analyze the protocol. We first show that it is sound, and then that it is $\WZK$ against explainable verifiers.

% \begin{proposition}
% \proref{fig:wzk_prot} is sound.
% \end{proposition}
% \begin{proof}
% Assume toward contradiction that there exists a polynomial-size (w.l.o.g deterministic prover) $\zkmP=\set{\zkmP_\secp}$ that (for infinitely many $\secp\in\Nat$) breaks soundness with noticeable probability $\varepsilon(\secp) =\secp^{-O(1)}$. Fix $\secp$ and $\ins\in \zo^\secp\setminus \lang$ such that $\zkmP_\secp$ convinces the verifier of accepting with probability $\varepsilon$. 

% \paragraph{Augmenting the interaction with extraction.} We parse any verifier message $(\wi_2,\cmt,\zkVCT,\obfC,\zkVCT',\rsrePK')$, as two parts $(\wi_2,z)$. For any $z$, we consider a \WI prover $\wimP_z$ whose first message is the same as $\zkmP_\secp$, and given a message $\wi_2$ from the verifier $\wiV$, computes the third $\wi_3$ message by running $\zkmP_\secp$ on $(\wi_2,z)$, emulating a message form $\zkV$. For any transcript $T=(\wi_1,(\wi_2,z),(\wi_3,\zkPCT))$ of an execution between $\zkmP_\secp$ and $\zkV$, we consider the result $\wit_T$ of running the witness extractor $\wit_T \gets \zkE^{\wimP_z,\ins}(1^{4/\varepsilon},\Psi,\wi_1,\wi_2,\wi_3)$, where $\Psi$ is the instance determined by the transcript $T$. (Note that $\wit_T$ is a random variable that depends on $T$ and the extractor's coins.)

% Let $F$ be the event, over a transcript $T$ and coins of the extractor $\zkE$, that $\zkV$ accepts the WI proof and the extracted witness $\wit_T$ does {\bf not} attest that $\zkPCT$ is a zero encryption; that is, $\wit_T$ is {\bf not} randomness $r'$ such that $\zkPCT = \rsreE(0;r')$. We next consider several hybrid experiments and show that the probability that $F$ occurs is preserved through these experiments, upto a negligible difference. To reach a contradiction, we show that $F$ occurs in the first hybrid with probability at least $\varepsilon$ and with probability at most $\varepsilon/2$ in the last hybrid. This is a contradiction since the gap $\varepsilon/2$ is noticeable. In what follows, in each hybrid $i$, we will denote by  $p_i$ the probability that $F$ occurs in that hybrid.  

% \paragraph{$\hyb_0$:} This is the real protocol.

% \begin{claim}
% $p_0 \geq \varepsilon$.
% \end{claim}
% \begin{proof}
% By definition, whenever $\zkV$ accepts, it decrypts $\zkPCT$ to $1$; thus, by the correctness of $\rsre$, the ciphertext $\zkPCT$ cannot be opened to an encryption of $0$.  The claim now follows from the fact that $\zkmP_\secp$ convinces $\zkV$ with probability $\varepsilon$.
% \end{proof}


% \paragraph{$\hyb_1$:} In this hybrid, $\zkVCT'$ is an encryption of $0^\secp$ instead of the target $u$. 

% \begin{claim}
% $\abs{p_0-p_1} \leq \secp^{-\omega(1)}$.
% \end{claim}
% \begin{proof}
% The claim follows by the semantic security of the scheme $\rsre$. Indeed, given a noticeable difference between $p_0$ and $p_1$, we can distinguish an RSR encryption of a random $u$ from one of $0^\secp$, by emulating an interaction between $\zkmP_\secp$ and $\zkV$, running the extractor, and testing whether $F$ occurs. 
% \end{proof}



% \paragraph{$\hyb_2$:} In this hybrid, the obfuscation $\obfC \gets \ccSim(1^\secp,1^\ell)$ is simulated rather than an obfuscation of $\CC{\fheD_{\fheK},u}$, where $\ell$ is the size of the decryption circuit $\fheD_{\fheK}$.


% \begin{claim}
% $\abs{p_1-p_2} \leq \secp^{-\omega(1)}$.
% \end{claim}
% \begin{proof}
% The claim follows by the CC simulation guarantee. Indeed, given a noticeable difference between $p_1$ and $p_2$, we can distinguish, given $\fheK$, an obfuscation of $\CC{\fheD_{\fheK},u}$ for a random $u$, from a simulated obfuscation contradicting the CC guarantee. Using the fact that now $\zkVCT'$ is an encryption of $0^\secp$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
% \end{proof}


% \paragraph{$\hyb_3$:} In this hybrid, $\zkVCT$ is an encryption of $0^\secp$ instead of the commitment randomness $r$.


% \begin{claim}
% $\abs{p_2-p_3} \leq \secp^{-\omega(1)}$.
% \end{claim}
% \begin{proof}
% The claim follows by the semantic security of the FHE scheme $\fhe$. Indeed, given a noticeable difference between $p_2$ and $p_3$, we can distinguish, an encryption of a random $r$ from an encryption of $0^\secp$. Since now the FHE key $\fheK$ is not needed to compute the obfuscation $\obfC$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
% \end{proof}


% \paragraph{$\hyb_4$:} In this hybrid, $\cmt$ is a commitment to $1$ instead of $0$.

% \begin{claim}
% $\abs{p_3-p_4} \leq \secp^{-\omega(1)}$.
% \end{claim}
% \begin{proof}
% The claim follows by hiding of the commitment. Given a noticeable difference between $p_3$ and $p_4$, we can distinguish, a commitment to zero from a commitment to one. In this hybrid, $\zkVCT$ no longer depends on the commitment randomness, so we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
% \end{proof}

% .

% \medskip\noindent
% It is left to show that in $\hyb_4$, $F$ occurs with probability at most $\varepsilon/2$. 

% \begin{claim}
% $p_4 \leq \varepsilon/2$.
% \end{claim}
% \begin{proof}
% Assume toward contradiction that $p_4 > \varepsilon/2$. First, observe that in hybrid $\hyb_4$:
% \begin{itemize}
% \item
% $\ins\notin \lang$.
% \item
% $\cmt \in \COM(1)$, and by perfect binding there does not exist $r$ such that $\cmt = \COM(0;r)$.
% \item
% By the CC simulation guarantee, except with negligible probability $2^{-\secp}$, there does not exist $\evciph$ such that $\obfC(\evciph) = 1$.
% \end{itemize}
% In particular, we can fix the second part $z$ of the  verifier's message. Such that with probability at least $\varepsilon/2-2^{-\secp} >\varepsilon/4$, over $\wi_2$:
% \begin{enumerate}
    
%     \item 
%     The above three conditions hold (for $\cmt,\obfC$ fixed by $z$).
%     \item
%     The WI verifier $\wiV$ accepts the proof given by $\wimP_z$ (for the statement $\Psi$ fixed by $z$).
%     \item
%     The extractor $\zkE^{\wimP_z,\ins}(1^{4/\varepsilon/},\Psi,\wi_1,\wi_2,\wi_3)$ outputs $\wit_T$ that does not attest that $\zkPCT$ is a zero encryption. 
% \end{enumerate}
% By the fact that $\ins\notin \lang$, the above contradicts the instance-dependent proof of knowledge guarantee of the the \WI proof. Indeed, by (1), the only witness that $\Psi$ can have must attest that $\zkPCT$ is a zero encryption. By  (2), the extracted witness $\wit_T$ must be such a witness except with negligible probability $\secp^{-\omega(1)}$, which contradicts (3) and the fact that $\varepsilon/4>\secp^{-O(1)}$.
% \end{proof}
% This concludes the proof of soundness.
% \end{proof}
% \nir{consider extedning to AOK, or remarking about it}.

% \begin{proposition}\label{prp:sim}
% \proref{fig:wzk_prot} is weak zero-knowledge against explainable verifiers.
% \end{proposition}

% \begin{proof}
% \def \ranmal {r^*}  
% We describe the simulator $\zkS$. Throughout, we assume w.l.o.g that $\zkmV$ outputs its view consisting of its random coins and prover messages. (Otherwise, we consider a new verifier of this form, along with a new distinguisher who computes internally the original verifier output, and then applies the original distinguisher.)

% \medskip
% \paragraph{$\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
% \begin{itemize}

% \item
% Sample coins $\ranmal$ for $\zkmV_\secp$. Henceforth, $\zkmV_{\ranmal}$ denotes the corresponding (deterministic) verifier.
% \item
% Sample a first $\WI$ message and state $(\wi_1,\tau_\zkP)\gets \wiP_1^\ins(1^\secp)$ and feeds them to $\zkmV_{\ranmal}$. 
% \item
% If the verifier aborts, output $(\ranmal,\wi_1,\bot)$.
% \item 
% Obtain $(\wi_2,\cmt,\zkVCT,\obfC, \zkVCT',\rsrePK')$ from $\zkmV_{\ranmal}$.
% \item
% Construct the ({\em homomorphic simulation}) circuit $\HC(r)$ that given an input $r$:
% \begin{itemize}
% \item
% Constructs a distinguisher $\rsremD'(\zkPCT)$ for the RSR encryption that given a ciphertext $\zkPCT$: 
% \begin{itemize}
% \item
% Samples a third $\WI$ message $$\wi_3 \gets \wiP_2^{\ins}(\Psi,r,\wi_1,\wi_2;\tau_\zkP)$$
% for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK')$, using as the witness the randomness $r$ attesting that $\cmt=\COM(0;r)$.
% \item
% Runs $\zkmD_\secp(\ranmal,\wi_1,(\zkPCT,\wi_3))$.
% \end{itemize}
% \item 
% Applies the decryptor
% $$
% \tilde u \gets \rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon})\enspace,
% $$
% and output $\tilde u$.
% \end{itemize}  
% All randomness required by the above, as well as the WI prover state $\tau_\zkP$ are hardwired to $\HC$.
% \item
% Compute $\evciph = \fheEv(\HC,\zkVCT)$.

% \item
% If $\obfC(\evciph)=1$: 
% \begin{itemize}
% \item
% Sample $\zkPCT\gets \rsreE_{\rsrePK'}(1)$. 
% \item
% Sample a third $\WI$ message 
% $$\wi_3 \gets \wiP_2^{\ins}(\Psi,\evciph,\wi_1,\wi_2;\tau_\zkP)$$
% for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK')$, using as the witness $\evciph$ attesting that $\obfC(\evciph)=1$. 
% \end{itemize}
% \item
% Otherwise:
% \begin{itemize}
% \item
% Sample $\zkPCT\gets \rsreE_{\rsrePK'}(0)$. 
% \item
% Sample a third $\WI$ message 
% $$\wi_3 \gets \wiP_2^{\ins}(\Psi,r',\wi_1,\wi_2;\tau_\zkP)$$
% for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK')$, using as the witness the randomness $r'$ attesting that $\zkPCT\gets \rsreE_{\rsrePK'}(0;r')$. 
% \end{itemize}
% \item
% Output $(\ranmal,\wi_1,(\zkPCT,\wi_2))$.
% \end{itemize}

% \paragraph{Simulation validity.} The simulator clearly runs in polynomial time (in its input length). We focus on proving validity. Let $\zkmV=\set{\zkmV_\secp}_\secp$ be a polynomial-size explainable verifier, let $\zkmD=\set{\zkmD_\secp}_\secp$  be a polynomial-size distinguisher, and let $\varepsilon(\secp)=\secp^{-O(1)}$. 
% % Fix any $\secp$, and $x\in \lang\cap\zo^\secp$ such that the message sent by $\zkmV_\secp$ is explainable (i.e., it is consistent with some honest verifier message as specified in \proref{fig:wzk_prot}).

% We first consider an alternative simulator $\zkS'$ that is given as additional input a witness $\wit\in\RL(\ins)$, and computes witness indistinguishable proofs in trapdoor mode. Specifically, $\zkS'$ samples the first \WI message and state $(\wi_1,\tau_\zkP)\gets \wibP_1^{\ins,\wit}(1^\secp)$ using the trapdoor prover $\wibP_1$ instead of the real prover $\wiP_1$. We similarly consider an alternative honest prover $\zkP'$ that samples the \WI message and state using the trapdoor prover $\zkbP_1$. We argue that the views generated by $\zkS'$ and $\zkP'$ are indistinguishable from those generated by $\zkS$, and $\zkP$, respectively.

% \begin{claim}
% There exists a negligible $\mu(\secp)$ such that for all $\secp\in\Nat$, $\ins\in\lang\cap\zo^\secp$, and $\wit\in\RL(\ins)$,
% \begin{align*}
% \zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) &\approx_{\zkmD_\secp,\mu}  \zkS'(\ins,\wit,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) \enspace, \\
% \view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins) &\approx_{\zkmD_\secp,\mu}  \view_{\zkmV_\secp}\prot{\zkP'(\wit)}{\zkmV_\secp}(\ins)\enspace.
% \end{align*}

% \begin{proof}
% Both for $\zkS$ and $\zkS'$ the entire simulation can be performed given the first $\WI$ message $(\wi_1,\tau_\zkP)$ as external input. Thus any distinguisher between the two simulators directly translates to a a distinguisher that violates the indistinguishability of trapdoor proofs in the underlying instance-dependent \WI. The same holds for $\zkP$ and $\zkP'$.
% \end{proof}

% \end{claim}

% From hereon, we focus on proving that $\zkS'$ successfully simulates $\zkP'$.
% \begin{claim}\label{clm:sim_val}
% There exists a negligible $\nu(\secp)$ such that for all $\secp\in\Nat$, $\ins\in\lang\cap\zo^\secp$, and $\wit\in\RL(\ins)$,
% \begin{align*}
% \zkS'(\ins,\wit,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon}) \approx_{\zkmD_\secp,\nu} \view_{\zkmV_\secp}\prot{\zkP'(\wit)}{\zkmV_\secp}(\ins)\enspace.
% \end{align*}
% \end{claim}

% \begin{proof}
% \nir{this proof is faulty --- simulator cannot resample in $\rsremD'$ \WI proofs, at least not w/o the equivocation state, which we cannot give it.
% Proof should still work w/o resampling, but have to be more careful.
% }

% First, since the verifier $\zkmV$ is explainable, the generated transcript in each f the two distributions is explainable, except with negligible probability $\mu(\secp)$. Thus, it suffices to prove indistinguishability conditioned on the transcript being explainable. Also, since the first messages $\wi_1$ of $\zkS'$ and $\zkP'$ are distributed identically, it suffices to show indistinguishability for each fixed first message $\wi_1$, and verifier randomness $\ranmal$ such that the message sent by $\zkmV_{\ranmal}$ is explainable. Henceforth, we fix such $\ranmal$, $\wi_1$, and explainable verifier message $m_\zkV$ (we do not fix the state \WI prover state $\tau_\zkP$, but only condition on $\wi_1$). If the message $\zkV$ is an abort, then $\zkS'$ and $\zkP'$ behave identically (also aborting). Otherwise, the message is of the form $m_\zkV = (\wi_2,\cmt,\zkVCT,\obfC, \zkVCT',\rsrePK')$.

% Let $\Delta$ be the advantage of the distinguisher $\rsremD'$ (as defined in the simulation procedure) in distinguishing zero-encryptions from one-encryptions:
% \begin{align*}\Delta := \abs{\underset{\rsremD',\rsreE}{\EE}\[\rsremD'(\rsreE_{\rsrePK'}(0))- \rsremD'(\rsreE_{\rsrePK'}(1))\]}\enspace.
% \end{align*}

% We consider two cases.

% \paragraph{Case 1: $\Delta > \varepsilon$.} Let $u$ be the target string underlying the obfuscated CC program $\obfC$, and recall that $\zkVCT'\in \rsreE_{\rsrePK'}(u)$. Then by the random self reducibility of $\rsre$, with overwhelming probability $1-2^{-\secp}$, it holds that
% $$
% \rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon}) = u\enspace,
% $$
% in which case, $\HC(r) = u$. Assume that this is indeed the case.

% By the correctness of $\fhe$, the ciphertext $\evciph=\fheEv(\HC,\evciph)$ obtained by the simulator satisfies:
% $$
% \fheD_{\fheK}(\evciph) = u\enspace,
% $$
% and thus by the one-sided correctness of the CC obfuscator $\O$,
% $$
% \obfC(\evciph) = 1\enspace.
% $$
% In this case, the simulator generates a prover message $(\zkPCT,\wi_3)$ exactly like the honest prover, with the exception of using $\evciph$ as the witness for computing $\wi_2$, instead of $\wit \in \RL(\ins)$. By the perfect witness indistinguishability of trapdoor proofs, it follows that in this case the messages $\wi_3$ generated by $\zkP'$ and $\zkS'$ are distributed identically, and thus so are the view generated by $\zkP'$ and that generated by $\zkS'$.

% Overall, in case 1 (and conditioned the fixed $\ranmal,\wi_1,m_\zkV$),
% $$ \view_{\zkmV_\secp}\prot{\zkP'(\wit)}{\zkmV_\secp}(\ins))  \approx_{\zkmD_\secp,2^{-\secp}} \zkS'(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace.
% $$

% \paragraph{Case 2: $\Delta \leq \varepsilon$.} Here we consider two sub-cases according to whether the simulator still obtains a ciphertext $\evciph$ such that $\obfC(\evciph)=1$ or not. In case it does obtain such $\evciph$, the analysis proceeds exactly as in case 1. 

% Henceforth, we assume that the simulator does not obtain such a witness, in which case, the simulator samples $\zkPCT \gets \rsreE_{\rsrePK'}(0;r')$ and uses $r'$ as the witness for computing $\wi_2$. 

% To complete the proof of validity we prove that in this case
% $$
% \ranmal,\rsreE_{\rsrePK'}(0;r'),\wi_2(r') \hspace{2mm} \approx_{\zkmD_\secp,\varepsilon}  \hspace{2mm} \ranmal, \rsreE_{\rsrePK'}(1;r'),\wi_2(\wit)\enspace, 
% $$
% where $\wi_2(r')$ and $\wi_2(\wit)$ denote the \WI messages computed using the witnesses $r'$ and $\wit$, respectively.

%   To prove this we consider several hybrids and prove that they are indistinguishable.

% \paragraph{$\hyb_0$:} In this hybrid, the prover message is generated as $\rsreE_{\rsrePK'}(1;r'),\wi_2(\wit)$ like in the real protocol.

% \paragraph{$\hyb_1$:} In this hybrid, the $\WI$ message $\wi_2$ is generated using as as a witness the randomness $r$ attesting that $\cmt = \COM(0;r)$ instead of using $\wit$. This hybrid is distributed identically to the previous one by the perfect witness indistinguishability of the proof system. 


% \paragraph{$\hyb_2$:} In this hybrid, the ciphertext $\zkPCT \gets \rsreE_{\rsrePK'}(0)$ is generated as an encryption of zero instead of one. This hybrid is $(\zkmD_\secp,\varepsilon)$-close to the previous one by our assumption that $\Delta\leq \varepsilon$, and the definition of $\rsremD'$.

% \paragraph{$\hyb_3$:} In this hybrid, the $\WI$ message $\wi_2$ is generated using as as a witness the randomness $r'$ attesting that $\zkPCT = \rsreE_{\rsrePK'}(0;r')$ instead of using the randomness $r$ for the commitment. This hybrid is distributed identically to the previous one by the perfect witness indistinguishability of the proof system. In this hybrid, the prover message is generated as $\rsreE_{\rsrePK'}(0;r'),\wi_2(r')$ like in the simulated protocol.

% Overall, in case 2 (and conditioned the fixed $\ranmal,\wi_1, m_\zkV$),
% $$ \view_{\zkmV_\secp}\prot{\zkP'(\wit)}{\zkmV_\secp}(\ins))  \approx_{\zkmD_\secp,\varepsilon} \zkS'(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace.
% $$
% %
% In total (and without any conditions),
% $$ \view_{\zkmV_\secp}\prot{\zkP'(\wit)}{\zkmV_\secp}(\ins))  \approx_{\zkmD_\secp,\mu+2^{-\secp}+\varepsilon} \zkS'(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace,
% $$
% where $\mu$ accounts for non-explainable verifier messages, $2^{-\secp}$ is the error in the first case and $\varepsilon$ is the error in the second. Thus \clmref{clm:sim_val} follows with $\nu=\mu+2^{-\secp}$.
% \end{proof}
% This completes the proof of \prpref{prp:sim}.
% \end{proof}

% \begin{remark}[On the use of perfect indistinguishability of trapdoor proofs]
% In the above proof, perfect witness indistinguishability is used in several places. It can be replaced with statistical indistinguishability at the account of making the proof slightly more complicated. It cannot be replaced, however, with computational indistinguishability. A place where perfect (or statistical) indistinguishability becomes essential is when invoking indistinguishability of proofs using as the witness the randomness $r$ encrypted in $\fheCT_\zkV$ and proofs using $\wit$ (or other witnesses). Indeed, the witness $r$ is only implicitly determined and cannot be obtained efficiently by a computational reduction. 
% \end{remark}

% \begin{remark}[On using relaxed random self-reducible encryption]
% We rely on relaxed RSR encryption by slightly tweaking the protocol. Specifically, in the protocol, the encryption $\zkPCT$ will be under the alternative RSR encryption algorithm $\rsretE$. The simulation and analysis remain the same.
% \end{remark}

% \subsection{A Two-Message Protocol}\label{sec:2wzk_expl}

% In this section, we construct a two-message \WZK argument against explainable verifiers. We start by presenting the protocol and then proceed to analyze it.

% \nir{TODO. think how to unify}

===============================================

\subsubsection{Analysis}
We now analyze the protocol. We first show that it is sound, and then that it is $\WZK$ against explainable verifiers.

\begin{proposition}
\proref{fig:wzk_prot} is sound.
\end{proposition}
\begin{proof}
Assume toward contradiction that there exists a polynomial-size (w.l.o.g deterministic) prover $\zkmP=\set{\zkmP_\secp}$ that (for infinitely many $\secp\in\Nat$) breaks soundness with noticeable probability $\varepsilon(\secp) =\secp^{-O(1)}$. Fix $\secp\in\Nat$ and $\ins\in \zo^\secp\setminus \lang$ such that $\zkmP_\secp$ convinces the verifier of accepting with probability $\varepsilon$. 

\paragraph{Augmenting the interaction with extraction.} We parse any verifier message $(\cm_2,\wi_1,\cmt,\zkVCT,\obfC,\zkVCT',\rsrePK')$, as two parts $(\cm_2,z)$. For any $z$, we consider a sender $\commS_z$ whose first message is the same $\cm_1$ output by $\zkmP_\secp$, and given a message $\cm_2$ from the receiver $\comR$, computes the third message $\cm_3$ by running $\zkmP_\secp$ on $(\cm_2,z)$, emulating a message form $\zkV$. For any transcript $T=(\cm_1,(\cm_2,z),(\cm_3,\zkPCT,\wi_2))$ of an execution between $\zkmP_\secp$ and $\zkV$, we consider the result $s_T$ of running the witness extractor $s_T \gets \zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$. (Note that $s_T$ is a random variable that may depend on $T$ and the extractor's coins.)

Let $F$ be the event, over a transcript $T$ and coins of the extractor $\zkE$, that: 
\begin{enumerate}
    \item
    $\zkV$ successfully verifies the commitment transcript $(\cm_1,\cm_2,\cm_3)$,
    \item $\zkV$ accepts the WI argument $(\wi_1,\wi_2)$,
    \item
    the
    the extracted string $s_T$ does {\bf not} attest that $\zkPCT$ is a zero encryption; that is, $s_T$ is {\bf not} randomness $r'$ such that $\zkPCT = \rsreE(0;r')$.
\end{enumerate} 
%
We next consider several hybrid experiments and show that the probability that $F$ occurs is preserved through these experiments, upto a negligible difference. To reach a contradiction, we show that $F$ occurs in the first hybrid with probability at least $\varepsilon$ and with probability at most $\varepsilon/2$ in the last hybrid. This is a contradiction since the gap $\varepsilon/2$ is noticeable. In what follows, in each hybrid $i$, we will denote by  $p_i$ the probability that $F$ occurs in that hybrid.  

\paragraph{$\hyb_0$:} This is the real protocol.

\begin{claim}
$p_0 \geq \varepsilon$.
\end{claim}
\begin{proof}
By definition, whenever $\zkV$ accepts, it decrypts $\zkPCT$ to $1$; thus, by the correctness of $\rsre$, the ciphertext $\zkPCT$ cannot be opened to an encryption of $0$.  The claim now follows from the fact that $\zkmP_\secp$ convinces $\zkV$ with probability $\varepsilon$.
\end{proof}


\paragraph{$\hyb_1$:} In this hybrid, $\zkVCT'$ is an encryption of $0^\secp$ instead of the target $u$. 

\begin{claim}
$\abs{p_0-p_1} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the semantic security of the scheme $\rsre$. Indeed, given a noticeable difference between $p_0$ and $p_1$, we can distinguish an RSR encryption of a random $u$ from one of $0^\secp$, by emulating an interaction between $\zkmP_\secp$ and $\zkV$, running the extractor, and testing whether $F$ occurs. 
\end{proof}



\paragraph{$\hyb_2$:} In this hybrid, the obfuscation $\obfC \gets \ccSim(1^\secp,1^\ell)$ is simulated rather than an obfuscation of $\CC{\fheD_{\fheK},u}$, where $\ell$ is the size of the decryption circuit $\fheD_{\fheK}$.


\begin{claim}
$\abs{p_1-p_2} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the CC simulation guarantee. Indeed, given a noticeable difference between $p_1$ and $p_2$, we can distinguish, given $\fheK$, an obfuscation of $\CC{\fheD_{\fheK},u}$ for a random $u$, from a simulated obfuscation contradicting the CC guarantee. Using the fact that now $\zkVCT'$ is an encryption of $0^\secp$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}


\paragraph{$\hyb_3$:} In this hybrid, $\zkVCT$ is an encryption of $0^\secp$ instead of the commitment randomness $r$.


\begin{claim}
$\abs{p_2-p_3} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by the semantic security of the FHE scheme $\fhe$. Indeed, given a noticeable difference between $p_2$ and $p_3$, we can distinguish, an encryption of a random $r$ from an encryption of $0^\secp$. Since now the FHE key $\fheK$ is not needed to compute the obfuscation $\obfC$, we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}


\paragraph{$\hyb_4$:} In this hybrid, $\cmt$ is a commitment to $1$ instead of $0$.

\begin{claim}
$\abs{p_3-p_4} \leq \secp^{-\omega(1)}$.
\end{claim}
\begin{proof}
The claim follows by hiding of the commitment. Given a noticeable difference between $p_3$ and $p_4$, we can distinguish, a commitment to zero from a commitment to one. In this hybrid, $\zkVCT$ no longer depends on the commitment randomness, so we can again emulate an interaction between $\zkmP_\secp$ and $\zkV$. 
\end{proof}

.

\medskip\noindent
It is left to show that in $\hyb_4$, $F$ occurs with probability at most $\varepsilon/2$. 

\begin{claim}
$p_4 \leq \varepsilon/2$.
\end{claim}
\begin{proof}
Assume toward contradiction that $p_4 > \varepsilon/2$. First, observe that in hybrid $\hyb_4$:
\begin{itemize}
\item
$\ins\notin \lang$.
\item
$\cmt \in \COM(1)$, and by perfect binding there does not exist $r$ such that $\cmt = \COM(0;r)$.
\item
By the CC simulation guarantee, except with negligible probability $2^{-\secp}$, there does not exist $\evciph$ such that $\obfC(\evciph) = 1$.
\end{itemize}
In particular, we can fix the second part $z$ of the  verifier's message such that with probability at least $\varepsilon/2-2^{-\secp}$, over $\cm_2$:
\begin{enumerate}
    
    \item 
    The above three conditions hold (for $\cmt,\obfC$ fixed by $z$).
    \item
    The WI verifier $\wiV$ accepts the argument (for the statement $\Psi$).
    \item
    The commitment verifier $\comV$ accepts the transcript $(\cm_1,\cm_2,\cm_3)$.
    \item
    The extractor $\zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$ outputs $s_T$ that does not attest that $\zkPCT$ is a zero encryption. 
\end{enumerate}
Invoking the soundness of the $\WI$ argument, it follows that with probability at least $\varepsilon/2-2^{-\secp} \secp^{-\omega(1)}\gg 2^{-\secp}$, over $\cm_2$:
\begin{enumerate}
    \item 
    The commitment verifier $\comV$ accepts the transcript $(\cm_1,\cm_2,\cm_3)$.
    \item
    $\exists r'$ such that $(\cm_1,\cm_2,\cm_3) \in \comS(r')$, and $r'$ attests that $\zkPCT$ is a zero encryption.
    \item
    The extractor $\zkE^{\commS_z}(1^\secp,1^{4/\varepsilon})$ outputs $s_T$ that does not attest that $\zkPCT$ is a zero encryption. In particular, $s_T\neq r'$. 
\end{enumerate}
This contradicts the extraction guarantee of the commitment.
\end{proof}
This concludes the proof of soundness.
\end{proof}

\begin{proposition}\label{prp:sim}
\proref{fig:wzk_prot} is weak zero-knowledge against explainable verifiers.
\end{proposition}

\begin{proof}
\def \ranmal {r^*}  
We describe the simulator $\zkS$. Throughout, we assume w.l.o.g that the malicious verifier $\zkmV$ outputs its view consisting of its random coins and prover messages.
(Otherwise, we consider a new verifier of this form, along with a new distinguisher who computes internally the original verifier output, and then applies the original distinguisher.)

\medskip
\paragraph{$\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
\begin{enumerate}
\item
Sample coins $\ranmal$ for $\zkmV_\secp$. Henceforth, $\zkmV_{\ranmal}$ denotes the corresponding (deterministic) verifier.
\item
Sample a random $r'\gets \zo^\secp$ and a first commitment message and state $(\cm_1,\tau)\gets \comS(r')$ corresponding to a commitment to $r'$. Store the randomness $r_{\cm}$ used to generate the commitment. Feed $\cm_1$  to $\zkmV_{\ranmal}$. 
\item
If the verifier aborts, output $(\ranmal,\cm_1,\bot)$.
\item \label{stp:ver_mes}
Obtain $(\cm_2,\cmt,\zkVCT,\obfC, \zkVCT',\rsrePK',\wi_1)$ from $\zkmV_{\ranmal}$
\item
Compute the third commitment message $\cm_3 \gets \comS(\cm_1,\cm_2;\tau)$.
\item
Construct the ({\em homomorphic simulation}) circuit $\HC(r)$ that given an input $r$:
\begin{itemize}
\item
Construct a distinguisher $\rsremD'(\zkPCT)$ for the RSR encryption that given a ciphertext $\zkPCT$: 
\begin{itemize}
\item
Samples at random a second $\WI$ message $$\wi_2 \gets \wiP(\Psi,r,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r$ attesting that $\cmt=\COM(0;r)$.
\item
Runs $\zkmD_\secp(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{itemize}
\item 
Applies the decryptor
$$
\tilde u \gets \rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon})\enspace,
$$
and output $\tilde u$.
\end{itemize}  
All randomness required by the above is hardwired into $\HC$.
\item
Compute $\evciph = \fheEv(\HC,\zkVCT)$.

\item \label{stp:td1}
If $\obfC(\evciph)=1$: 
\begin{itemize}
\item
Sample $\zkPCT\gets \rsreE_{\rsrePK'}(1)$. 
\item
Sample a second $\WI$ message 
$$\wi_2 \gets \wiP(\Psi,\evciph,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness $\evciph$ attesting that $\obfC(\evciph)=1$. 
\end{itemize}
\item
Otherwise:\label{stp:td2}
\begin{itemize}
\item
Compute $\zkPCT =  \rsreE_{\rsrePK'}(0;r')$, where $r'$ is the randomness underlying the extractable commitment. 
\item
Sample a second $\WI$ message 
$$\wi_2 \gets \wiP(\Psi,(r',r_\cm),\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r'$ attesting that $\zkPCT\gets \rsreE_{\rsrePK'}(0;r')$ and the commitment randomness $r_\cm$. 
\end{itemize}
\item
Output $(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{enumerate}

\paragraph{Simulation validity.} The simulator clearly runs in polynomial time (in its input length). We focus on proving validity. Let $\zkmV=\set{\zkmV_\secp}_\secp$ be a polynomial-size explainable verifier, let $\zkmD=\set{\zkmD_\secp}_\secp$  be a polynomial-size distinguisher, and let $\varepsilon(\secp)=\secp^{-O(1)}$. 
% Fix any $\secp$, and $x\in \lang\cap\zo^\secp$ such that the message sent by $\zkmV_\secp$ is explainable (i.e., it is consistent with some honest verifier message as specified in \proref{fig:wzk_prot}).

We consider a sequence of hybrid simulators that transition from the simulator to the prover, and prove that the views generated by each two consecutive hybrids are indistinguishable.

\paragraph{$\zkS_0$:} This is the real simulator $\zkS$.

\paragraph{$\zkS_1$:} This simulator is the same as $\zkS$, only that in Step \ref{stp:td2}, if it needs to give an argument (due to unsuccessful extraction of a proper $\evciph$), it uses the witness $\wit$, instead of $(r',r_\cm)$.
%\daksh{Here, I suggest that instead of using the witness $\wit$ only when there is unsuccessful extraction of a proper $\evciph$, the simulator {\em always} uses $\wit$ to generate the WI arguments (that is, in steps 6, 8, 9). Even though its possible that the distinguisher breaks WI under the hood, the overall view at the end of the simulation (including the probability of unsuccessful extraction of $\evciph$) cannot change. Then it seems like we can switch directly from $S_2$ to $P_0$ below, without requiring any non-uniform fixing. But then why do we even need $\mathsf{com}(0;r)$ from the receiver? What do you think? I may be missing something.}

\paragraph{$\zkS_2$:} This simulator is the same as $\zkS_1$, only that instead of an extractable commitment $(\cm_1,\cm_2,\cm_3)$ to $r'$, it provides a commitment to $0^\secp$.

\paragraph{$\zkS_3$:} This simulator is inefficient. It acts the same as $\zkS_2$, only that:
\begin{itemize}
    \item
    It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
    \item
    Then it finds the commitment randomness $r$, and uses it to provide proofs both in Step \ref{stp:td1} and in Step \ref{stp:td2}.
\end{itemize}

\paragraph{$\zkP_1$:} This simulator is also inefficient. It acts the same as the honest prover $\zkP$, only that:
\begin{itemize}
    \item
    It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
    \item
    Then it finds the commitment randomness $r$, and uses it to provide the \WI argument.
\end{itemize}

\paragraph{$\zkP_0$:} This simulator emulates the real prover.

To deduce the validity of the simulator, we prove:
\begin{claim}\label{clm:wzk_main}
There exists a negligible $\nu(\secp)$ such that for all $\secp\in\Nat$, $\ins\in\lang\cap\zo^\secp$, $\wit\in\RL(\ins)$, $i\in [3]$,
\begin{align*}
\zkS_{i-1}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\nu}
\zkS_{i}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace,\\
\zkS_{3}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\varepsilon+2^{-\secp}}
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins) \enspace,\\
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins)  &\approx_{\zkmD_\secp,\nu}
\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\enspace.
\end{align*}
\end{claim}

\begin{proof}
We prove the indistinguishability of each two consecutive hybrid simulators.

\medskip\noindent
\underline{$\zkS \approx \zkS_1$:} Recall that the only difference between these two simulators is that $\zkS_1$ uses the witness $\wit$ in Step \ref{stp:td2}, instead of $(r',r_{\cm})$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument.

$\wimV$ runs $\zkS$ to sample a transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS$ produces. Instead, it outputs as the first \WI message the message $\wi_1$ produced by $\zkmV$ during the simulation, as well as the statement $\Psi$ and $\wit_0=(r',r_\cm)$ and $\wit_1 = \wit$ as the two witnesses. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generated by $\zkS$, except that $\wi_2$ generated by $\zkS$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\zo$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkS_1 \approx \zkS_2$:} Recall that the only difference between these two simulators is that $\zkS_2$ commits to $0^\secp$ instead of to $r'$ like $\zkS_1$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$, then we construct a receiver $\commR$ that breaks the indistinguishability of the extractable commitment with the same advantage $\delta$. 

$\commR$ emulates $\zkS_1$, when sampling $r'$, $\commR$ submits to the challenger $s_1=r'$ and $s_2 = 0^\secp$. Then, instead of sampling $\cm_1$ as part of the simulation, $\commR$ obtains it from an outside challenger. It proceeds with the emulation of $\zkS_1$, feeding $\cm_1$ to $\zkmV$, and obtaining $\cm_2$ as part of $\zkmV$'s message. $\commR$ sends  $\cm_2$ to the challenger and obtains $\cm_3$. It then performs the rest of the emulation using $\cm_3$ (note that $\zkS_1$ no longer requires the randomness underlying the commitment in Step \ref{stp:td2}). 

It is left to observe that for each $i\in\set{1,2}$, when the challenger commits to $s_i$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\commR$ has advantage $\delta$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkS_2 \approx \zkS_3$:} Recall that the difference between these two simulators is that $\zkS_3$ aborts if the verifier's message is not explainable, and if it is uses the commitment randomness $r$ as the witness in Steps \ref{stp:td1} and $\ref{stp:td2}$, instead of $\evciph$ and $\wit$, respectively. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the simulator $\zkS_3$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two simulators are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkS$ from $\zkS_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkS_2$ starting from the point it obtains the message from $\zkmV$ (Step \ref{stp:ver_mes}), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS_2$ produces. Instead: 
\begin{itemize}
    \item If the transcript reaches Step \ref{stp:td1} (corresponding to successful extraction of $\evciph$), $\wimV$ sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_2 = \evciph$ and $\wit_3 = r$.
    \item
    If the transcript reaches Step \ref{stp:td2} (corresponding to unsuccessful extraction of $\evciph$), $\wimV$ sends to the challenger $\wi_1$ and $\Psi$ with witnesses $\wit_2 = \wit$ and $\wit_3 = r$.
\end{itemize}
It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkS_2$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\set{2,3}$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge. 

\medskip\noindent
\underline{$\zkP_1 \approx \zkP$:} We jump to prove this indistinguishability as it is very similar to the previous one (the tired reader is advised to skip it).

Recall that the difference between these two provers is that $\zkP_1$ aborts if the verifier's message is not explainable, and if it is, uses the commitment randomness $r$ as the witness when proving $\Psi$ instead of $\wit$ like $\zkP$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two provers with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the prover $\zkP_1$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two provers are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkP$ from $\zkP_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkP$ starting from the point it obtains the message from $\zkmV$ (the third protocol message), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkP_1$ produces. Instead, it sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_0 = \wit$ and $\wit_1 = r$. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkP$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs. 

It is left to observe that for each $i\in\set{0,1}$, the generated view is distributed identically to that generated by $\zkP_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge.

\medskip\noindent
\underline{$\zkS_3 \approx \zkP_1$:} Note that up to receiving the verifier's $\zkmV$ message, and adding the generation of $\cm_3$, the views generated by the two simulators are distributed identically. Thus, to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability of these two simulators, it suffices to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability conditioned on any fixing of the first prover message, verifier randomness $\ranmal$ and message, and $\cm_3$. Note that if the verifier's message is not explainable, \daksh{Previously, it said not explainable or $\bot$ -- I found this confusing. Moreover, since $\bot$ is not explainable, I just removed ``or $\bot$''.} both simulators abort, and thus we concentrate on the case that the verifier's message is explainable. From hereon consider such a fixing and let $r$ be the corresponding randomness.

Let $\Delta$ be the advantage of the probabilistic distinguisher $\rsremD'$ (as defined in the simulation procedure) in distinguishing zero-encryptions from one-encryptions:
\begin{align*}\Delta := \abs{\underset{\rsremD',\rsreE}{\EE}\[\rsremD'(\rsreE_{\rsrePK'}(0))- \rsremD'(\rsreE_{\rsrePK'}(1))\]}\enspace.
\end{align*}
%
We consider two cases.

\paragraph{Case 1: $\Delta > \varepsilon$.} Let $u$ be the target string underlying the obfuscated CC program $\obfC$, and recall that $\zkVCT'\in \rsreE_{\rsrePK'}(u)$, due to explainability. Then by the random self reducibility of $\rsre$, with overwhelming probability $1-2^{-\secp}$, over the coins of $\rsretD$, it holds that
$$
\rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon}) = u\enspace,
$$
in which case, $\HC(r) = u$. Assume that this is indeed the case.

By the correctness of $\fhe$, the ciphertext $\evciph=\fheEv(\HC,\evciph)$ obtained by the simulator $\zkS_3$ satisfies:
$$
\fheD_{\fheK}(\evciph) = u\enspace,
$$
and thus by the one-sided correctness of the CC obfuscator $\O$,
$$
\obfC(\evciph) = 1\enspace.
$$
This corresponds to successful extraction of $\evciph$, and will result in the simulator $\zkS_3$ behaving identically to the prover $\zkP_1$ (in Step \ref{stp:td1}) --- sampling $\zkPCT$ as a one encryption and $\wi_2$ using the witness $r$. 

Thus, in case 1, we have $(\zkmD_\secp,2^{-\secp})$-indistinguishability.

\paragraph{Case 2: $\Delta \leq \varepsilon$.} Here we consider two sub-cases according to whether the simulator still obtains a ciphertext $\evciph$ such that $\obfC(\evciph)=1$ or not. In case it does obtain such $\evciph$, the simulator behaves exactly like $\zkP_1$. Henceforth, we assume that the simulator does not obtain such a witness, in which case it reaches Step \ref{stp:td2}. Here the difference between the simulator $\zkS_3$ and prover $\zkP_1$ is that the first samples $\zkPCT \gets \rsreE_{\rsrePK'}(0)$, whereas the second samples $\zkPCT \gets \rsreE_{\rsrePK'}(1)$. The advantage of $\zkmD_\secp$ in distinguishing the two is exactly the advantage $\Delta \leq \varepsilon$ of $\rsremD'$. This completes the proof of this case, and of \clmref{clm:wzk_main}.
\end{proof}



\begin{remark}[On using relaxed random self-reducible encryption]
We can rely on relaxed RSR encryption by slightly tweaking the protocol. Specifically, in the protocol, the encryption $\zkPCT$ will be under the alternative RSR encryption algorithm $\rsretE$. The simulation and analysis remain the same.
\end{remark}

==> zkproof.tex <==
\section{Semi-Composable Zero-Knowledge}
\label{sec:zk-proof}

\begin{lemma}
\proref{fig:parallel_zk} is quantum semi-composable computational zero-knowledge.
\end{lemma}

\begin{proof}

We define the following collections of random variables (each indexed by $\secp$). Each is defined with respect to the adversary $\zkV^* = \{\zkV^*_\secp,\rho_\secp\}_{\secp \in \mathbb{N}}$ we are considering, as well as a sequence of honest party instance-witness pairs $\{\{x_{i,\secp} \in \cL \cap \{0,1\}^{\ell(\secp)}, w_{i,\secp} \in \cR_\cL\}_{i \notin I}\}_{\secp \in \mathbb{N}}$ for some polynomial $\ell(\cdot)$. Throughout, whenever we say abort, we mean that either the verifier aborts, or it fails to prove one of its WI statement (causing the prover to abort).

\begin{itemize}
    \item Let $\mathsf{Pr}^{\mathsf{Abort}}_{\mathsf{Real}}(\zkV^*)$ be the probability that $\zkV^*$ aborts in the real interaction with the $n$ honest provers.
    \item Let $\mathsf{Pr}^{\mathsf{Abort}}_{\mathsf{Sim}}(\zkV^*)$ be the probability that $\zkV^*$ aborts in $\zkSimNoAbort$ (i.e. the outcome is $\bot$).
    \item Let $\zkSim(\zkV^*) \coloneqq \{\zkSim(1^\secp,1^n,I,\zkV^*_\secp,O_{\rho_\secp})\}_{\secp \in \mathbb{N}}$.
    \item Let $\zkSimNoAbort(\zkV^*) \coloneqq \{\zkSimNoAbort(1^\secp,n,I,\zkV^*_\secp,\rho_\secp)\}_{\secp \in \bbN}$.
    \item Let $\zkSimAbort(\zkV^*) \coloneqq \{\zkSimAbort(1^\secp,n,I,\zkV^*_\secp,\rho_\secp)\}_{\secp \in \bbN}$.
    \item Let $\mathsf{RealNoAbort}(\zkV^*)$ be the distribution $\mathsf{Real}(\zkV^*)$ conditioned on there not being an abort.
    \item Let $\mathsf{RealAbort}(\zkV^*)$ be the distribution $\mathsf{Real}(\zkV^*)$ conditioned on there being an abort.
    \item Let $\mathsf{SimNoAbort}(\zkV^*)$ be the distribution $\zkSimNoAbort$ conditioned on there not being an abort (i.e. conditioned on the output not being $\bot$).
    \item Let $\mathsf{SimAbort}(\zkV^*)$ be the distribution $\zkSimAbort$ conditioned on there being an abort (i.e. conditioned on the output not being $\bot$).
\end{itemize}

%The following distributions will not be used explicitly in the hybrids, but will be convenient to define for the proof.

%\begin{itemize}
    %\item Let $\mathsf{RealNoAbort}_\bot(\zkV^*)$ be the distribution $\mathsf{Real}(\zkV^*)$, except that whenever an abort occurs, the distribution outputs $\bot$.
    %\item Let $\mathsf{RealAbort}_\bot(\zkV^*)$ be the distribution $\mathsf{Real}(\zkV^*)$, except that if an abort \emph{does not} occur, the distribution outputs $\bot$.
    %\item Let $\zkSim_\bot(\zkV^*)$ be the distribution $\zkSim(\zkV^*)$, except that whenever an abort occurs, instead of calling $\zkSimAbort$, the distribution outputs $\bot$.
    %\item Let $\zkSim^{\mathsf{Abort}}_\bot(\zkV^*)$ be the distribution produced by running only one iteration of the procedure described in step 2 of $\zkSimAbort$, except that whenever an abort \emph{does not} occur, the distribution outputs $\bot$.
%\end{itemize}

Following~\cite{BS20}, we show that $\mathsf{Real}(\zkV^*) \approx_c \zkSim(\zkV^*)$ via a sequence on hybrids. In particular, we show that 

\begin{align*}
    \mathsf{Real}(\zkV^*) &\substack{(1) \\ \equiv \\ \ } (1-\mathsf{Pr}^\mathsf{Abort}_\mathsf{Real}(\zkV^*))\mathsf{RealNoAbort}(\zkV^*) + (\mathsf{Pr}^\mathsf{Abort}_\mathsf{Real}(\zkV^*))\mathsf{RealAbort}(\zkV^*)\\
    &\substack{(2) \\ \approx_s \\ \ }(1-\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{RealNoAbort}(\zkV^*) + (\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{RealAbort}(\zkV^*)\\
    &\substack{(3) \\ \approx_c \\ \ } (1-\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{SimNoAbort}(\zkV^*) + (\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{RealAbort}(\zkV^*)\\
    &\substack{(4) \\ \approx_c \\ \ } (1-\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{SimNoAbort}(\zkV^*) + (\mathsf{Pr}^\mathsf{Abort}_\mathsf{Sim}(\zkV^*))\mathsf{SimAbort}(\zkV^*)\\
    &\substack{(5) \\ \approx_s \\ \ }\zkSim(\zkV^*),
\end{align*}

where 

\begin{enumerate}
    \item The equality $(1)$ follows by definition.
    \item The indistinguishability $(2)$ follows as a corollary of~\cref{claim:ind-non-abort}. Indeed, $\mathsf{RealNoAbort}_\bot(\zkV^*) \approx_c \zkSimNoAbort(\zkV^*)$ in particular implies that the difference in the probability that the verifier aborts in the real interaction versus the simulated interaction is negligible.
    \item The indistinguishability $(3)$ follows as a corollary of~\cref{claim:ind-non-abort}. This can be seen by considering two cases. First, if the probability that the verifier aborts in the real interaction is negligible, then $\mathsf{RealNoAbort}(\zkV^*) \approx_c \mathsf{SimNoAbort}(\zkV^*)$ directly follows from~\cref{claim:ind-non-abort}, and the indistinguishability follows. Otherwise, this probability is non-negligible, meaning that $\mathsf{RealAbort}(\zkV^*)$ is efficiently sampleable. Thus, a reduction to~\cref{claim:ind-non-abort} can sample from the distribution $\mathsf{RealAbort}(\zkV^*)$ whenever it receives $\bot$ from its challenger.\footnote{A more formal analysis of this can be found in~\cite[Lemma~3.2]{BS20}.}
    \item The indistinguishability $(4)$ follows as a corollary of~\cref{claim:ind-abort} via a similar analysis as the last step.
    \item The indistinguishability $(5)$ follows directly from~\cref{claim:sim-fail} and the definition of $\zkSim(\zkV^*)$.  
\end{enumerate}





\begin{claim}(The Simulation Fails with Negligible Probability)
\label{claim:sim-fail}
There is a negligible function $\mu(\cdot)$ such that for every $\secp \in \mathbb{N}$, $\Pr[\zkSim(\zkV^*) = \mathsf{FAIL}] \leq \mu(\secp)$.
\end{claim}

The proof of this claim is identically to the proof of~\cite[Claim 3.6]{BS20}, so we omit it.

It remains to show that simulation runs in expected polynomial time. However, the proof of this is identical to the proof of~\cite[Claim 3.3]{BS20}, so we omit it.

\end{proof}
